N$^2$: A Unified Python Package and Test Bench for Nearest Neighbor-Based Matrix Completion

Nearest neighbor (NN) methods have re-emerged as competitive tools for matrix completion, offering strong empirical performance and recent theoretical guarantees, including entry-wise error bounds, confidence intervals, and minimax optimality. Despite their simplicity, recent work has shown that NN approaches are robust to a range of missingness patterns and effective across diverse applications. This paper introduces N$^2$, a unified Python package and testbed that consolidates a broad class of NN-based methods through a modular, extensible interface. Built for both researchers and practitioners, N$^2$ supports rapid experimentation and benchmarking. Using this framework, we introduce a new NN variant that achieves state-of-the-art results in several settings. We also release a benchmark suite of real-world datasets, from healthcare and recommender systems to causal inference and LLM evaluation, designed to stress-test matrix completion methods beyond synthetic scenarios. Our experiments demonstrate that while classical methods excel on idealized data, NN-based techniques consistently outperform them in real-world settings.

==> appendices/library.tex <==
\section{\lib{} Package and Interface}\label{sec:library}

We now present our unified Python package, \lib{}, for nearest neighbor algorithms for matrix completion. In particular, we provide a class structure which abstracts the estimation procedure utilized in each different nearest neighbor method as well as the the $\distancemod$ and $\averagemod$ modules described above in \cref{sec:nn-overview}. On top of that, our library facilitates easy extensions to other nearest neighbors algorithms and other data types on top of scalars and distributions. For example, as long as a distance and average notion are well defined, our library can be easily applied to a matrix of images or text strings.

\paragraph{Class structure.} The core functionality of \lib{} is based on two abstract classes: \texttt{EstimationMethod} and \texttt{DataType}. 

\texttt{EstimationMethod} classes contain the logic to impute a missing entry such as how to use calculated distances. In the context of the modules in \cref{sec:nn-overview}, this class determines the weighting function or, in the context of $\drnn$ and $\autonn$, how to compose estimates. We separate this from the \texttt{DataType} abstraction because several estimation methods can be used for multiple data types. For example, \texttt{RowRowEstimator} implements the $\rownn$ procedure for any data type given to it, such as scalars or distributions.

\texttt{DataType} classes implement the $\distancemod$ and $\averagemod$ modules for any kind of data type (e.g. scalars which use squared distance and simple averaging). This abstract class allows for our package to extend to any data types beyond the ones we tested. For instance, a practitioner can easily add a \texttt{DataType} for text strings which uses vector embeddings to find distances and averages between between strings without needing to rewrite any of the estimation procedure.

\paragraph{Interface.} To use our library, a user simply has to instantiate a composite class \texttt{NearestNeighborImputer} with their \texttt{EstimationMethod} and \texttt{DataType} of choice. We provide constructor functions to automatically create popular \texttt{NearestNeighborImputer} classes such as a two-sided nearest neighbor estimator with the scalar data type. From a design pattern point of view, this is known as a \emph{Composite} design pattern \cite[pg. 163]{gamma1993design}. We use this design pattern so that anyone looking to customize the estimation procedure can do so for any kind of data type simultaneously. Similarly, with the exception of doubly robust estimators, each estimation procedure works out of the box with any data type that implements the \texttt{DataType} abstract class. The Doubly robust estimation method does not work out of the box with distributions because a subtraction operation is not well defined in the distribution space.

Finally, the user simply needs to input (i) a data matrix, (ii) a mask matrix which specifies which values are missing, and (iii) the row and column to impute. Thus, a user can test out different estimation procedures by changing just one line of code. Separately from the core functionality, we have also implemented several cross-validation classes which take in a \texttt{NearestNeighborImputer} class and find the best hyperparameters to use (e.g., distance thresholds and weights).

% NN 2 pages

% Star NN, Auto NN at most 1 page.

% library
% 1~1.5page

% case
% 3pages

==> appendices_workshop/case_study_details.tex <==
\section{Case Study Details}\label{app:case-studies}

The boxplots are generated using matplotlib's \cite{matplotlib} standard boxplot function. The box shows the first, second, and third quartiles. The bottom line shows the first quartile minus the 1.5$\times$ the interquartile range. The top line shows the third quartile plus 1.5$\times$ the interquartile range. All experiments are run on standard computing hardware (MacBook Pro with an M2 Pro CPU with 32 GB of RAM).

\subsection{Synthetic data generation}\label{app:synthetic_gen}

Generate $\measurement{i, t} = \sample{i, t} \sim N(\theta_{i, t}, \sigma^2)$, i.e., scalar matrix completion setting, with a linear factor structure $\theta_{i, t} = u_i v_t$. Row latent factors $u_i \in \real^4$ are i.i.d. generated across $i = 1, ..., N$, where each entry of $u_i$ follow a uniform distribution with support $[-0.5, 0.5]$; column latent factors $v_t \in \real^4$ are generated in an identical manner. The missingness is MCAR with propensity $p_{i, t} = 0.5$ for all $i$ and $t$. Further, the size of column and rows are identical $N = T$. For the left panel in \cref{fig:auto_perf}, the noise level is set as $\sigma = 0.001$ and for the right panel $\sigma = 1$.

% . \kc{@CC pls finish.} The missingness was 


\subsection{HeartSteps V1}

The mobile application was designed to send notifications to users at various times during the day to encourage anti-sedentary activity such as stretching or walking. Participants could be marked as unavailable during decision points if they were in transit or snoozed their notifications, so notifications were only sent randomly if a participant was available and were never sent if they were unavailable. 
To process the data in the framework of \cref{eq:model}, we let matrix entry $Z_{i, t}$ be the average one hour step count for participant $i$ and decision point $t$ when a notification is sent (i.e. $A_{i, t} = 1$) and unknown when a notification is not sent (i.e. $A_{i, t} = 0$). The treatment assignment pattern is represented as the 37 x 200 matrix visualized in \cref{fig:heart_missing}.  
We use the dataset downloaded from \url{https://github.com/klasnja/HeartStepsV1} (CC-BY-4.0 License).
% \cc{Is it worth mentioning the alternative framework with $X_{1}^{(1)}(i, t), ..., X_{12}^{(1)}(i, t)$ and $X_{1}^{(0)}(i, t), ..., X_{12}^{(0)}(i, t)$. In particular, mentioning the distributional setting and/or the observations under no notification.}
% \kc{probably not.}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figure/hs_mask_blues.pdf}
    \caption{\tbf{HeartSteps V1 data notification pattern.} The dark blue entries indicate that the app sent a notification to a sedentary participant---the entry has value $A_{i, t} = 1$. The white entries indicate that the participant was available but did not receive a notification or they were active immediately prior to the decision point. The light blue entries indicate the participant was unavailable. We assign the value $A_{i, t} = 0$ for all the white and light blue entries.}
    \label{fig:heart_missing}
\end{figure} 



\subsection{MovieLens}\label{app:movielens}
We load MovieLens via a custom \texttt{MovieLensDataLoader} that (i) downloads and caches the \texttt{ml‑1m.zip} archive, (ii) reads \texttt{ratings.dat} into a user $\times$ movie pivot table, and (iii) constructs the binary mask where observed entries correspond to rated user–movie pairs. The data matrix is $\measurement{} \in\{1,\dots,5\}^{6040\times3952}$ and mask matrix is $\missing{} \in\{0,1\}^{6040\times3952}$. The data can be downloaded from \url{https://grouplens.org/datasets/movielens/1m/}. See \url{https://files.grouplens.org/datasets/movielens/ml-1m-README.txt} for the usage license.

\subsection{Proposition 99}
\label{app:prop99}

\input{icml2025/prop99}

Data comes primarily from the Tax Burden on Tobacco compiled by Orzechowski and Walker~\cite{cdcBurdenTobacco} (ODC-By License). Using synthetic control methods, Abadie et al. construct a weighted combination of control states that closely resembles California's pre-1988 characteristics and cigarette consumption patterns. The optimal weights produce a synthetic California primarily composed of Colorado (0.164), Connecticut (0.069), Montana (0.199), Nevada (0.234), and Utah (0.334), with all other states receiving zero weight. The treatment effect is estimated as the difference between actual California per-capita cigarette sales and those of synthetic California after Proposition 99's implementation. By 2000, this analysis revealed that annual per-capita cigarette sales in California were approximately 26 packs lower than what they would have been without Proposition 99, representing about a 25\% reduction in cigarette consumption. To validate these findings, the authors conducted placebo tests by applying the same methodology to states not implementing tobacco control programs, confirming that California's reduction was unusually large and statistically significant (p = 0.026).

Proposition 99, the California Tobacco Tax and Health Protection Act of 1988, dataset spans from 1970 to 2000, providing 19 years of pre-intervention data before Proposition 99 was implemented in 1988 and 12 years of post-intervention data. It provides annual state-level cigarette consumption measured as per capita cigarette sales in packs based on tax revenue data. This data serves as a real data benchmark for many of the variants of synthetic controls~\cite{athey2021matrix}. We use the CDC dataset for the Nearest Neighbors methods and only use the target variable (i.e., cigarette consumption measured in packs per capita), and the dataset from SyntheticControlMethods library\footnote{\url{https://github.com/OscarEngelbrektson/SyntheticControlMethods/tree/master} (Apache-2.0 License)} for the SC baseline, since it relies on additional covariates.

\subsection{PromptEval}
\subsection{Efficient LLM evaluation: PromptEval}
\label{sub:llm}

% \begin{wrapfigure}{R}{0.5\textwidth}
%     \begin{center}
%     \includegraphics{figure/prompteval_est_errors_boxplot-p0.5.pdf}
%     \end{center}
%     \caption{\tbf{Kolmogorov-Smirnov distance with missingness at 50\%.} $\mmd$ using column-wise nearest neighbors performs the best in terms of the KS distance.}
%     \label{fig:ks}
% \end{wrapfigure}

The rapid advancement of LLMs have placed them at the center of many modern machine learning systems, from chatbots to aids in medical education \cite{geathers2025benchmarking}. In practice, system architects want to strike the right balance of real-world performance and cost, but navigating this Pareto frontier is a daunting task. 2024 alone saw at least 10 new models from Anthropic, Google, Meta, and OpenAI, not even counting the multitude of open-source fine-tuned models built on top of these.
% (Moreover, this number is likely to only grow as training models becomes more accessible, thanks in part to DeepSeek R1.) 
On specific tasks, smaller, fine-tuned models may even outperform the latest frontier models, in addition to being more cost effective.

We investigate how matrix completion, specifically nearest neighbor methods, can alleviate some of these burdens. We use the PromptEval dataset \cite{polo2024efficient}, which evaluates $15$ open-source language models (ranging in size from 3B to 70B parameters) and $100$ different prompting techniques across the 57 tasks of the MMLU benchmark \citep{hendrycks2020measuring}. In practice, the performance of a model depends---sometimes dramatically---on the precise input prompt. This suggests that we need to consider the performance of a model across a wide range of prompts, rather than any one prompt in particular. 
Thus, we model this problem as a distributional matrix completion problem with $N=15$, $T=57$, and $n=100$.
Given one of 57 tasks, we aim to accurately characterize the performance of each model without resorting to exhaustive evaluation.
Nearest neighbors leverage commonalities across models and tasks to estimate the performance distribution of each entry, which was otherwise not considered in \cite{polo2024efficient}; previous literature achieves efficient evaluation per model and task in isolation without leveraging any across model / task information. 

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.47\textwidth]{figure/ksbyp_prompteval_plot.pdf} & \includegraphics[width=0.45\textwidth]{figure/distributions-entry40-tp4.0.pdf} \\
        (a) Mean KS distance between estimated &
        (b) $\kernelnn$ vs. $\wassersteinnn$ \\
        and ground-truth distributions
    \end{tabular}
    \caption{\textbf{Distributional nearest neighbor methods enable efficient LLM evaluation on MMLU.} We estimate LLM score distributions across all models and tasks given only a limited number of model-task evaluations, determined by the propensity $p$. See \cref{sub:llm} for a detailed discussion.}
    \label{fig:llm}
\end{figure}

\paragraph{Results \& Discussion.}
We randomly include each entry in the matrix independently with probability $p\in \braces{0.3,0.5,0.7}$ and impute the missing entries using the $\kernelnn$ and $\wassersteinnn$ methods of \cref{tab:summary}. For each method, we consider both the the row-wise and column-wise variants.
\cref{fig:llm}(a) reports the mean Kolmogorov-Smirnov (KS) distance between the imputed and ground-truth distributions across the entries in the test set for varying missingness values. As expected, estimation error decreases as $p$ increases.
% the number of observed entries increases. 
% versus the ground truth at varying levels of $p$ for a select entry in the matrix. At $p=0.3$, we avoid 70\% of LLM evaluations, yet still recover the distribution of prompt scores with reasonable quality. At $p=0.5$ and $p=0.7$, column-wise NN with $\mmd$ performs the best.
\cref{fig:llm}(b) visualizes the imputed distributions using row-wise $\kernelnn$ and column-wise $\wassersteinnn$ (at $p=0.7$) for a select entry, along with the ground-truth distribution. Even with 30\% of matrix entries missing, distributional NN methods are able to recover the underlying distribution.

% MMLU is a multiple choice Q\&A benchmark with $57$ tasks, with a total of near $14$K examples\footnote{\url{https://github.com/felipemaiapolo/prompteval} (MIT License)}. $15$ different models, e.g., variants of Llama 3~\cite{llama3}, Mistral~\cite{jiang2023mistral} and Gemma~\cite{team2024gemma}. The examples are fed into the models with $100$ different varying prompting templates. The prompt templates are created by traversing between $3$ node modules, namely a \textit{separator}, a \textit{space} and an \textit{operator}~(see \cite{polo2024efficient} for details), from which $100$ unique prompt templates are created. The unitxt~\cite{bandel2024unitxt} preprocessing library is used to construct the dataset and evaluation is done by LM-Eval-Harness~\cite{eval-harness} library. The number of examples differ per task and each examples are evaluated on a model~(verifiable, so assigned $0$ or $1$ for correctness) by wrapping the examples with $100$ different prompt templates. 




% % \iffalse
% Fixing task $\tau \in \mathcal S$ and a model $m \in \mathcal M$, let $Y_{i, t} \in \{0, 1\}$ be the $\tau$ model score of question $q_t$ masked with the prompting template $p_i$. We drop dependence of $Y_{i, t}$ on $\tau, m$. \cite{polo2024efficient} assumes a model on $Y_{i, t}$
% \begin{align}
%     Y_{i, t} \stackrel{\mathrm{i.i.d.}}{\sim} \mathrm{Bernoulli} (\mu_{i, t}).
% \end{align}
% Propensity $\mu_{i, t}$ is parametrized via $\psi, \gamma$ in the following sense
% \begin{align}
%     \mu_{i, t} = \mathbb P(Y_{i, t} = 1; \psi, \gamma) = \sigma \big( f_\psi(x_i) - g_\gamma(z_t) \big)    
% \end{align}
% where $x_i, z_t$ are prompt, question specific covariates respectively. This is named the extended Raasch model.

% The ground truth~(estimand) here is the CDF of the averaged scores $Y_i = \frac{1}{T}\sum_{t = 1}^{T}Y_{i, t} \in [0, 1]$ across the prompt templates $p_i$. We only have access to a subset of binary observations $\mathcal E\subset [100] \times [T]$. $\hat\psi, \hat \gamma$ are obtained via entries $\mathcal E$ and model based imputation is implemented. 

% The modeling approach of \cite{polo2024efficient} has the advantage of incorporating covariate information, but the independence assumption and the fact that they simply use linear models $f_\psi, g_\gamma$ could make their attempt sub-optimal. We take a different approach, NN. But

% \begin{itemize}
%     \item NN does not output binary values
%     \item NN does not account for covariates. 
% \end{itemize}
% We could still make a comparison. While giving up on using covariate information, we assume a factor model and employ NN with majority voting, i.e. if $\tilde{Y}_{i, t}$ is the NN estimate, the final binary estimator is
% \begin{align}
%     \hat{Y}_{i, t} = \mathbf{1} ( \tilde{Y}_{i, t} \geq 1/2 ).    
% \end{align}
% Depending on which method works better (Raasch vs. NN) we can see if the assumptions necessary for \cite{polo2024efficient} is appropriate. If NN works better, than it implies that the factor structure is plausible, even more so as NN did not incorporate covariate information. 

% \fi


% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figure/est_errors_grid_barplot.pdf}
%     \caption{}
%     \label{fig:scalar_models}
% \end{figure}

% \subsubsection{How to do more}

% We can do more with Dist-MC framework --- we permute the dimensions and see if there is any meaningful insight. Here we consider a distributional MC framework with dimension template * task * model. So the idea is to approximate the distribution of the (example) averaged scores across different models. Per template and task, the performance variation across different models are estimated .


==> appendices_workshop/cv.tex <==
\section{Cross-Validation}\label{app:cv}

For each nearest neighbor method, we use cross-validation to optimize hyperparameters including distance thresholds and weights, depending on which nearest neighbor algorithm is chosen. Specifically, for each experiment, we choose a subset of the training test to optimize hyperparameters by masking those matrix cells and then estimating the masked values. We utilize the HyperOpt library \cite{bergstra2013making} to optimize (possibly multiple) hyperparamters using the Tree of Parzen Estimator \cite{bergstra2011algorithms}, a Bayesian optimization method. Our package supports both regular distance thresholds and percentile-based thresholds, which adapt to the distances calculated within the specific dataset.

==> appendices_workshop/guarantees.tex <==
\section{Structural assumptions}
\label{app:guarantees}

Provable guarantees of nearest neighbors in matrix settings \cref{eq:model} can be shown when structural assumptions are imposed on the distributions $\dist{i, t}$ and the missingness $\missing{i, t}$. We collect existing results from \cite{li2019nearest,dwivedi2022doubly,choi2024learning,feitelberg2024distributional,sadhukhan2024adaptivity,sadhukhan2025adaptivelyweightednearestneighborsmatrix}. Given data with missing observations from \cref{eq:model}, the practitioner is interested in learning information of the distributions, e.g., mean of the distributions $\sbraces{ \meanparam{i, t} = \int x d\dist{i, t}(x)}.$

% When $\missing{i, t} = 0$, we have no accessible information from $\dist{i, t}$, and when $A_{i, t} = 1$, we do not have access to the exact distribution $\mu_{i, t}$ rather only a single measurement from $\dist{i, t}$ are available. 


% For provable guarantees of the MC algorithms, structural assumptions on the model \cref{eq:model} are in order. 

The first assumption specifies the factor structure on the mean; that is, there exists latent factors $u_i, v_t$ that collectively characterize the signal of each entry $(i, t)$ of the matrix~\cite{li2019nearest,dwivedi2022counterfactual,agarwal2023causal,choi2024learning,feitelberg2024distributional}. Such a factor model is analogous to the low rank assumptions commonly imposed in matrix completion~\cite{candes2012exact}. The second assumption specifies how the missing pattern $\missing{i, t}$ was generated; for instance missing completely at random~(MCAR) assumes that $\missing{i, t}$ are independent to all other randomness present in the model \cref{eq:model} and that all entries have positive probability of being observed.

% \footnote{$\propensity{i, t} := \Prob(\missing{i, t} = 1) > 0$ for all $i, t$.}.



\subsection{Factor model}

For the scalar matrix completion problem, i.e., \cref{eq:model} with $n = 1$, the main goal is to learn~(or impute) the mean of the underlying distribution $\theta_{i, t}$ for any missing entries~\cite{li2019nearest,dwivedi2022doubly,dwivedi2022counterfactual,agarwal2023causal,sadhukhan2024adaptivity, sadhukhan2025adaptivelyweightednearestneighborsmatrix}. The majority of this literature assumes (i) an additive noise model $\dist{i, t} = \theta_{i, t} + \varepsilon_{i, t}$ for centered i.i.d. sub-Gaussian noise $\varepsilon$ and (ii) mean factor model, i.e., $\theta_{i, t} = f(u_i, v_t)$ for some latent factors $u_i, v_t$ and real valued function $f$. 

For the distributional matrix completion problem (i.e., \cref{eq:model} with $n > 1$) the main goal is to learn the underlying distribution itself~\cite{choi2024learning,feitelberg2024distributional}; a factor model is imposed on the distribution as a whole. For instance, a factor model is assumed on the kernel mean embedding of distributions; that is, there exist latent factors $u_i$ and $v_t$ and an operator $g$ such that $\int \kernel(x, \cdot)d\dist{i, t}(x) = g(u_i, v_t)$.


\subsection{Missingness pattern}
\label{app:missingness}

For both the scalar and distributional matrix completion problem \cref{eq:model}, the missing pattern~(i.e., how the missingness $\missing{j, s}$ was generated) can be categorized into three classes using the taxonomy of \cite{little2019statistical}: missing-completely-at-random~(MCAR), missing-at-random~(MAR) and missing-not-at-random~(MNAR). MCAR assumes that the missingness $\missing{i, t}$ is exogenous~(independently generated from all the randomness in the model) and i.i.d. with propensity $\Prob(\missing{i, t} = 1) = p > 0$ for all $(i, t)$. MAR is a more challenging scenario compared to MCAR as missingness is not exogenous, but its randomness depends on the observations. Further, propensities $p_{i, t}$ may differ for entries $(i, t)$ but positivity still holds, i.e., $\min_{i \in [N], t \in [T]}p_{i, t} > 0$. An important instance for MAR is the adaptive randomized policies~\cite{dwivedi2022personalization}. The MNAR setup is the most challenging as it assumes the missingness depends on the unobserved latent confounders, while positivity may also be violated, i.e., $\min_{i \in [N], t \in [T]}p_{i,t } = 0$. The staggered adoption pattern, where a unit remains treated once a unit is treated at some adoption time, is a popular example of MNAR, mainly because positivity is violated. See \cite{athey2021matrix,athey2022design} for more details on staggered adoption.

We briefly outline the structural assumptions existing nearest neighbor methods were shown to work with provable guarantees; for all the existing methods, factor models~(with slightly different details; compare the mean factorization~\cite{li2019nearest} and the distribution factorization~\cite{choi2024learning,feitelberg2024distributional}) are all commonly assumed.
\begin{itemize}
    \item (Scalar matrix completion) The vanilla versions of nearest neighbors~($\rownn$) in \cite{li2019nearest,dwivedi2022counterfactual} are shown to work for MCAR and MAR setup; the latter shows that simple nearest neighbors can provably impute the mean when the missingness is fully adaptive across all users and history. The variants of vanilla nearest neighbors $\drnn$~\cite{dwivedi2022doubly} is proven to work under MCAR, while $\tsnn$~\cite{sadhukhan2024adaptivity} is proven to work under unobserved confounding, i.e., MNAR. 
    \item (Distributional matrix completion) The $\kernelnn$~\cite{choi2024learning} is shown to recover the underlying distribution under MNAR, whereas $\wassersteinnn$~\cite{feitelberg2024distributional} is shown to work under MCAR. 
\end{itemize}


% \cite{li2019nearest} considers the same setting, with MCAR. 

% \cite{feitelberg2024distributional} considers MCAR in the distributional setup.

% \cite{dwivedi2022counterfactual} considers an arbitrarily adaptive design

% \cite{agarwal2023causal} considers a confounded factor model, while the positivity can be violated(?). 

% \cite{choi2024learning} considers a confounded missingness, where the positivity can be violated. 

% \cite{sadhukhan2024adaptivity} considers a confounded missingness, where the positivity can be violated. 

% \cite{sadhukhan2025adaptivelyweightednearestneighborsmatrix} considers a confounded missingness, where the positivity can be violated. 



==> appendices_workshop/library.tex <==
\section{\lib{} Package and Interface}\label{sec:library}

We now present our unified Python package, \lib{}, for nearest neighbor algorithms for matrix completion. In particular, we provide a class structure which abstracts the estimation procedure utilized in each different nearest neighbor method as well as the the $\distancemod$ and $\averagemod$ modules described above in \cref{sec:nn-overview}. On top of that, our library facilitates easy extensions to other nearest neighbors algorithms and other data types on top of scalars and distributions. For example, as long as a distance and average notion are well defined, our library can be easily applied to a matrix of images or text strings.

\paragraph{Class structure.} The core functionality of \lib{} is based on two abstract classes: \texttt{EstimationMethod} and \texttt{DataType}.

\texttt{EstimationMethod} classes contain the logic to impute a missing entry such as how to use calculated distances. 
% In the context of the modules in \cref{sec:nn-overview}, this class determines the weighting function or, in the context of $\drnn$ and $\autonn$, how to compose estimates. 
We separate this from the \texttt{DataType} abstraction because several estimation methods can be used for multiple data types. For example, \texttt{RowRowEstimator} implements the $\rownn$ procedure for any data type given to it, such as scalars or distributions.

% \texttt{DataType} classes implement the $\distancemod$ and $\averagemod$ modules for any kind of data type (e.g. scalars which use squared distance and simple averaging). 
\texttt{DataType} classes implement a \emph{distance} and \emph{average} function for any kind of data type. For scalars we use squared distance and simple averaging. For distributions, we implement two metrics, Wasserstein ($\wassersteinnn$) and kernel maximum mean discrepancy (MMD, $\kernelnn$). This abstract class allows for our package to extend to any data types beyond the ones we tested. For instance, a practitioner can easily add a \texttt{DataType} for text strings which uses vector embeddings to find distances and averages between between strings without needing to rewrite any of the estimation procedure.

\paragraph{Interface.} To use our library, a user simply has to instantiate a composite class \texttt{NearestNeighborImputer} with their \texttt{EstimationMethod} and \texttt{DataType} of choice. We provide constructor functions to automatically create popular \texttt{NearestNeighborImputer} classes such as a two-sided nearest neighbor estimator with the scalar data type. From a design pattern point of view, this is known as a \emph{Composite} design pattern \citep[pg. 163]{gamma1993design}. We use this design pattern so that anyone looking to customize the estimation procedure can do so for any kind of data type simultaneously. Similarly, with the exception of doubly robust estimators, each estimation procedure works out of the box with any data type that implements the \texttt{DataType} abstract class. The Doubly robust estimation method does not work out of the box with distributions because a subtraction operation is not well defined in the distribution space.

Finally, the user simply needs to input (i) a data matrix, (ii) a mask matrix which specifies which values are missing, and (iii) the row and column to impute. Thus, a user can test out different estimation procedures by changing just one line of code. Separately from the core functionality, we have also implemented several cross-validation classes which take in a \texttt{NearestNeighborImputer} class and find the best hyperparameters to use (e.g., distance thresholds and weights).

% NN 2 pages

% Star NN, Auto NN at most 1 page.

% library
% 1~1.5page

% case
% 3pages

==> appendices_workshop/nn-algo.tex <==
\section{Nearest neighbor algorithms}\label{app:nn-algo}

\subsection{Unified framework}\label{sec:unified-view}
We introduce two general modules~(namely $\distancemod$ and $\averagemod$) from which the variants of nearest neighbors are constructed. We introduce several shorthands used in the modules. Denote the collection of measurements, missingness, and weights:
\begin{align}
    \mc Z:=\big\{\measurement{j, s}\big\}_{j \in [N] , s \in [T]} , \quad  \mc A := \sbraces{\missing{j, s}}_{j \in [N], s \in [T]},\\ \qtext{and} \mc W := \sbraces{w_{j, s}}_{j \in [N],s \in [T]}.
\end{align} 
Let $\entrydist{x, x'}$ be a metric between $x, x' \in \mc X$ for some space $\mc X$. Further define $\entrydistest{\measurement{i, t}, \measurement{j, s}}$ as a data-dependent distance between any two observed entries $(i, t)$ and $(j, s)$ of the matrix \cref{eq:model}. The two modules can now be defined: 
\begin{itemize}
    \item[(i)] $\distancemod (\what{\varphi}, \mc Z, \mc A)$: Additional input is the data-dependent distance between entries of matrix $\what{\varphi}$ and output is the collection of row-wise and column-wise distance of matrix:
    \begin{align}\label{mod:distance}
        \distance{i, j}^{\row} &:= \frac{\sum_{s \neq t}\missing{i, s}\missing{j, s}\entrydistest{\measurement{i, s}, \measurement{j, s}}}{\sum_{s \neq t} \missing{i, s}\missing{j, s}} \qtext{and}\\ \distance{t, s}^{\col} &:= \frac{\sum_{j \neq i}\missing{j, t}\missing{j, s}\entrydistest{\measurement{j, t}, \measurement{j, s}}}{\sum_{j \neq i} \missing{j, t}\missing{j, s}},
    \end{align}
    \item[(ii)] $\averagemod (\varphi, \mc W, \mc Z, \mc A)$: Additional input are the weights $\mc W$, metric $\varphi$ and output is the optimizer
        \begin{align}\label{eq:ave-output}
           \what{\theta} = \argmin_{x \in \mc X}\sum_{j \in [N], s \in [T]} \weight{j, s}\missing{j, s}\entrydist{x, \measurement{j, s}}.
        \end{align}
        \iffalse
    \item[(iii)] \composemod($\what \theta_1$, $\what \theta_2$): For any two optimizers \cref{eq:ave-output} as input, the output is $f(\what \theta_1, \what \theta_2)$ for some function $f$.
    \fi
    % \begin{itemize}
    %     \item[$\mbf{subMod}2$] ($\weightmod$) 
    %     \item[$\mbf{subMod}1$] ($\neighbormod$) 
    % \end{itemize} 
    % \item[$\mbf{Mod}3$] $\subtractmod()$ Taking the difference of averages attained in module $\averagemod$.
\end{itemize}
% \begin{remark}
%     The two modules $\distancemod$ and $\averagemod$ are implicitly coupled via the weights $\weight{}$ in $\averagemod.$ For instance, a binary weight defined via the module $\distancemod$ and tuning parameters $\tuning$
%         \begin{align}\label{eq:std-weight}
%             \weight{j, s} = \indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}.
%         \end{align}
%     recovers $\rownn, \distnn, \tsnn, \drnn$. Otherwise, a non-binary weight $\weight{}$ recovers $\awnn$~\kc{@MP, TS: Fill up details.}
% \end{remark}
The $\distancemod$ module calculates the row-wise and column-wise distance of the matrix, by taking the average of the observed entry-wise distance $\entrydistest{\cdot, \cdot}$. The $\averagemod$ module calculates the weighted average of observed measurements, where the notion of average depends on the metric $\varphi$ and the space $\mc X$ on which the metric $\varphi$ is defined. 
\iffalse
If $\mc X = \real$ and $\varphi(x, x') = (x - x')^2$, then the average is simply weighted sample mean of observed entries. If $\mc X$ is the space of all square integrable probability measures on the real line, then the average is the barycenter of probability measures; see \cite{muandet2017kernel,bigot2017geodesic} and \cref{app:guarantees} for a comparison on the $\mmd$ and $\wasserstein$ barycenters. 
\fi
Notably, the weights $\mc W$ in the $\averagemod$ module encodes the entry information of the estimand. 

\begin{remark}\label{rem:row-nn}
The vanilla row-wise nearest neighbors~\cite{li2019nearest} that targets the mean $\theta_{i, t} = \int x d\dist{i, t}(x)$ of entry $(i, t)$ is recovered by first applying $\distancemod$ with $\entrydistest{\measurement{j, s}, \measurement{j', s'}} = {(\measurement{j, s} - \measurement{j', s'})^2}$, applying $\averagemod$ with the non-smooth weight
${\weight{j, s} = \indic{\distance{i,j}^\row \leq \tuning_1}\cdot \indic{\distance{s, t}^\col \leq 0}}$, and using the metric $\entrydist{x, y} = (x - y)^2$. Note that the non-smooth weight satisfies $\weight{j, t} = \indic{\distance{i, j}^\row \leq \tuning_1}$, whereas $\weight{j, s} = 0$ for $s \neq t$; by defining the nearest neighbor set $\mbf N_{t, \tuning_1} := \{ j \in [N] : \distance{j, t}^\row \leq \tuning_1 \}$, the $\averagemod$ module output can be rewritten as $\argmin_{x \in \real} \sum_{j \in \mbf N_{t, \tuning_1}} \missing{j, t}(x - \measurement{j, t})^2 = |\mbf N_{t, \tuning_1}|^{-1}\sum_{j \in \mbf N_{t, \tuning_1}}\measurement{j, t}$.
\end{remark}

\subsection{Existing methods}
\label{subsec: existing methods}
We present existing variants of nearest neighbors using the two modules introduced \cref{sec:unified-view}; all the methods presented here are recovered by sequentially applying $\distancemod$ and $\averagemod$ with the appropriate specification of $\what \varphi$, $\varphi$ and $\mc W$. 

For simple notation, we introduce a shorthand for the non-continuous weight
\begin{align}
    \weight{j, s}^{(i, t)}(\tuning_1, \tuning_2) := \indic{\distance{i,j}^\row \leq \tuning_1}\cdot \indic{\distance{s, t}^\col \leq \tuning_2}.
\end{align}

All methods except $\awnn$ and our newly proposed $\autonn$, have binary weights i.e., $w_{j,s}\in\sbraces{0,1}$. $\autonn$, detailed in \cref{sec:new-nn}, uses weights to carefully pool together the benefits of $\tsnn$ and $\drnn$. $\awnn$~\cite{sadhukhan2025adaptivelyweightednearestneighborsmatrix} improves upon $\rownn$  by adaptively choosing the weights which optimally balances the bias-variance tradeoff of $\rownn$ as follows % For notational convenience, we define a vector
\begin{align}\label{eq:star-nn-weight}
  &\big(\weight{1}^\star(i, t), ..., \weight{N}^\star(i, t)\big):= \\ &\argmin_{(v_{1}, ..., v_{N})\in \Delta_N} 2\log(2N)\widehat \sigma^2 \sum_{k \in [N]}v_{k}^2 + \sum_{k \in [N]}v_{k} A_{k,t}\distance{i,k}^\row.
\end{align}
where $\widehat \sigma^2$ is the estimated error and $\Delta_N$ is a simplex in $\real^N$; see \cite{sadhukhan2025adaptivelyweightednearestneighborsmatrix} for details of \cref{eq:star-nn-weight}. \cref{tab:summary} contains a concise summary of the existing nearest neighbor variants; see \cref{app:nn-algo} for a detailed exposition for each methods.


\iffalse
We also define the following weight function,
\begin{align}
    \widetilde {\weight{j, s}}^{(i, t)}:= \widetilde{\weight{j}}^{(i, t)} \cdot \indic{\distance{s, t}^\col \leq 0},
\end{align}
where the vector $\widetilde{\weight{}}^{(i, t)} = (\widetilde{\weight{1}}^{(i, t)}, \cdots, \widetilde{\weight{n}}^{(i, t)})$ is defined as,
 \begin{align}
  \widetilde{\weight{}}^{(i, t)}  := \mbox{arg min}_{\weight{}^{(i, t)}} \Big[2\log(2m)\widehat \sigma^2\|\weight{}^{(i, t)}\|_2^2 + \sum_{j =1 }^m  \weight{j}^{(i, t)} A_{j,t}\distance{i,j}^\row  \Big].
\end{align}
In the above optimization, $\weight{}^{(i, t)}$ is used to denote a candidate non-negative weight vector, the sum of whose elements is $1$. The estimate of error variance $\widehat \sigma^2$ is computed from $\mc Z$. 
\fi

\setlength\cellspacetoplimit{5pt}
\setlength\cellspacebottomlimit{5pt}

\begin{table}[H]
  \caption{\label{tab:summary}\textbf{Variants of nearest neighbors for matrix completion.}}
  \centering
  \begin{tabular}{clccc}
    \toprule
    \tbf{Type}
    &\tbf{Method} 
    & ${\what\varphi}(x, y)$ 
    & \def\arraystretch{1.2}\begin{tabular}{c} $\varphi(x, y)$
    \end{tabular} 
    & $\weight{j, s}$
    \\
    \midrule
   $n = 1$ &
    $\rownn$ \ \citep{li2019nearest} (\cref{algo:vanilla-nn}) & $(x - y)^2$
    & $(x - y)^2$
    & $\indic{\distance{i, j}^\row\leq \tuning_1, \distance{s, t}^\col \leq 0}$
    \\ 
    % \midrule
    &
    $\colnn$ \ \citep{li2019nearest} (\cref{algo:vanilla-nn}) & $(x - y)^2$
    & $(x - y)^2$
    & $\indic{\distance{i, j}^\row\leq 0, \distance{s, t}^\col \leq \tuning_2}$
    \\
    &
    $\tsnn$ \ \citep{sadhukhan2024adaptivity} \textup{(\cref{algo:tsnn})}
     & $(x - y)^2$
     & $(x - y)^2$ 
    & $\indic{\distance{i, j}^\row\leq \tuning_1, \distance{s, t}^\col \leq \tuning_2}$
    \\ 
    % \midrule
    % \midrule
    &
    $\awnn$ \ \citep{sadhukhan2025adaptivelyweightednearestneighborsmatrix} \textup{(\cref{algo:awnn})}
    & $(x - y)^2$
    & $(x - y)^2$ 
    & $\weight{j}^\star(i, t)\cdot\indic{\distance{s, t}^\col \leq 0}$
    \\
    \noalign{\vspace{5pt}}
    \cline{2-5}
    \noalign{\vspace{5pt}}
    &
    $\drnn$ \ \citep{dwivedi2022doubly} {(\cref{algo:dsnn})}
     & \multicolumn{3}{c}{$\rownn + \colnn - \tsnn$} 
    \\
    &
    $\autonn$ \ (\cref{sec:new-nn})
     & \multicolumn{3}{c}{$\alpha \cdot \drnn + (1 - \alpha) \cdot \tsnn$} 
    \\
     \midrule
$n > 1$     &
    $\kernelnn$ \ \citep{choi2024learning} (\cref{algo:vanilla-dnn}) & $\what \mmd_\kernel^2(x, y)$
    & $\mmd_\kernel^2(x, y)$
    & $\indic{\distance{i, j}^\row\leq \tuning_1, \distance{s, t}^\col \leq 0}$
    \\
    % \midrule
    &
    $\wassersteinnn$ \ \citep{feitelberg2024distributional} (\cref{algo:vanilla-dnn}) & $\hatwasserstein^2(x, y)$
    & $\wasserstein^2(x, y)$
    & $\indic{\distance{i, j}^\row\leq \tuning_1, \distance{s, t}^\col \leq 0}$
    \\ \bottomrule
  \end{tabular}
\end{table}

Under the distributional matrix completion setting~($n > 1$ in \cref{eq:model}), the methods $\kernelnn$ and $\wassersteinnn$ in \cref{tab:summary} take $\mu, \nu \in \mc X$ as square integrable probability measures, and $\entrydist{\mu, \nu}$ as either the squared maximum mean discrepency~(i.e. $\mmd_\kernel^2(\mu, \nu)$, see \cite{muandet2017kernel}) or squared Wasserstein metric~(i.e., $\wasserstein(\mu, \nu)$, see \cite{bigot2020}).
Further, the entry-wise distance $\entrydistest{x, y}$ in this case is either the unbiased U-statistics estimator $\what{\mmd}_\kernel^2(\measurement{i, t}, \measurement{j, s})$ for $\mmd_\kernel^2(\dist{i, t}, \dist{j, s})$~(see \cite{muandet2017kernel}) or the quantile based estimator $\hatwasserstein(\measurement{i, t}, \measurement{j, s})$ for $\wasserstein(\dist{i, t}, \dist{j, s})$~(see \cite{bigot2020}).

The nearest neighbor methods introduced in \cref{tab:summary} are elaborated in this section. We present two versions of each method; the first version explicitly constructs neighborhoods instead of subtly embedding them in the weights $\mc W$ of the $\averagemod$ module, and the second version specifies how each methods can be recovered by applying the two modules, $\distancemod$ and $\averagemod$, sequentially.


% Nearest neighbors is a local and non-parametric imputation technique that is shown to successfully estimate the means $\Theta$ when MCAR assumption is violated. \cite{dwivedi2022counterfactual,agarwal2023causal,choi2024learning}.
% \jf{Should we just explain a basic row-wise nearest neighbor algorithm instead of trying to generalize all the notation? I think that it is easy for us to explain in non-math terms how the notions of distance and averaging are different between the methods, but otherwise it's the same.} \kc{DRNN and TSNN would require a bit more of a general notation I think}
% \jf{Ya I think that doing the general notation makes it difficult to understand though and once the reader understands a simpler nearest neighbor algorithm, then we can explain the more complicated ones.} \kc{good point}

% \paragraph{Row-wise nearest neighbor algorithm} 

% Then the measurements within the neighbor $\neighbor{1, 1, \tuning}$ are processed~(a form of averaging) to output a single estimate.

\subsection{Vanilla nearest neighbors}

We elaborate on the discussion in \cref{rem:row-nn} and provide here a detailed algorithm based on the explicit construction of neighborhoods, which is essentially equivalent to $\rownn$ in \cref{tab:summary}. The inputs are measurements $\mc Z$, missingness $\mc A$, the target index $(i, t)$, and the radius $\tuning$.
\begin{itemize}
    \item[\textbf{Step 1:}] (Distance between rows) Calculate the distance between row $i$ and any row $j \in [N] \setminus \{i\}$ by averaging the squared Euclidean distance across overlapping columns:
    \begin{align}\label{eq:snn-distance}
        \distance{i, j} := \frac{\sum_{s \neq t}\missing{i, s}\missing{j, s}(\measurement{i, s} - \measurement{j, s})^2}{\sum_{s \neq t} \missing{i, s}\missing{j, s}}.
    \end{align}
    \item[\textbf{Step 2:}] (Construct neighborhood) Construct a neighborhood of radius $\tuning$ within the $t$th column using the distances $\{\distance{i, j}:j \neq i\}$: 
    \begin{align}
        \neighbors{t, \tuning} := \big\{ j \in [N] \setminus \{i\} : \distance{i, j} \leq \tuning \big\}
    \end{align}
    \item[\textbf{Step 3:}] (Average across observed neighbors) Take the average of measurements within the neighborhood:
    % For row-wise neighbors $\sbraces{ j \neq i : \varrho_{i, j} \leq \eta}$ within $\eta$ radius, average across observed neighbors within $t$th column,
    \begin{align}\label{eq:snn-average}
        \what{\theta}_{i, t, \eta} := \frac{1}{|\neighbors{t, \tuning}|}\sum_{j \in \neighbors{t,\tuning}}\missing{j, t}\measurement{j, t}.
    \end{align}
\end{itemize}
In practice, the input $\tuning$ for $\rownn$ should be optimized via cross-validation; we refer the reader to \cref{app:cv} for a detailed implementation.

We specify the exact implementation of the two modules $\distancemod$, $\averagemod$ to recover $\rownn$:
\begin{algorithm2e}[H]
\caption{$\rownn$ for scalar nearest neighbor} 
  \label{algo:vanilla-nn}
  \SetAlgoLined
  \DontPrintSemicolon
  \small
  {
\KwIn{\textup{$\mc Z, \mc A, \tuning,$ $(i, t)$}}
  \BlankLine
    Initialize entry-wise metric $\entrydistest{\measurement{j, s}, \measurement{j', s'}}\gets ( \measurement{j, s} - \measurement{j', s'} )^2$ and metric $\entrydist{x, y} \gets (x - y)^2$\\
    Initialize hyper-parameter ${\tuning} \gets (\tuning_1, 0)$\\
    Calculate row-wise metric $\big\{ \distance{i, j}^\row: j \neq i \big\} \gets $ $\distancemod(\what{\varphi}, \mc Z, \mc A)$ \\
    Initialize weight $\weight{j, s} \gets  \indic{\distance{i, j}^\row \leq \tuning_1, \distance{s, t}^\col \leq \tuning_2}$ \\
    Calculate average $\what \theta_{i, t} \gets \averagemod(\varphi, \mc W, \measurement{}, \missing{})$
    \BlankLine
\KwRet{$\what \theta_{i, t}$}
}
\end{algorithm2e} 
The discussion for $\rownn$ here can be identically made for $\colnn$ as well.


\subsection{Two-sided and doubly-robust nearest neighbors}

% A natural extension of the vanilla version of nearest neighbors introduced so far is to combine the row-wise and column-wise $\nn$. Different ways of combining the two vanilla $\nn$ were proposed in \cite{dwivedi2022doubly} and \cite{sadhukhan2024adaptivity}, each method coined doubly-robust nearest neighbors~(in short $\drnn$) and two-sided nearest neighbors~(in short $\tsnn$) respectively. The design of both $\drnn$ and $\tsnn$ are motivated by the underlying factor structure~(see \cref{app:guarantees}) of the matrix; $\tsnn$ averages the neighbors both across the $\row$s and $\col$s whereas $\drnn$ debiases the naive combination of $\rownn$ and $\colnn$, achieving superior results compared to the individual vanilla $\nn$s.

We elaborate on the variants of the vanilla nearest neighbors algorithm $\tsnn$ and $\drnn$ in \cref{tab:summary}; we first elaborate on an equivalent version of each of the methods which explicitly constructs neighborhoods.

In the following three step procedure, $\drnn$ and $\tsnn$ differs in the last averaging step: the inputs are the measurements $\mc Z$, missingness $\mc A$, the target index $(i, t)$, and the radii $\tuning = (\tuning_1, \tuning_2)$.
\begin{itemize}
    \item[\textbf{Step 1:}] (Distance between rows) Calculate the distance between row $i$ and any row $j \in [N] \setminus \{i\}$ and the distance between column $t$ and any column $s \in [T] \setminus \{t\}$:
    \begin{align}\label{eq:snn-distance}
        \distance{i, j}^{\row} := \frac{\sum_{s \neq t}\missing{i, s}\missing{j, s}(\measurement{i, s} - \measurement{j, s})^2}{\sum_{s \neq t} \missing{i, s}\missing{j, s}} \qtext{and} \distance{t, s}^{\col} := \frac{\sum_{j \neq i}\missing{j, t}\missing{j, s}(\measurement{j, t} - \measurement{j, s})^2}{\sum_{j \neq i} \missing{j, t}\missing{j, s}}
    \end{align}
    \item[\textbf{Step 2:}] (Construct neighborhood) Construct a row-wise and column-wise neighborhood of radius $\tuning_1$ and $\tuning_2$ respectively,
    % within the $t$th column using the distances $\{\distance{i, j}:j \neq i\}$: 
    \begin{align}
        \neighbors{t, \tuning_1}^\row := \big\{ j \in [N] \setminus \{i\} : \distance{i, j}^\row \leq \tuning \big\} \qtext{and} \neighbors{i, \tuning_2}^\col := \big\{ s \in [T] \setminus \{t\} : \distance{t, s}^\col \leq \tuning \big\}
    \end{align}
    \item[\textbf{Step 3:}] (Average across observed neighbors) Take the average of measurements within the neighborhood; the first and the second averaging correspond to $\drnn$ and $\tsnn$ respectively:
    % For row-wise neighbors $\sbraces{ j \neq i : \varrho_{i, j} \leq \eta}$ within $\eta$ radius, average across observed neighbors within $t$th column,
    \begin{align}\label{eq:drnn-tsnn-average}
        &\what{\theta}_{i, t, \eta}^{\mathsf{DR}} := \frac{\sum_{j \in \neighbors{t,\tuning_1}^\row, s \in \neighbors{i, \tuning_2}^\col}\missing{j, t}\missing{i, s}\missing{j, s}\big(\measurement{j, t} + \measurement{i, s} - \measurement{j, s}\big) }{\sum_{j \in \neighbors{t,\tuning_1}^\row, s \in \neighbors{i, \tuning_2}^\col}\missing{j, t}\missing{i, s}\missing{j, s}}\qtext{and} \\
        &\what{\theta}_{i, t, \eta}^{\mathsf{TS}} := \frac{\sum_{j \in \neighbors{t,\tuning_1}^\row, s \in \neighbors{i, \tuning_2}^\col}\missing{j, s}\measurement{j, s}}{\sum_{j \in \neighbors{t,\tuning_1}^\row, s \in \neighbors{i, \tuning_2}^\col}\missing{j, s}}.
        % \sum_{j \in \neighbors{t,\tuning}}\missing{j, t}\measurement{j, t}
    \end{align}
\end{itemize}

Next, we specity the exact implemention of the two modules $\distancemod$ and $\averagemod$ to recover $\tsnn$ and $\drnn$:

\begin{algorithm2e}[H]
\caption{$\tsnn$ for scalar matrix completion} 
  \label{algo:tsnn}
  \SetAlgoLined
  \DontPrintSemicolon
  \small
  {
\KwIn{\textup{$\mc Z, \mc A, \tuning,$ $(i, t)$}}
  \BlankLine
    Initialize entry-wise metric $\entrydistest{\measurement{j, s}, \measurement{j', s'}}\gets ( \measurement{j, s} - \measurement{j', s'} )^2$ and metric $\entrydist{x, y} \gets (x - y)^2$\\
    Initialize tuning parameter ${\tuning} \gets (\tuning_1, \tuning_2)$\\
    Calculate row-wise and column-wise metric $\big\{ \distance{i, j}^\row: j \neq i \big\}, \big\{ \distance{t, s}^\col: s \neq t \big\} \gets $ $\distancemod(\what \varphi, \measurement{}, \missing{})$ \\
    Initialize weight $\weight{j, s} \gets  \indic{\distance{i, j}^\row \leq \tuning_1, \distance{s, t}^\col \leq \tuning_2}$ \\
    Calculate average $\what \theta_{i, t} \gets \averagemod(\varphi, \mc W, \mc Z, \mc A)$
    \BlankLine
\KwRet{$\what \theta_{i, t}$}
}
\end{algorithm2e} 

For $\drnn$ algorithm below, we consider $\mc Z$ and $\mc A$ to be $N\times T$ sized matrices, so that their transpose is well defined. Then note that $\colnn$ is simply applying \cref{algo:vanilla-nn} with transposed observation matrices. 
\begin{algorithm2e}[H]
\caption{$\drnn$ for scalar matrix completion} 
  \label{algo:dsnn}
  \SetAlgoLined
  \DontPrintSemicolon
  \small
  {
\KwIn{\textup{$\mc Z, \mc A, \tuning,$ $(i, t)$}}
  \BlankLine
    Initialize $\rownn \gets$ \cref{algo:vanilla-nn} with inputs $(\mc Z, \mc A, \tuning, (i, t))$ and $\tuning \gets (\tuning_1, 0)$ \\
    Initialize $\colnn \gets$ \cref{algo:vanilla-nn} with input $(\mc Z^T, \mc A^T, \tuning, (i, t))$ and $\tuning \gets (\tuning_1, 0)$\\
    Initialize $\tsnn \gets$ \cref{algo:tsnn} with inputs $(\mc Z, \mc A, \tuning, (i, t))$ and ${\tuning} \gets (\tuning_1, \tuning_2)$ \\
    Calculate $\what \theta_{i, t} \gets \rownn + \colnn-\tsnn$
    \BlankLine
\KwRet{$\what \theta_{i, t}$}
}
\end{algorithm2e} 

% \begin{remark}[$\drnn$ and $\tsnn$]
%     \kc{One of the crucial difference between the two is in the number of samples that are averaged upon. }
%     \kc{Although both methods were defined for the same $\tuning$~(for convenience), note that the radii are chosen differently for the two methods in CV}\kc{Each methods perform optimally at different environments~(@CC empirical by differing SNR)---a need for adaptive procedure.}
% \end{remark}



\subsection{Distributional nearest neighbors}

% In \cite{choi2024learning,feitelberg2024distributional}, a generalization of matrix completion framework \cref{eq:model} is proposed, namely the distributional matrix completion model. Each entries of the matrix are assigned multiple measurements that are sampled from a distribution unique per entry:
% \begin{align}
% \qtext{for} i \in [N], t\in[T]:\quad Z_{i, t} :=
%      \begin{cases}
%         X_{1}(i, t), \ldots, X_{n}(i, t) \ \sim \ \mu_{i, t}&\qtext{if} A_{i, t}=1, \\
%         \mrm{unknown}&\qtext{if} A_{i, t}=0.
%     \end{cases}
%     \label{eq:model-dist}
% \end{align}
% Given this data with missing observations, the practitioner is interested in estimating the whole collection of distributions $\sbraces{\dist{i, t}}_{(i, t) \in [N]\times [T]}$. When $\missing{i, t} = 0$, we have no accessible information from $\dist{i, t}$, and when $\missing{i, t} = 1$, we do not have access to the exact distribution $\dist{i, t}$, rather only $n$ measurements from $\dist{i, t}$ are available. See \cref{app:guarantees} for more details on how factor structure is imposed on distributions.

% Unlike the mean factor models~\cite{dwivedi2022doubly}, factor structure is imposed on the distributional level. For \cite{choi2024learning}, factor model is imposed on the kernel mean embeddings of the distributions. 

Unlike the scalar nearest neighbor methods, distributional nearest neighbors necessitate a distributional notion of distance between rows and columns of matrix and a distributional analog of averaging. \cite{choi2024learning} and \cite{feitelberg2024distributional} use maximum mean discrepency~(in short $\mmd$) of kernel mean embeddings~\cite{muandet2017kernel} and Wasserstein metric~(in short $\wasserstein$)~\cite{bigot2020} respectively both for defining the distance between rows / columns and for averaging. The corresponding barycenters of $\mmd$ and $\wasserstein$~\cite{cohen2020estimating,bigot2017geodesic} are used for averaging, and so the methods are coined kernel nearest neighbors~(in short $\kernelnn$) and 
Wasserstein nearest neighbors~(in short $\wassersteinnn$) respectively.

\iffalse


Here we provide the vanilla version~(row-wise) of distributional nearest neighbors. The extension of vanilla distributional nearest neighbors to the two-sided and doubly-robust version is of future interest. For a simple exposition, we set $\varrho(\mu, \nu)$ to be a metric between any two distributions $\mu, \nu$, later specified as either $\mmd$ or $\wasserstein$, and $\what \varrho(\mu, \nu)$ an estimator of $\varrho(\mu, \nu)$ constructed by samples from $\mu$ and $\nu$. The multiple measurements $\measurement{i, t}$ in \cref{eq:model-dist} can be equivalently regarded as an empirical distribution.
% is regarded as an empirical distribution.


% \newcommand{\kernelnn}{\mathsf{KernelNN}}
% \newcommand{\wassersteinnn}{\mathsf{W_2NN}}
\kc{If there is no space in the end, then we can simplify the dnn algo by referring to $\rownn$ and changing few definitions. Seems like there is not much space left to discuss the methods.}
\fi


We elaborate on a vanilla version three step procedure of $\kernelnn, \wassersteinnn$ that explicitly constructs neighborhoods. The input are measurements $\mc Z$, missingness $\mc A$, the target index $(i, t)$ and the radius $\tuning$,
\begin{itemize}
    \item[\textbf{Step 1:}] (Distance between rows) Calculate the distance between row $i$ and any row $j \in [N] \setminus \{i\}$ by averaging the estimator of distribution metric $\what \varrho$:
    \begin{align}\label{eq:snn-distance}
        \distance{i, j}^{\mmd} := \frac{\sum_{s \neq t}\missing{i, s}\missing{j, s} \what{\mmd}_\kernel^2 ( \measurement{i, s}, \measurement{j, s} ) }{\sum_{s \neq t} \missing{i, s}\missing{j, s}} \qtext{and}  \distance{i, j}^{\wasserstein} := \frac{\sum_{s \neq t}\missing{i, s}\missing{j, s} \hatwasserstein^2 ( \measurement{i, s}, \measurement{j, s} ) }{\sum_{s \neq t} \missing{i, s}\missing{j, s}}.
    \end{align}
    \item[\textbf{Step 2:}] (Construct neighborhood) Construct a neighborhood of radius $\tuning$ within the $t$th column using the distances $\{\distance{i, j}:j \neq i\}$: 
    \begin{align}
        \neighbors{t, \tuning}^\mmd := \big\{ j \in [N] \setminus \{i\} : \distance{i, j}^\mmd \leq \tuning \big\} \qtext{and}  \neighbors{t, \tuning}^{\wasserstein} := \big\{ j \in [N] \setminus \{i\} : \distance{i, j}^{\wasserstein} \leq \tuning \big\}
    \end{align}
    \item[\textbf{Step 3:}] (Average across observed neighbors) Set $\mu^Z_{i, t} = n^{-1}\sum_{\ell = 1}^{n} \dirac_{\sample{\ell}(i, t)}$ as the empirical measure of the multiple measurements $\measurement{i, t}$. Take the barycenter within the neighborhood:
    % For row-wise neighbors $\sbraces{ j \neq i : \varrho_{i, j} \leq \eta}$ within $\eta$ radius, average across observed neighbors within $t$th column,
    \begin{align}\label{eq:dnn-average}
        \what{\mu}^{\mmd}_{i, t, \tuning} := \frac{1}{|\neighbors{t, \tuning}^\mmd|} \sum_{j \in \neighbors{t, \tuning}^\mmd} \missing{j, t} \mu_{j, t}^Z \quad\text{and}
        \what{\mu}^{\wasserstein}_{i, t, \tuning} := \argmin_{\mu} \sum_{j \in \in \neighbors{t, \tuning}^{\wasserstein}} \wasserstein^2(\mu, \mu_{j, t}^Z).
    \end{align}
\end{itemize}
For further details on the $\wasserstein$ and $\mmd$ algorithms see \cite{feitelberg2024distributional} and \cite{choi2024learning}, respectively.

\begin{algorithm2e}[H]
\caption{Vanilla~(row-wise) distributional nearest neighbor} 
  \label{algo:vanilla-dnn}
  \SetAlgoLined
  \DontPrintSemicolon
  \small
  {
\KwIn{\textup{$\mc Z, \mc A, \kernel, \tuning,$ $(i, t)$}}
  \BlankLine
    Initialize entry-wise metric $\entrydistest{\measurement{j, s}, \measurement{j', s'}} \gets$ $\what{\mmd}^2_\kernel(\measurement{j, s}, \measurement{j', s'})$ or $\hatwasserstein^2(\measurement{j, s}, \measurement{j', s'})$ \\
    Initialize metric $\entrydist{x, y} \gets$ ${\mmd}^2_\kernel(x, y)$ or $\wasserstein^2(x, y)$ \\
    Initialize tuning parameter ${\tuning} \gets (\tuning_1, 0)$\\
    Calculate row-wise metric $\big\{ \distance{i, j}^\row: j \neq i \big\} \gets $ $\distancemod(\what\varphi, \measurement{}, \missing{})$ \\
    Initialize weight $\weight{j, s} \gets  \indic{\distance{i, j}^\row \leq \tuning_1, \distance{s, t}^\col \leq \tuning_2}$ \\
    Calculate average $\what \mu_{i, t} \gets \averagemod(\varphi, \mc W, \mc Z, \mc A)$
    \BlankLine
\KwRet{$\what \mu_{i, t}$}
}
\end{algorithm2e} 




\subsection{Adaptively weighted nearest neighbors}
\label{app:star-nn}

We elaborate on the adaptive variant of the vanilla nearest neighbor algorithm $\awnn$ as mentioned in \cref{subsec: existing methods} and \cref{tab:summary}. The input are measurements $\mc Z$, and missingness $\mc A$. Note that there is no need for radius parameter $\eta$ and hence no CV.

\begin{itemize}
    \item[\textbf{Step 1:}] (Distance between rows and initial noise variance estimate) Calculate an estimate for noise variance and then the distance between any pair of distinct rows $i, j \in [N]$ by averaging the squared Euclidean distance across overlapping columns:
    \begin{align}\label{eq:snn-distance}
        \distance{i, j} := \frac{\sum_{s \neq t}\missing{i, s}\missing{j, s}(\measurement{i, s} - \measurement{j, s})^2}{\sum_{s \neq t} \missing{i, s}\missing{j, s}},\quad \overline{Z}\gets \frac{\sum_{j,s\in[N]\times[T]}A_{j,s}Z_{j,s}}{\sum_{j,s\in[N]\times[T]}A_{j,s}}, \qtext{and}
        \what{\sigma}^2\gets \frac{\sum_{j,s\in[N]\times[T]}A_{j,s}(Z_{j,s} - \overline{Z})^2}{\sum_{j,s\in[N]\times[T]}A_{j,s}}.
    \end{align}
    
    \item[\textbf{Step 2:}] (Construct weights) For all rows and columns $(i,t)\in[N]\times[T]$, evaluate $ w^{(i, t)} = ( w_{1, t}, \cdots,  w_{n, t})$, the weights that optimally minimizes the following loss involving an estimate of the noise variance $\what\sigma^2$,
    \begin{align}
    \label{eq: awnn weights}
         w^{(i, t)}    =\mbox{arg min}_{\widehat w^{(i, t)}}\brackets{2\log(2m/\delta)\widehat \sigma^2\|\widehat w^{(i,t)} \|_2^2 + \sum_{i' \in [N]} \widehat w_{i', t} A_{i',t} \widehat \rho_{i', i} }, 
    \end{align}
where $\widehat w^{(i, t)} = (\widehat w_{1, t}, \cdots, \widehat w_{n, t})$ is a non-negative vector that satisfy $\sum_{i' = 1}^n \what w_{i', t}A_{i',t} = 1$.
    \item[\textbf{Step 3:}] (Weighted average) Take the weighted average of measurements:
    % For row-wise neighbors $\sbraces{ j \neq i : \varrho_{i, j} \leq \eta}$ within $\eta$ radius, average across observed neighbors within $t$th column,
    \begin{align}\label{eq:awnn-average}
        \widehat \theta_{i,t} = \sum_{i' \in[N]}\widehat w_{i', t} A_{i',t}X_{i',t}, \qquad \forall (i,t)\in[N]\times[T]
    \end{align}

    \item[\textbf{Step 4:}] (Fixed point iteration over noise variance) Obtain new estimate of noise variance and stop if difference between old and new $\what\sigma^2$ is small.
    \begin{align}
        \what{\sigma}^2\gets \frac{1}{\sum_{i\in[N],t\in[T]}\missing{i,t}}\sum_{i\in[N],t\in[T]}\parenth{Z_{i,t}-\what{\theta}_{i,t}}^2\missing{i,t}
    \end{align}
\end{itemize}

\paragraph{No cross-validation in AWNN} The optimization problem in \cref{eq: awnn weights} can be solved exactly in linear time (worst case complexity) using convex optimization~\cite{sadhukhan2025adaptivelyweightednearestneighborsmatrix}. $\awnn$ doesn't rely on radius parameter $\tuning$. Not only it automatically assigns neighbors to ${(i, t)^{th}}$ entry during its weight calculation(non-neighbors get zero weight), but also takes into account the distance of the neighbors from the ${(i, t)^{th}}$ entry. The closer neighors get higher weights and vice - versa.

We further specify the exact implementation of the two modules $\distancemod$, $\averagemod$ to recover $\awnn$:


\begin{algorithm2e}[H]
\caption{$\awnn$ for scalar nearest neighbor} 
  \label{algo:awnn}
  \SetAlgoLined
  \DontPrintSemicolon
  \small
  {
\KwIn{\textup{$\mc Z, \mc A, $ $(i, t)$}}
  \BlankLine
    Initialize entry-wise metric $\entrydistest{\measurement{j, s}, \measurement{j', s'}}\gets ( \measurement{j, s} - \measurement{j', s'} )^2$ and metric $\entrydist{x, y} \gets (x - y)^2$\\
    Initialize noise - variance estimate ${\sigma_\eps^2} \gets \mrm{Variance}\parenth{\braces{\measurement{i,t}}_{(i,t)\in[N]\times[T]}}$\\
    Calculate row-wise metric $\big\{ \distance{i, j}^\row: j \neq i \big\} \gets $ $\distancemod(\what{\varphi}, \mc Z, \mc A)$ \\
    Initialize weight $\braces{\weight{1, t},\dots, \weight{n, t}  }\gets\mbox{arg min}_{\widehat w^{(i, t)}}\brackets{2\log(2m/\delta)\widehat \sigma^2\|\widehat w^{(i,t)} \|_2^2 + \sum_{i' \in [N]} \widehat w_{i', t} A_{i',t} \widehat \rho_{i', i} }$ \\
    Calculate average $\what \theta_{i, t} \gets \averagemod(\varphi, \mc W, \measurement{}, \missing{})$
    \BlankLine
\KwRet{$\what \theta_{i, t}$}
}
\end{algorithm2e} 


\input{icml2025/nn-new}


\iffalse
\kc{@TS, MP}


We introduce and discuss new variant of nearest neighbors that improve upon the shortcomings of previously introduced nearest neighbor algorithms on the scalar matrix \cref{eq:model}. First, cross-validation is a crucial step for all nearest neighbors, but the computation run-time scales as $O(N^2T^2|E|)$ where $E$ is the search space for $\tuning$ and $|E|$ its cardinality; there are $NT$ number of $\tuning$ to determine for $NT$ number of estimands and the row or column distance calculation requires at most $N^2 \vee T^2$ number of calculations. \kc{@TS, MP: How does $\awnn$ improve exactly in terms of order?.} Second, 

\kc{@TS, MP, pls fill in the details}

$\rownn$ can be viewed as $|\neighbors{t, \tuning}|$ nearest neighbors getting a weight of $\frac{1}{|\neighbors{t, \tuning}|}$ while others are assigned to a weight of 0. A natural generalization is introducing non-negative weights with closer neighbors getting higher weights and vice versa. A precise formulation will be for some $\neighbors{t} \subseteq [N]$, we assign 

\begin{align}
    \what{w}^{(i)}_{i',t} &= \indic{i'\in\neighbors{t}}\brackets{\frac{1}{|\neighbors{t}|} - \frac{1}{c\sigma^2}\parenth{\drow - \frac{1}{|\neighbors{t}|}\sum_{i'\in \neighbors{t}}\drow}} 
\end{align}

where $\sigma^2$ is the noise variance in the model and $c$ is a constant which ensures $\what{w}^{(i)}_{i',t}\geq 0$ $\forall i'\in [N]$.

\TSc{Needs different set of notations, have to include description of $\sigma^2$ in overview section.}
\fi



\iffalse
\begin{algorithm2e}[H]
\caption{Star NN\ --\ Return estimates of signals $\theta_{i,j}$ in a matrix of size $n\times m$ with small MSE} 
  \label{algo:row_star_NN}
  \SetAlgoLined
  \DontPrintSemicolon
  \small
  {
\KwIn{\textup{$n\times m$ Data Matrix $X$}}
  \BlankLine
    Initialize $\what{\sigma}^2\gets \Vararg{\parenth{X_{i,j}}_{i,j\in [n]\times[m]} }/10$\\
    \BlankLine
    $\drow \gets$ L2-row-distance$\parenth{X_{i\cdot},X_{i_0\cdot}}$, $\forall i,i_0\in[n]$ s.t. $i\neq i_0$\\[2pt]
    \BlankLine
    $\parenth{\what\theta_{i,j}}_{i,j\in [n]\times[m]} \gets$ {\normalsize\rowimputelink}\,$\parenth{X, \what\sigma^2, \frac{1}{\sqrt{n}},\parenth{\drow}_{i,i_0\in[n]^2}}$
    \\[2pt]
    \BlankLine
    $\what{\sigma}^2\gets \frac{1}{nm}\sum_{i\in[n],j\in[m]}\parenth{X_{i,j}-\what{\theta}_{i,j}}^2$\\
    \BlankLine
    Repeat Step 3 till the difference between new and old $\what\sigma^2$ is small.\\
    \BlankLine
\KwRet{\textup{$\parenth{\what\theta_{i,j}}_{i,j\in [n]\times[m]}$}}
}
\end{algorithm2e} 


\begin{algorithm2e}[H]
\caption{Row Imputer\ --\ Return weighted average of $\parenth{X_{i,j}}_{i,j\in [n]\times[m]}$ as the estimates of $\theta_{i,j}$'s} 
  \label{algo:row_imputer}
  \SetAlgoLined
  \DontPrintSemicolon
  {
  %
\KwIn{\textup{$n\times m$ Data Matrix $X$, noise variance estimate $\what\sigma^2$, probability $\delta$, row-wise distances $\what{d}^2\parenth{\cdot,\cdot}$ }}
 \BlankLine
$\what{d}^2\parenth{\cdot,\cdot}\gets \what{d}^2\parenth{\cdot,\cdot} - 2\what\sigma^2, \mathrm{Diag}\parenth{\what{d}^2\parenth{\cdot,\cdot}}\gets 0$\\[2pt]
    \For{$j = 1,\ldots, m$}
        {
        $\mathcal{A}(j)\gets\braces{i\in [n]|A_{i,j} = 1}$ 
            % $N_j\gets\abss{\mathcal{A}_j}$
            \\[2pt]
        \For{$i_0 = 1, \ldots, n$}
            {
            $u \gets $ {\normalsize \wgtadjlink}$\parenth{\braces{\frac{1}{\abss{\mathcal{A}_j}}-\frac{1}{8\what\sigma^2\log(1/\delta)}\parenth{\drow - \drowmeanfrac}}_{i\in[n]}}$\\[2pt]
            $\Wgt \gets$ $\begin{cases}
                &\max\braces{0, \frac{1}{\abss{\mathcal{A}_j}}-\frac{1}{8\what\sigma^2\log(1/\delta)}\parenth{\drow - \drowmeanfrac} - u}, \text{ if } i\in \mathcal{A}_j\\
                &0\hspace{10cm}\qtext{else}
            \end{cases}$\\[2pt]
            $\what\theta_{i_0,j}\gets\sum_{i\in\mathcal{A}_j}\Wgt X_{i,j}$
            }
        }      
  \KwRet{\textup{estimated signal matrix $\parenth{\what\theta_{i,j}}_{i,j\in [n]\times[m]}$}}
}
\end{algorithm2e} 



\begin{algorithm2e}[H]
\caption{Weight Adjuster\ --\ For a sequence $\pseqann$ with $\sumn a_i=1$, returns $u$ such that $\sumn\max\braces{a_i-u,0}=1$} 
  \label{algo:wgt_adjuster}
  \SetAlgoLined
  \DontPrintSemicolon
  \small
  {
  %
\KwIn{\textup{$n$-length sequence $\pseqann$ such that $\sumn a_i=1$}}
  \BlankLine
    $\pseqnn{b}{n}\gets \text{Sort}\parenth{\pseqann} \text{ in decreasing order}$\\[2pt]
    \BlankLine
    Initialize $\text{sum}\gets 0$\\[2pt]
    \BlankLine
    \For{$k=1,\ldots, n$}
        {
        $\text{sum}\gets\text{sum} + b[k]$\\[2pt]
        $u \gets \parenth{\text{sum} - 1}/k$\\[2pt]
        \If{$k == n \qtext{or} b_{k+1}\leq u$}
            {return $u$}
        }
}
\end{algorithm2e} 
\fi

\iffalse
\paragraph{Scalar nearest neighbors~($n = 1$)}
Target the mean $\theta_{i, t}$ under scalar matrix completion, i.e., $\measurement{j, s} = \sample{1}(i, t)$, and set $\entrydist{x, x'} = \entrydistest{x, x'} = (x - x')^2$. Sequentially implement modules $\distancemod$ and $\averagemod$ with the following specifics;
% we present a vanilla version of nearest neighbors, namely row-wise nearest neighbors~($\rownn$) and column-wise nearest neighbors~($ \colnn$), and two of its variants, two-sided nearest neighbors~($\tsnn$) and doubly-robust nearest neighbors~($\drnn$); refer to \cref{tab:summary_of_nn} for a concise comparison between the methods.


% \kc{(In progress) Still cleaning up and organizing.}
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
%         {$\rownn$} & $\weight{j, s} = \indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2} \ \ \text{with $\tuning = (\tuning_1, 0)$}.$ \\
%          {$\colnn$} & $\weight{j, s} = \indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2} \ \ \text{with $\tuning = (0, \tuning_2)$}.$\\
%          {$\tsnn$} & $\weight{j, s} = \indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2} \ \ \text{with $\tuning = (\tuning_1, \tuning_2)$}$. \\
%          {$\drnn$} & $\rownn + \colnn - \tsnn$.
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}

{$\rownn$}: $\weight{j, s} = \indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}$ with $\tuning = (\tuning_1, 0)$.

{$\colnn$}: $\weight{j, s} = \indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2} $ with $\tuning = (0, \tuning_2)$.

{$\tsnn$}: $\weight{j, s} = \indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}$ with $\tuning = (\tuning_1, \tuning_2)$.

{$\awnn$}: $w_{j, s} = A_{j,s}\brackets{\frac{1}{\sum_{i = 1}^NA_{i,s}} - \frac{1}{c\sigma^2}\parenth{\distance{i, j}^\row  - \ol{\distance{i}^\row }} - u}_+$ where $u$ is a constant so that $\sum_{j\in[N]}w_{j, s} = 1$ \kc{@TS, MP The notations are a bit heavy, can you simplify? Also, where is the column index $t$ in your weights?} 

{$\drnn$}: $\rownn + \colnn - \tsnn$. 
% \kc{Maybe adding subtract module makes things more neat?@Raaz: also does this hold when missingness is present??}

% \kc{I think the exact form of $\drnn$ has the following form:
% \begin{align}
%     \frac{\sum_{s\in \mbf N_{i, \tuning_2}}\missing{i, s}\measurement{i, s}w^{(1)}_s}{\sum_{s \in \mbf N_{i, \tuning_2}}\missing{i, s}w^{(1)}_s} + \frac{\sum_{j \in \mbf N_{t, \tuning_1}}\missing{j, t}\measurement{j, t}w_j^{(2)}}{\sum_{j \in \mbf N_{t, \tuning_1}}\missing{j, t}w_j^{(2)}} - \frac{\sum_{j \in \mbf N_{t, \tuning_1}}\sum_{s \in \mbf N_{i, \tuning_1}}\missing{i, s}\missing{j, t}\missing{j, s}\measurement{j, s}}{\sum_{j \in \mbf N_{t, \tuning_1}}\sum_{s \in \mbf N_{i, \tuning_1}}\missing{i, s}\missing{j, t}\missing{j, s}}
% \end{align}
% where $w_s^{(1)} = \sum_{j \in \mbf N_{t, \tuning_1}}\missing{j, t}\missing{j, s}$, $w_j^{(2)} = \sum_{s \in \mbf N_{i, \tuning_2}}\missing{i, s}\missing{j, s}$.}


% implement module $\distancemod(\what{\varphi}, \mc Z, \mc A)$ with the entry-wise distance as $\entrydistest{\measurement{j, s}, \measurement{j', s'}} = (\measurement{j, s} - \measurement{j', s'})^2$. Define the weights $\weight{j, s} = \indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}$ as a result of the first module. Then, implement the second module $\averagemod(\weight{}, \tuning, \varphi, \mc Z, \mc A)$ with $\varphi()$ the hyper-parameter vector $\Vec{\tuning} = (\tuning_1, 0)$ for some $\tuning_1$.

\paragraph{Distributional nearest neighbors~($n > 1$)} Target the distribution $\dist{i, t}$ under distribution matrix completion, i.e., $\measurement{i, t} = [\sample{1}(i, t), ..., \sample{n}(i, t)]$, and set $\weight{j, s} = \indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}$ with $\tuning = (\tuning_1, 0)$. Sequentially implement modules $\distancemod$ and $\averagemod$ with the following specifics;

{$\kernelnn$}: $\entrydistest{\measurement{i, t}, \measurement{j, s}} = \what{\mmd^2}_\kernel(\measurement{i, t}, \measurement{j, s})$ and $\entrydist{\mu, \nu} = \mmd_\kernel^2(\mu, \nu)$

{$\wassersteinnn$}: $\entrydistest{\measurement{i, t}, \measurement{j, s}} = \hatwasserstein(\measurement{i, t}, \measurement{j, s})$ and $\entrydist{\mu, \nu} = \wasserstein^2(\mu, \nu)$.

\fi



\iffalse
\subsection{Automated nearest neighbors}

\kc{with MP, could be doing a theoretical analysis of $\autonn$ (probably after 15th); for now this sub-section can be deleted.}
\fi

\iffalse
Define real valued functions $f_\gamma, g_\gamma \in \real$ on the real line, that are indexed by $\gamma \in [-1, 1]$ while also satisfying\footnote{An example of $f_\gamma, g_\gamma$ would be
\begin{align}
    f_\gamma(x) = (-\gamma/2 + 1/2) x + (\gamma/2 + 1/2) \qtext{and} g_\gamma(x) = (-\gamma/2 + 1/2)x.
\end{align}} 
\begin{align}
    f_{-1}(x) = x, \ g_{-1}(x) = x \qtext{and} f_1(x) = 1, \ g_{1}(x) = 0 \qtext{for all $x \in \real$.}
\end{align}
Implement $\distancemod$ module and define the neighborhoods $\neighbors{t, \tuning_1}^\row := \{j \neq i: \dist{i, j}^\row \leq \tuning_1\}$ and $\neighbors{i, \tuning_2}^\col := \{s \neq t: \dist{s, t}^\col \leq \tuning_2\}$. Then implement the averaging step,
\begin{align}
    &\what{\theta}_{i, t, \eta}^{\ \gamma} := \frac{\sum_{j \in \neighbors{t,\tuning_1}^\row, s \in \neighbors{i, \tuning_2}^\col}f_\gamma({\missing{j, t}})f_\gamma({\missing{i, s}})\missing{j, s}\big(g_\gamma(\syntheticmeasurement{j, t}) + g_\gamma(\syntheticmeasurement{i, s}) + \gamma \measurement{j, s}\big) }{\sum_{j \in \neighbors{t,\tuning_1}^\row, s \in \neighbors{i, \tuning_2}^\col}f_\gamma(\missing{j, t})f_\gamma(\missing{i, s})\missing{j, s}}
\end{align}
where 
\begin{align}
    \syntheticmeasurement{j, s} := \begin{cases}
        \text{average across row $j$ or column $s$} &\qtext{if $A_{j, s} = 0$}\\
        \measurement{j, s} &\qtext{if $A_{j, s} = 1$}.
    \end{cases}
\end{align}
Notice that $\what\theta^{\ -1}_{i, t, \tuning} = \what{\theta}^{\dr}_{i, t, \tuning}$ and $\what\theta^{\ 1}_{i, t, \tuning} = \what{\theta}^{\ts}_{i, t, \tuning}$; so the uniform~(over $\real$) behavior of $f_\gamma, g_\gamma$ as $\gamma$ fluctuates would characterize how $\what \theta^{\gamma}_{i, t, \tuning}$ interpolates between $\drnn$ and $\tsnn$. A cross-validated $\gamma$ enables $\nn$ to adapt to the environment of the real world data. 
\fi

==> eurips2025/case-study.tex <==
\section{\lib{}-Bench and Results}\label{sec:case-study}

In this section, we evaluate several nearest neighbor algorithms provided by our library, \lib{}, on real-world data. As part of our package, we include data loaders which automatically download the necessary datasets and format them for evaluation. These datasets and loaders comprise our proposed benchmark for nearest neighbor matrix completion algorithms, \lib{}-\textbf{Bench}. We also test several existing popular matrix completion techniques~\cite{hastie2015matrix,chatterjee2015matrix}. For details on our experimental setup, computing hardware, and boxplot generation, see \cref{app:case-studies}.


% ----------------
\iffalse
\subsection{Synthetic data}
\label{sub:simulations}


We first compare different matrix completion techniques on a synthetically generated data set. Our goal is to track the performance of different algorithms as the matrix size scales. We generate data matrix of size $N \times T$, where measurements $\measurement{i, t}$~(when $\missing{i, t} = 1$) are generated from distribution $\mu_{i, t} = \theta_{i, t} + \varepsilon_{i, t}$ where $\varepsilon_{i, t}$ are exogenous and i.i.d. centered Normal random variables. For more specifics on the data generation, see \cref{app:synthetic_gen}. The task here is to
\fi

% our synthetic data matrices with $d$-dimensional row latent factors $\uset := \{u_i, i\in[N]\}$, and column latent factors $\vset := \{v_t, t\in[T]\}$. For the following experiments, we let ${u_i \sim \text{Unif}[-0.5, 0.5]}$ for all $i \in [N]$ and ${v_t \sim \text{Unif}[-0.5, 0.5]}$ for all $t \in [T]$. 

% ----------------
\subsection{Personalized healthcare: HeartSteps}
\label{sub:hs}

% \paragraph{Case-study introduction}

The HeartSteps V1 study~(HeartSteps study for short) is a clinical trial designed to measure the efficacy of the HeartSteps mobile application for encouraging non-sedentary activity \cite{klasnja2019efficacy}. The HeartSteps V1 data and its subsequent extensions have been widely used for benchmarking a variety of tasks including counterfactual inference of treatment effect \cite{dwivedi2022counterfactual, choi2024learning}, reinforcement learning for intervention selection \cite{liao2019rlheartsteps}, and micro-randomized trial design \cite{qian2022microrandomized}. In the HeartSteps study, $N = 37$ participants were under a 6-week period micro-randomized trial, where they were provided with a mobile application and an activity tracker. Participants independently received a notification with probability $p = 0.6$ for $5$ pre-determined decision points per day for 40 days~($T = 200$). We denote observed entries $Z_{i, t}$ as the mean participant step count for one hour after a notification was sent and unobserved entries as the unknown step count for decision points where no notification was sent. Our task is to estimate the counterfactual outcomes: the participant's step count should they have received a different treatment (notification or no notification) than they did at specific time points during the study. 
% By computing the counterfactual outcome, we can also estimate the treatment effect of an intervention on an individual.
 

% Thus, the treatment application~(notification sent) is subject to an an individual's latent characteristics such as their personal schedule and daily routines. 

%availability of individuals encoded in the randomized trial implies that treatment application~(notification sent)

%Further, as notification are never sent during non-available times, positivity is clearly violated in this example.    % random given that they are available, positivity is violated as unavailable times has 0.0 probability 


% We proceed on our empirical analysis by imposing the potential outcome observation model \cref{mod:potential-outcome} on the HeartSteps data. 


\paragraph{Results \& Discussion.} We benchmark the performance of the matrix completion methods by measuring absolute error on held-out observed step counts across 10 participants in the last 50 decision points. We use the remaining data to find nearest neighbor hyperparameters using cross-validation. To benchmark distributional nearest neighbors methods ($\kernelnn$ and $\wassersteinnn$) against the scalar methods, we first set each entry to have the number of samples $n = 60$, where each sample is the 1 minute step count before imputation. Then, we take the mean of the imputed empirical distribution as the estimate. 

In \cref{fig:hs-results}(a), we compare the absolute error of the imputed values across the nearest neighbor and baseline methods. The scalar nearest neighbor methods far out-perform USVT and are on par with SoftImpute. The two distributional nearest neighbor methods far outperform all methods operating in the scalar setting; it suggests that matching by distributions collect more homogeneous neighbors, thereby decreases the bias of the method, compared to matching only the first moments as done in most scalar matrix nearest neighbor methods. 

% which suggests that finding neighbors using a distributional distance can enhance the quality of the neighbors and reduce the bias of the estimate. 

In \cref{fig:hs-results} panel (b), we show an example of an imputed entry in the distributional nearest neighbors setting. In this case, the ground truth distribution is bimodal, as the participant was largely sedentary (0 steps) with small amounts of activity. While both $\kernelnn$ and $\wassersteinnn$ capture the sedentary behavior of the participant, $\kernelnn$ is able to recover the bimodality of the original distribution whereas $\wassersteinnn$ cannot. 


% \begin{wrapfigure}{R}{0.5\textwidth}
%     \begin{center}        \includegraphics{figure/hs_est_errors_boxplot.pdf}
%     \end{center}
%     \caption{\tbf{HeartSteps V1: Estimation error under notification sent.} We apply log-transform to the raw step counts before imputing.}
%     \label{fig:hs-results}
% \end{wrapfigure}

\begin{figure}[ht]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.47\textwidth]{figure/hs_est_errors_boxplot.pdf} &  
        \includegraphics[width=0.33\textwidth]{figure/hs_distplot_48.pdf} \\
        (a) Absolute error of mean step count prediction &
        (b) $\kernelnn$ vs. $\wassersteinnn$
    \end{tabular}
    \caption{\tbf{HeartSteps: estimating step count under scalar and distributional matrix completion settings.} Panel (a) shows the absolute error of predicted step count of the nearest neighbor methods against matrix completion baselines (SoftImpute, USVT). Panel (b) shows an example of an imputed entry in the distributional matrix completion setting.
    }
    \label{fig:hs-results}
\end{figure}
% ----------------

\subsection{Movie recommendations: MovieLens}\label{sec:movielens}
\begin{wrapfigure}{R}{0.5\textwidth}
    \begin{center}        \includegraphics{figure/movielens_est_errors_boxplot.pdf}
    \end{center}
    \caption{\tbf{MovieLens: Estimation error for a random subsample of size 500.} For experimental settings and discussion see \cref{sec:movielens}.}
    \label{fig:movielens-error}
\end{wrapfigure}

The MovieLens 1M dataset \cite{movielens} contains 1 million ratings (1–5 stars) from 6,040 users on 3,952 movies. Collaborative filtering on MovieLens has long been a benchmark for matrix-completion methods: neighborhood-based algorithms~\cite{sarwar2001item}, latent-factor models~\cite{koren2009matrix}, and, more recently, nearest neighbors interpreted as blind regression under a latent–variable model~\cite{li2019nearest}. These assist practitioners in data-driven recommendation systems, since more accurate rating imputation directly drives better personalized suggestions and user engagement. This is a standard scalar matrix completion problem with $N=6,040$ and $T=3,952$. Each rating is an integer in $\{1,\dots,5\}$. The dataset has a very high percentage of missing values: 95.53\% missing. Our task is to estimate unobserved ratings using various matrix completion algorithms. We benchmark the performance of nearest neighbors against matrix factorization by measuring absolute error on held‑out ratings. See \cref{app:movielens} for additional details on the dataset.

\paragraph{Results \& Discussion.} We fit the nearest neighbor methods using a random sample of size 100 from the first 80\% of the dataset to choose nearest neighbor hyperparameters via cross-validation.We then test the method on a random subsample of size 500 from the last 20\% of the dataset. As observed in \cref{fig:movielens-error}, all nearest neighbor methods have a lower average error than USVT and a much lower standard deviation of errors, with $\colnn$, $\rownn$, $\drnn$, and $\autonn$ performing the best out of the nearest neighbor methods. SoftImpute performs on par with the nearest neighbor methods. Note that the nearest neighbor methods perform well even while only being trained on a tiny subset of the data of size 100 out of the 1 million ratings available.


% ----------------
% \input{icml2025/llm_evaluation_new}
% \input{icml2025/llm_evaluation}

==> eurips2025/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our main claims in our abstract are a unified framework, a unified Python package, and a new test bench for nearest neighbor-based matrix completion methods. We present our unified framework for nearest neighbor-based matrix completion methods in \cref{sec:unified-view}. We present our package structure in \cref{sec:library}. Finally, we describe the new test bench in \cref{sec:case-study}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss improvements to our Python package in \cref{sec:conclusion}. The algorithms described in \cref{sec:nn-overview} use theoretical assumptions for their theoretical guarantees, but these assumptions do not affect the algorithms themselves, and thus pose no limitations on our Python package or test bench.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not claim any theoretical results in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All of our results can be reproduced with the code on our GitHub, which is (anonymously) linked in the paper. Each experiment has its own folder with instructions on how to run the experiments. We provide Python files which automatically download the necessary data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide an anonymous GitHub link to our open-source code. Every experiment can be reproduced with the Python files we provide separately from our Package source files. The new Python package we present, also in the GitHub link, can be installed quickly on standard computing hardware and do not require access to GPU's or any other specialized hardware.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For each experimental setup, we describe how we split up the datasets into train and test sets. We describe in detail how our hyperparameters are chosen in the Appendix. We also provide the code we use to choose hyperparameters in our open-source repository.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe how we generate our boxplots to compare error across methods in \cref{app:case-studies}. We also detail how our error bars are generated in our figures in the respective figures which have error bars.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe our computing setup in \cref{app:case-studies}. It is standard laptop hardware.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our research conforms with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work does not have any direct societal impact. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our new Python package and test bench do not pose a significant risk for misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Every library and dataset used in this work is properly cited and credited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work primarily releases a new code library that we have placed under the MIT License.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve any work with human subjects nor crowdsourcing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include any human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper's proposed algorithms do not involve LLM's in an important way.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> eurips2025/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

In this paper, we present a unified framework, Python library (\lib{}), and test bench (\lib{}-\textbf{Bench}) for nearest neighbor-based matrix completion algorithms. We demonstrate how our library supports a diverse set of datasets spanning patient-level healthcare causal inference (HeartSteps) and recommendation systems (MovieLens). 
% See the appendix for  counterfactual inference for panel data (Proposition 99), and LLM evaluation (PromptEval). 
Our framework and library facilitates researchers and practitioners to try NN methods on novel datasets as well as extend the package with more complex methods.

In future work, we plan on speeding up the runtime of \lib{}, particularly for commonly used settings such as scalars-valued matrices. We also plan on adding support for distributed datasets too large to fit into memory. Finally, we plan on extending the library to other nearest neighbor algorithms, such as approximate nearest neighbors methods and ones that use linear regression instead of simple averaging.

% \ag{Future work: (1) speeding up, (2) bringing together approximate nearest neighbors (find references from supervised learning literature: \url{https://scholar.google.com/citations?user=9r7_pN8AAAAJ&hl=en})}

==> eurips2025/intro.tex <==
\section{Introduction}

Nearest neighbor methods are a class of non-parametric algorithms widely used for regression, classification and pattern recognition. Due to their scalability and success under models with minimal assumptions, nearest neighbor methods have recently been adopted for practical fields such as matrix completion and counterfactual inference in panel data settings. Matrix completion is a well-established field that supplies practitioners with many tools to recover underlying matrices using partial or even noisy observations~\cite{hastie2015matrix,chatterjee2015matrix,keshavan2010matrix}, with recommendation systems~\cite{koren2009matrix,recht2011simpler} as an important use-case. Panel data counterfactual inference aims at learning the treatment effect of policies across time~\cite{bai2009panel,bai2021matrix,athey2021matrix}. One important example is individualized healthcare predictions~\cite{klasnja2019efficacy}. Nearest neighbor methods were recently recognized as effective in providing granular inference guarantees for both matrix completion and counterfactual inference when either the missingness or the policy treatment are not completely random and confounded~\cite{ma2019missing,dwivedi2022counterfactual,agarwal2023causal}. 

% because they have bee?n shown to be competitive in terms of accuracy, can impute entry-wise, and are widely used in practice.


% Data scientists looking to use matrix completion to impute missing data have a diverse set of tools at their disposal including spectral based methods~\cite{hastie2015matrix,chatterjee2015matrix}, gradient methods (\cite{keshavan2010matrix}), 

% and nearest neighbor methods~\cite{li2019nearest,dwivedi2022counterfactual,agarwal2023causal,choi2024learning,feitelberg2024distributional}. 

Despite nearest neighbor methods popularity, there is no unified package that lets a user easily switch between different kinds of nearest neighbor algorithms for matrix completion and counterfactual inference. In this paper, we present a package\footnote{\url{https://github.com/aashish-khub/NearestNeighbors}} to unify several nearest neighbor methods under a single interface, so users can easily choose the method that suits their data the best.

%(\href{https://anonymous.4open.science/r/NearestNeighbors-7D12/README.md}{GitHub link: \lib{}})  
% Next, we review two broad applications of nearest neighbors and matrix completion: recommendation systems and panel data settings.

% \paragraph{Recommendation systems} In the problem of a recommendation system, multiple users submit ratings / preferences for a subset of items, and the vendor recommends items based on the partial rating information \cite{rennie2005fast}. Prediction of unseen ratings is the key to a good recommendation, and the predictions are based on the patterns of the partially observed ratings which can be formalized into a matrix completion problem. A popular instance is the Netflix problem, an open competition for the best prediction algorithm of user ratings of films. Users~(rows of matrix) have the option to rate the films~(columns of matrix). However, users typically rate only a subset of films, and the ratings are commonly biased towards their preferences. Under the common belief that only a few factors drive the preference and ratings of the users, many matrix completion algorithms have resorted to the low rank assumption on the ratings matrix~\cite{recht2011simpler,candes2012exact}. Variants of nearest neighbors~(in short, $\nn$) recently were introduced to correct for the potential bias originating from the fact that observation patterns are influenced by the matrix entries~(e.g. ratings) themselves and by unmeasured confounders~\cite{agarwal2023causal,abadie2024doubly}. 

% \paragraph{Panel data} Panel data constitutes measurements of multiple units that are tracked over time~(hence a type of longitudinal data) as they undergo different types of interventions at different times~\cite{bai2009panel}. Panel data is used to analyze the causal effects of any policies, treatments, or business decisions that affect the subjects in the data, making this data type essential in econometrics and health studies. Matrix completion algorithms enable estimation of these causal effects at the unit$\times$time level, the most granular scale where causal effects can be estimated~\cite{athey2021matrix,agarwal2023causal}. For example, consider a mobile health app trying to learn the effectiveness of two exercise routines. Suppose the app alternates two routines across $N$ different users repeatedly over $T$ weeks, where their health activities~(say physical step counts) throughout each week are recorded. Then, we can use matrix completion to impute the counterfactual step counts under treatment and control, allowing us to estimate causal effects at the most granular scale.

\subsection{Our contributions}

\newcommand{\starnn}{\mathsf{StarNN}}
\newcommand{\autonn}{\mathsf{AutoNN}}

Overall, our contributions in this paper are summarized below: 
% \kc{if we are not using (C1)... later in the paper, maybe consider using simple dots?}
% \begin{enumerate}[label=(C\arabic*)]
\begin{enumerate}
    \item We provide a unified, easy to implement nearest neighbor library that contains a breadth of nearest neighbor algorithms for matrix completion problems.
    \item We present a unified framework for nearest neighbor algorithms that facilitates extending to new variants.
    % \item We introduce a new nearest neighbors algorithm, auto nearest neighbors~(in short $\autonn$), which aims both to improve on the existing methods and demonstrate the ease of developing new variants with our library.
    \item We demonstrate our library's wide applicability through several real-world data sets in a new test bench called \lib{}\textbf{-Bench}.
\end{enumerate}

% \subsection{Related work}
% We contextualize our contributions in the context of both nearest neighbors as a general algorithm and matrix completion specifically.

% \paragraph{Nearest neighbors}

% As introduced above, nearest neighbor methods are widely used for non-parametric regression, classification, and pattern recognition~\cite{cover1967nearest,cannings2020local}. Recently, nearest neighbor methods were introduced as an effective algorithm for matrix completion problems~\cite{li2019nearest,agarwal2023causal,dwivedi2022counterfactual}, especially when the missingness depended on observations and unobserved confounders. The fact that nearest neighbor methods target a single entry at a time via matching makes it effective against various types of missing patterns. The class of algorithms has grown to account for a wide range of applications~\cite{dwivedi2022doubly,choi2024learning,feitelberg2024distributional,sadhukhan2024adaptivity, sadhukhan2025adaptivelyweightednearestneighborsmatrix}, with a focus on inference for personalized treatment effects in the causal inference literature. Our library, \lib{}, is designed to easily implement the vanilla versions of nearest neighbors~\cite{li2019nearest,dwivedi2022counterfactual} as well as its unweighted~\cite{dwivedi2022doubly,sadhukhan2024adaptivity} and weighted~\cite{sadhukhan2025adaptivelyweightednearestneighborsmatrix} variants. Finally, \lib{} is also capable of distributional matrix completion~\cite{choi2024learning,feitelberg2024distributional}.

% \paragraph{Other matrix completion methods}

% % \kc{@ MP, TS: Let's make this less notation heavy, more comprehensive citations, include soft-impute~\cite{hastie2015matrix} as it is one of our benchmarks.} 

% Universal singular value thresholding (USVT), proposed in \cite{chatterjee2015matrix,bhattacharya2022matrix}, is a classical spectral-based method for performing matrix completion; its core functionality is based on a singular value decomposition of the matrix and thresholding the singular values.
% %
% SoftImpute, introduced by \cite{hastie2015matrix}, is another widely used optimization-based algorithm for matrix completion. The algorithm computes ridge-regression updates of the low-rank factors iteratively and finally soft-thresholds the singular values to impose a nuclear norm penalty. 
% %
% Notably USVT and SoftImpute have provable guarantees when missingness is completely at random, but empirically fail when the missing pattern depends on the observed entries or the unobserved confounders~\cite{agarwal2023causal}. Our real-world analysis in \cref{sec:case-study} once again demonstrates this point.

% The USVT algorithm completes a matrix by imputing zero for all the missing entries of the matrix, obtaining a estimate $\widehat p$ of the observation probability, performing a singular value decomposition of the imputed matrix, and retaining only those singular values that exceed $\tau \sqrt{\min\{N, T\}}$ (where $\tau > 2 \widehat p$). 

% \cite{chatterjee2015matrix} shows that the proposed algorithm attains minimax optimal performance when estimating matrices constrained by a bounded nuclear norm. 

\paragraph{Existing software for matrix completion and nearest neighbors}

Scikit-Learn \cite{scikit-learn}, a popular Python package for machine learning tools, implements a simple k-nearest neighbor algorithm for imputing missing values in a feature matrix. However, their implementation is designed for the feature matrix setting. So, neighbors are only defined across samples (row-wise). Additionally, they do not provide any implementation for more advanced nearest neighbor algorithms, nor does their package allow for easy extendability like our proposed package. 
% Another package which implements nearest neighbors for matrix completion is the Synthetic Nearest Neighbors (SNN) package (\url{https://github.com/deshen24/syntheticNN}). SNN implements a specific nearest neighbor algorithm for the causal matrix completion setting. 

% \paragraph{Organization}

% \cref{sec:nn-overview} contains an overview of the existing nearest neighbor algorithms implemented in our library, \lib{}. 
% % \cref{sec:new-nn} introduces a new nearest neighbor algorithm, $\autonn$, that is also implemented in \lib{}. 
% \cref{sec:library} touches upon the high-level (class) structure of \lib{}, as well as the interface for practitioners. \cref{sec:case-study} tests different variants of nearest neighbor methods and classical methods on our new test bench of diverse datasets called \lib{}-\textbf{Bench}. Finally, in \cref{sec:conclusion}, we provide concluding remarks and outline future directions of research.








==> eurips2025/library.tex <==
\section{\lib{} Package and Interface}\label{sec:library}

We now present our unified Python package, \lib{}, for nearest neighbor algorithms for matrix completion. In particular, we provide a class structure which abstracts the estimation procedure utilized in each different nearest neighbor method and is facilitated by $\distancemod$ and $\averagemod$ modules described in more detail in \cref{app:nn-algo}. On top of that, our library enables easy extension to other nearest neighbors algorithms and other data types on top of scalars and distributions. For example, as long as a distance and average notion are well defined, our library can be easily applied to a matrix of images or text strings. 

% \paragraph{Class structure.} The core functionality of \lib{} is based on two abstract classes: \texttt{EstimationMethod} and \texttt{DataType}.

% \texttt{EstimationMethod} classes contain the logic to impute a missing entry such as how to use calculated distances. 
% % In the context of the modules in \cref{sec:nn-overview}, this class determines the weighting function or, in the context of $\drnn$ and $\autonn$, how to compose estimates. 
% We separate this from the \texttt{DataType} abstraction because several estimation methods can be used for multiple data types. For example, \texttt{RowRowEstimator} implements the $\rownn$ procedure for any data type given to it, such as scalars or distributions.

% % \texttt{DataType} classes implement the $\distancemod$ and $\averagemod$ modules for any kind of data type (e.g. scalars which use squared distance and simple averaging). 
% \texttt{DataType} classes implement a \emph{distance} and \emph{average} function for any kind of data type. For scalars we use squared distance and simple averaging. For distributions, we implement two metrics, Wasserstein ($\wassersteinnn$) and kernel maximum mean discrepancy (MMD, $\kernelnn$). This abstract class allows for our package to extend to any data types beyond the ones we tested. For instance, a practitioner can easily add a \texttt{DataType} for text strings which uses vector embeddings to find distances and averages between between strings without needing to rewrite any of the estimation procedure.

\paragraph{Interface.} The core functionality of \lib{} is based on two abstract classes: \texttt{EstimationMethod} and \texttt{DataType}. The details of these classes can be found in \cref{app:class_struct}. To use our library, a user simply has to instantiate a composite class \texttt{NearestNeighborImputer} with their \texttt{EstimationMethod} and \texttt{DataType} of choice. We provide constructor functions to automatically create popular \texttt{NearestNeighborImputer} classes such as a two-sided nearest neighbor estimator with the scalar data type. From a design pattern point of view, this is known as a \emph{Composite} design pattern \citep[pg. 163]{gamma1993design}. We use this design pattern so that anyone looking to customize the estimation procedure can do so for any kind of data type simultaneously. Similarly, with the exception of doubly robust estimators, each estimation procedure works out of the box with any data type that implements the \texttt{DataType} abstract class. The Doubly robust estimation method does not work out of the box with distributions because a subtraction operation is not well defined in the distribution space.

Finally, the user simply needs to input (i) a data matrix, (ii) a mask matrix which specifies which values are missing, and (iii) the row and column to impute. Thus, a user can test out different estimation procedures by changing just one line of code. Separately from the core functionality, we have also implemented several cross-validation classes detailed in \cref{app:cv} which take in a \texttt{NearestNeighborImputer} class and find the best hyperparameters to use (e.g., distance thresholds and weights). 

% NN 2 pages

% Star NN, Auto NN at most 1 page.

% library
% 1~1.5page

% case
% 3pages

==> eurips2025/llm_evaluation.tex <==
\subsection{Efficient LLM evaluation}

Recent works show there is non-trivial variability of performance of language models across different prompting techniques\cite{sclar2023quantifying,polo2024efficient}, a natural follow up task being identification of the best performing prompting templates for certain tasks and language models~\cite{shi2024best,polo2024efficient}. The difficulty here is that there are near infinite ways of prompting, so an efficient evaluation framework has been investigated thoroughly~\cite{ye2023predictable,perlitz2023efficient}. Motivated by \cite{polo2024efficient}, we use the MMLU dataset~\cite{hendrycks2020measuring} and empirically demonstrate that our nearest neighbors method can achieve efficient evaluation. Under a fixed task~(e.g. abstract algebra, political science) various questions / examples are queried to a specific model, where each questions are restructured using different prompting templates. Either the model answers the question correctly or not and correctness is recorded. 

\paragraph{Results \& Discussion}

\kc{Do both SNN and DNN}

There are $57$ tasks and $15$ models total; the number of questions / examples depend on the task of interest and there is a fixed set of $100$ prompting templates that is applied to whatever question of whatever task. \kc{Could make a sub-section that explains MMLU.}


We consider a distributional matrix completion setup and implement a Dist-NN to estimate the distribution of averaged scores across templates~(template instances are of no value, as we aim to learn the overall variation) leveraging information across different models and different tasks. Imputation in \cite{polo2024efficient} was done while fixing model and task, so the commonalities that may exist across different models and tasks were not utilized.




% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figure/template_subject_model_by_propensity.pdf}
%     \caption{\kc{Figure needs adjustment, will not include boxplots of MMD errors for Kernel NN as most of them are zero---Wasserstein NN might have meaningful boxplots.} p = , standardize X }
%     \label{fig:temp_sub_model}
% \end{figure}



==> eurips2025/llm_evaluation_new.tex <==
\subsection{Efficient LLM evaluation: PromptEval}
\label{sub:llm}

% \begin{wrapfigure}{R}{0.5\textwidth}
%     \begin{center}
%     \includegraphics{figure/prompteval_est_errors_boxplot-p0.5.pdf}
%     \end{center}
%     \caption{\tbf{Kolmogorov-Smirnov distance with missingness at 50\%.} $\mmd$ using column-wise nearest neighbors performs the best in terms of the KS distance.}
%     \label{fig:ks}
% \end{wrapfigure}

The rapid advancement of LLMs have placed them at the center of many modern machine learning systems, from chatbots to aids in medical education \cite{geathers2025benchmarking}. In practice, system architects want to strike the right balance of real-world performance and cost, but navigating this Pareto frontier is a daunting task. 2024 alone saw at least 10 new models from Anthropic, Google, Meta, and OpenAI, not even counting the multitude of open-source fine-tuned models built on top of these.
% (Moreover, this number is likely to only grow as training models becomes more accessible, thanks in part to DeepSeek R1.) 
On specific tasks, smaller, fine-tuned models may even outperform the latest frontier models, in addition to being more cost effective.

We investigate how matrix completion, specifically nearest neighbor methods, can alleviate some of these burdens. We use the PromptEval dataset \cite{polo2024efficient}, which evaluates $15$ open-source language models (ranging in size from 3B to 70B parameters) and $100$ different prompting techniques across the 57 tasks of the MMLU benchmark \citep{hendrycks2020measuring}. In practice, the performance of a model depends---sometimes dramatically---on the precise input prompt. This suggests that we need to consider the performance of a model across a wide range of prompts, rather than any one prompt in particular. 
Thus, we model this problem as a distributional matrix completion problem with $N=15$, $T=57$, and $n=100$.
Given one of 57 tasks, we aim to accurately characterize the performance of each model without resorting to exhaustive evaluation.
Nearest neighbors leverage commonalities across models and tasks to estimate the performance distribution of each entry, which was otherwise not considered in \cite{polo2024efficient}; previous literature achieves efficient evaluation per model and task in isolation without leveraging any across model / task information. 

% \rd{We have to explain why this method is better here.}

% Scalar matrix completion is one approach to achieving such parsimony. In the language of matrix completion, we define the rows to be model-prompt pairs and the columns to be MMLU questions (14,079 in total).
% \ag{probably have to explain what a prompt is}
% Widely used to evaluate frontier LLMs, MMLU comprises $57$ tasks (e.g. abstract algebra, political science) \ag{insert the total number of questions} totally $14079$ questions in the test set.
% Each task is associated with varying questions, each associated with a ground-truth answer. 
% When faced with identifying the best prompting technique, considering all combinations of (1) model, (2) prompting technique, and (3) task is not only expensive, but also highly wasteful \cite{shi2024best,polo2024efficient}. 
% Nearest neighbor methods enable a cheap way to identify the best prompt.
% \citet{sclar2023quantifying,polo2024efficient} show that different prompting techniques lead to widely different results.
% \paragraph{Speeding up best prompt identification.}
% For a given a model, our first problem is to estimate the fitness of a prompting technique on a particular task. Note that each MMLU task is associated with a set of question (ranging in size from 100 to ???).
% We then randomly include each entry of the matrix independently with probability $p$ and estimate the missing entries.
% For each model, task, and prompt combination, we aggregate the scores (both observed and estimated) to obtain a value between 0 and 1. We then apply further aggregation to obtain a distribution for each model-task pair.
% \cref{tab:llm_scalar} shows the Kolmogorov statistic between the estimated and ground-truth distributions.
% In principle, standard matrix completition methods like USVT are well-suited for MCAR settings like the one considered here, yet nearest neighbor methods still perform the best empirically.
% Nearest neighbor methods are able to leverage commonalities across questions and prompts to estimate missing entries.

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=0.47\textwidth]{figure/ksbyp_prompteval_plot.pdf} 
        &  
        \includegraphics[width=0.45\textwidth]{figure/distributions-entry40-tp4.0.pdf} 
        \\
        (a) Mean KS distance between estimated and
        &
        (b) $\kernelnn$ vs. $\wassersteinnn$ \\
         ground-truth distributions
    \end{tabular}
    \caption{\textbf{Distributional nearest neighbor methods enable efficient LLM evaluation on MMLU.} We estimate LLM score distributions across all models and tasks given only a limited number of model-task evaluations, determined by the propensity $p$. See \cref{sub:llm} for a detailed discussion.}
    \label{fig:llm}
\end{figure}

\paragraph{Results \& Discussion.}
We randomly include each entry in the matrix independently with probability $p\in \braces{0.3,0.5,0.7}$ and impute the missing entries using the $\kernelnn$ and $\wassersteinnn$ methods of \cref{tab:summary}. For each method, we consider both the the row-wise and column-wise variants.
\cref{fig:llm}(a) reports the mean Kolmogorov-Smirnov (KS) distance between the imputed and ground-truth distributions across the entries in the test set for varying missingness values. As expected, estimation error decreases as $p$ increases.
% the number of observed entries increases. 
% versus the ground truth at varying levels of $p$ for a select entry in the matrix. At $p=0.3$, we avoid 70\% of LLM evaluations, yet still recover the distribution of prompt scores with reasonable quality. At $p=0.5$ and $p=0.7$, column-wise NN with $\mmd$ performs the best.
\cref{fig:llm}(b) visualizes the imputed distributions using row-wise $\kernelnn$ and column-wise $\wassersteinnn$ (at $p=0.7$) for a select entry, along with the ground-truth distribution. Even with 30\% of matrix entries missing, distributional NN methods are able to recover the underlying distribution.

% To further reduce estimation error, we look to exploit commonalities across the models.
% We consider a distributional matrix completion setup and implement a Dist-NN to estimate the distribution of averaged scores across templates~(template instances are of no value, as we aim to learn the overall variation) leveraging information across different models and different tasks. 
% Imputation in \cite{polo2024efficient} was done while fixing model and task, so the commonalities that may exist across different models and tasks were not utilized.

% \ag{Maybe we should also include baseline from PromptEval for the distributional setting? That will make this section even stronger I think.}


% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figure/template_subject_model_by_propensity.pdf}
%     \caption{\kc{Figure needs adjustment, will not include boxplots of MMD errors for Kernel NN as most of them are zero---Wasserstein NN might have meaningful boxplots.} p = , standardize X }
%     \label{fig:temp_sub_model}
% \end{figure}



==> eurips2025/nn-new.tex <==
\subsection{New variant: Auto nearest neighbors}\label{sec:new-nn}

$\tsnn$ is a generalization of $\rownn$ and $\colnn$ by setting one of the tuning parameters to zero~(see \cref{tab:summary}), whereas the idea underlying $\drnn$ is fundamentally different from that of $\tsnn$; $\drnn$ debiases a naive combination of $\rownn$ and $\colnn$ whereas $\tsnn$ simply boosts the number of measurements averaged upon, thereby gaining from lower variance. 
So we simply interpolate the two methods for some hyper-parameter $\alpha \in [0, 1]$; see \cref{tab:summary}.
Notably the hyper-parameter $\tuning$ for both $\drnn$ and $\tsnn$ are identical when interpolated.

Suppose $\dist{i, t} = \theta_{i, t} + \varepsilon_{i, t}$ in \cref{eq:model} where $\varepsilon_{i, t}$ are centered i.i.d. sub-Gaussian distributions across $i $ and $t$.
% \rd{why do we need Gaussian noise?}. 
When $\sigma$ is large in magnitude, $\tsnn$ denoises the estimate by averaging over more samples, hence providing a superior performance compared to $\drnn$ in a noisy scenario. When $\sigma$ is small so that bias of nearest neighbor is more prominent, $\drnn$ effectively debiases the estimate so as to provide a superior performance compared to $\tsnn$. The linear interpolator $\autonn$ \textit{automatically} adjusts to the underlying noise level and debiases or denoises accordingly; such property is critical when applying nearest neighbors to real world data set where the noise level is unknown. We refer to \cref{fig:auto_perf} for visual evidence.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.35\textwidth]{figure/sims_plot_mednoise_format.pdf}
    \includegraphics[width=0.35\textwidth]{figure/sims_plot_highnoise_format.pdf}
    \caption{\tbf{Synthetic data experiments.} The data on the left has high signal-to-noise ratio, whereas the data on the right has low signal-to-noise ratio. See \cref{app:synthetic_gen} for details on the data generating process. Each point corresponds to the mean absolute error ± 1 standard error across 30 trials.}
    \label{fig:auto_perf}
\end{figure}

\newcommand{\colsize}{N_{1, \eta_2}^{\mrm{col}}}
\newcommand{\rowsize}{N_{1, \eta_1}^{\mrm{row}}}

==> eurips2025/nn-overview.tex <==
\section{Nearest Neighbors for Matrix Completion}\label{sec:nn-overview}


% \kc{Start with a table as in page 2 of \href{https://arxiv.org/pdf/2404.12290}{link}. Then refer to the specific algorithms within the table~(with appropriate references). Then present 4 modules: distance calculation, averaging, subraction, weighting. Start with the abstract modules and specify. For DNN, add as a specific in the row-wise NN. All the settings compress. Need to cut it by page 4. }

% \kc{(2 pages)}

We now introduce the mathematical model for matrix completion:
% \kc{$\dist{i, t}$ to additive noise model.}
\begin{align}
\qtext{for} i \in [N], t\in[T]:\\ \measurement{i, t}  :=
     \begin{cases}
        \sample{1}(i, t), ..., \sample{n}(i, t) \ \sim \ \dist{i, t}&\qtext{if} \missing{i, t}=1, \\
        \mrm{unknown}&\qtext{if} \missing{i, t}=0.
    \end{cases}
    \label{eq:model}
\end{align}
In other words, for matrix entries where $\missing{i, t} = 1$, we observe $n$ measurements $\measurement{i, t}$ that takes value $\sample{i, t}$ realized from distribution $\dist{i, t}$. When $n = 1$, i.e., $\measurement{i,t} = \sample{1}(i, t)$, we refer to \cref{eq:model} as the \textit{scalar matrix completion} model; scalar matrix completion is the most common problem posed in the literature~\cite{candes2012exact,recht2011simpler,koren2009matrix,hastie2015matrix,chatterjee2015matrix,dwivedi2022counterfactual,dwivedi2022doubly,agarwal2023causal}, where the goal is to learn the mean of the underlying distributions $\sbraces{ \meanparam{i, t} = \int x d\dist{i, t}(x)}_{i \in [N],t \in [T]}.$ When there are more than one observed measurements per entry, i.e., $\measurement{i, t} = [\sample{1}(i, t), ..., \sample{n}(i, t)]$ for $n \geq 2$, we refer to \cref{eq:model} as the \textit{distributional matrix completion} problem, the goal being the recovery of the distributions as a whole.
%
We refer the readers to \cref{app:guarantees} for a detailed discussion on the structural assumptions imposed on the model \cref{eq:model}.

==> eurips2025/prop99.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figure/CA-synthetic-control.pdf} \\
    (a) Synthetic controls for California in post-intervention period \\
    \includegraphics[width=0.47\textwidth]{figure/sc_est_errors_boxplot.pdf} \\
    (b) Absolute error on control states
    \caption{\tbf{Nearest neighbor methods generate high-fidelity synthetic controls in counterfactual inference for panel data.} 
    % \rd{Are we trying to promote synthetic control? We should label it as SC. Also all colors in the left side is not easy.}
    % \ag{Todo: get rid of vertical grid lines in left plot; add ``Cigarette consumption (packs per capita)'' to y-axis on right figure; add line segments from label to line}
    }
    \label{fig:prop99}
\end{figure}

% \cite{cdcStateTobacco}
Next we consider a panel data setting, where our goal is to estimate the effect of the California Tobacco Tax and Health Protection Act of 1988 (a.k.a. Proposition 99) on annual state-level cigarette consumption\footnote{measured as per capita cigarette sales in packs}.
By definition, the counterfactual cigarette consumption in California---had Proposition 99 never been enacted---is not observed. 
\cite{abadie2010synthetic} introduce the notion of a ``synthetic control'' to serve as a proxy for this unobserved value based on ``neighboring'' \emph{control states} that never instituted a tobacco tax. These states are not close in a geographical sense, but rather close due to similarities in other covariates\footnote{GDP per capita, beer consumption, percent aged 15–24, and cigarette retail prices}. 
% See also: \cite{abadie2003economic}
We take a different approach and use only the observed cigarette consumption levels from the control states, of which there are 38 in total. Thus, we frame our problem as a scalar matrix completion problem with $N=39$ and $T=31$ (see \cref{eq:model}). The last row in the matrix corresponds to the state of California. 
% \ag{Mention that the staggered adoption missingness pattern, which falls under MNAR \cref{app:missingness} makes the estimation problem challenging.}
% We only observe measurements for California in the pre-intervention period (before 1989). 
% Thus, the missingness pattern is known as \emph{staggered adoption} \todo{cite}.
% Variants of nearest neighbors were adopted to construct synthetic controls to account for potentially existing unobserved confounders~\cite{agarwal2023causal}.

\paragraph{Results \& Discussion.}
% Whereas \cref{sub:hs} saw how nearest neighbor methods can effectively estimate counterfactual quantities for personalized treatments, 
For each method, we use a 64-16-20 train-validation-test split and use cross validation to fit any hyperparameters. \cref{fig:prop99} plots the various synthetic controls for California (left) and absolute error of each method on the 38 control states, for which we do observe the no-treatment values (right).
From \cref{fig:prop99}(a), we see that nearest neighbor methods, in particular $\tsnn$ and $\rownn$, are roughly on par with the gold-standard synthetic control method of \cite{abadie2010synthetic} (``SC'') for estimating California's counterfactual cigarette consumption in the post-intervention period (after 1989). This is despite the fact that the nearest neighbor methods rely on less information for the estimation task.
From \cref{fig:prop99}(b), we see that all nearest neighbor methods, with the exception of $\colnn$, achieve similar error levels as the synthetic control baseline. $\rownn$ achieves even lower error levels.
See supplementary experiment details in \cref{app:prop99}.

==> eurips2025/struct_app.tex <==
\section{Class Structure Details}\label{app:class_struct}

The core functionality of \lib{} is based on two abstract classes: \texttt{EstimationMethod} and \texttt{DataType}.

\texttt{EstimationMethod} classes contain the logic to impute a missing entry such as how to use calculated distances. 
% In the context of the modules in \cref{sec:nn-overview}, this class determines the weighting function or, in the context of $\drnn$ and $\autonn$, how to compose estimates. 
We separate this from the \texttt{DataType} abstraction because several estimation methods can be used for multiple data types. For example, \texttt{RowRowEstimator} implements the $\rownn$ procedure for any data type given to it, such as scalars or distributions.

% \texttt{DataType} classes implement the $\distancemod$ and $\averagemod$ modules for any kind of data type (e.g. scalars which use squared distance and simple averaging). 
\texttt{DataType} classes implement a \emph{distance} and \emph{average} function for any kind of data type. For scalars we use squared distance and simple averaging. For distributions, we implement two metrics, Wasserstein ($\wassersteinnn$) and kernel maximum mean discrepancy (MMD, $\kernelnn$). This abstract class allows for our package to extend to any data types beyond the ones we tested. For instance, a practitioner can easily add a \texttt{DataType} for text strings which uses vector embeddings to find distances and averages between between strings without needing to rewrite any of the estimation procedure.

==> icml2025/case-study.tex <==
\section{\lib{}-Bench and Results}\label{sec:case-study}

In this section, we evaluate several nearest neighbor algorithms provided by our library, \lib{}, on real-world data. As part of our package, we include data loaders which automatically download the necessary datasets and format them for evaluation. These datasets and loaders comprise our proposed benchmark for nearest neighbor matrix completion algorithms, \lib{}-\textbf{Bench}. We also test several existing popular matrix completion techniques~\cite{hastie2015matrix,chatterjee2015matrix}. For details on our experimental setup, computing hardware, and boxplot generation, see \cref{app:case-studies}.


% ----------------
\iffalse
\subsection{Synthetic data}
\label{sub:simulations}


We first compare different matrix completion techniques on a synthetically generated data set. Our goal is to track the performance of different algorithms as the matrix size scales. We generate data matrix of size $N \times T$, where measurements $\measurement{i, t}$~(when $\missing{i, t} = 1$) are generated from distribution $\mu_{i, t} = \theta_{i, t} + \varepsilon_{i, t}$ where $\varepsilon_{i, t}$ are exogenous and i.i.d. centered Normal random variables. For more specifics on the data generation, see \cref{app:synthetic_gen}. The task here is to
\fi

% our synthetic data matrices with $d$-dimensional row latent factors $\uset := \{u_i, i\in[N]\}$, and column latent factors $\vset := \{v_t, t\in[T]\}$. For the following experiments, we let ${u_i \sim \text{Unif}[-0.5, 0.5]}$ for all $i \in [N]$ and ${v_t \sim \text{Unif}[-0.5, 0.5]}$ for all $t \in [T]$. 

% ----------------
\subsection{Personalized healthcare: HeartSteps}
\label{sub:hs}

% \paragraph{Case-study introduction}

The HeartSteps V1 study~(HeartSteps study for short) is a clinical trial designed to measure the efficacy of the HeartSteps mobile application for encouraging non-sedentary activity \cite{klasnja2019efficacy}. The HeartSteps V1 data and its subsequent extensions have been widely used for benchmarking a variety of tasks including counterfactual inference of treatment effect \cite{dwivedi2022counterfactual, choi2024learning}, reinforcement learning for intervention selection \cite{liao2019rlheartsteps}, and micro-randomized trial design \cite{qian2022microrandomized}. In the HeartSteps study, $N = 37$ participants were under a 6-week period micro-randomized trial, where they were provided with a mobile application and an activity tracker. Participants independently received a notification with probability $p = 0.6$ for $5$ pre-determined decision points per day for 40 days~($T = 200$). We denote observed entries $Z_{i, t}$ as the mean participant step count for one hour after a notification was sent and unobserved entries as the unknown step count for decision points where no notification was sent. Our task is to estimate the counterfactual outcomes: the participant's step count should they have received a different treatment (notification or no notification) than they did at specific time points during the study. 
% By computing the counterfactual outcome, we can also estimate the treatment effect of an intervention on an individual.
 

% Thus, the treatment application~(notification sent) is subject to an an individual's latent characteristics such as their personal schedule and daily routines. 

%availability of individuals encoded in the randomized trial implies that treatment application~(notification sent)

%Further, as notification are never sent during non-available times, positivity is clearly violated in this example.    % random given that they are available, positivity is violated as unavailable times has 0.0 probability 


% We proceed on our empirical analysis by imposing the potential outcome observation model \cref{mod:potential-outcome} on the HeartSteps data. 


\paragraph{Results \& Discussion.} We benchmark the performance of the matrix completion methods by measuring absolute error on held-out observed step counts across 10 participants in the last 50 decision points. We use the remaining data to find nearest neighbor hyperparameters using cross-validation. To benchmark distributional nearest neighbors methods ($\kernelnn$ and $\wassersteinnn$) against the scalar methods, we first set each entry to have the number of samples $n = 60$, where each sample is the 1 minute step count before imputation. Then, we take the mean of the imputed empirical distribution as the estimate. 

In \cref{fig:hs-results}(a), we compare the absolute error of the imputed values across the nearest neighbor and baseline methods. The scalar nearest neighbor methods far out-perform USVT and are on par with SoftImpute. The two distributional nearest neighbor methods far outperform all methods operating in the scalar setting; it suggests that matching by distributions collect more homogeneous neighbors, thereby decreases the bias of the method, compared to matching only the first moments as done in most scalar matrix nearest neighbor methods. 

% which suggests that finding neighbors using a distributional distance can enhance the quality of the neighbors and reduce the bias of the estimate. 

In \cref{fig:hs-results} panel (b), we show an example of an imputed entry in the distributional nearest neighbors setting. In this case, the ground truth distribution is bimodal, as the participant was largely sedentary (0 steps) with small amounts of activity. While both $\kernelnn$ and $\wassersteinnn$ capture the sedentary behavior of the participant, $\kernelnn$ is able to recover the bimodality of the original distribution whereas $\wassersteinnn$ cannot. 


% \begin{wrapfigure}{R}{0.5\textwidth}
%     \begin{center}        \includegraphics{figure/hs_est_errors_boxplot.pdf}
%     \end{center}
%     \caption{\tbf{HeartSteps V1: Estimation error under notification sent.} We apply log-transform to the raw step counts before imputing.}
%     \label{fig:hs-results}
% \end{wrapfigure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{figure/hs_est_errors_boxplot.pdf}\\
    \includegraphics[width=0.47\textwidth]{figure/hs_est_errors_boxplot.pdf}\\
    (a) Absolute error of mean step count prediction\\
    \includegraphics[width=0.33\textwidth]{figure/hs_distplot_48.pdf} \\
    (b) $\kernelnn$ vs. $\wassersteinnn$
    \caption{\tbf{HeartSteps: estimating step count under scalar and distributional matrix completion settings.} Panel (a) shows the absolute error of predicted step count of the nearest neighbor methods against matrix completion baselines (SoftImpute, USVT). Panel (b) shows an example of an imputed entry in the distributional matrix completion setting.
    }
    \label{fig:hs-results}
\end{figure}
% ----------------

\subsection{Movie recommendations: MovieLens}\label{sec:movielens}
\begin{figure}
    \begin{center}        \includegraphics{figure/movielens_est_errors_boxplot.pdf}
    \end{center}
    \caption{\tbf{MovieLens: Estimation error for a random subsample of size 500.} For experimental settings and discussion see \cref{sec:movielens}.}
    \label{fig:movielens-error}
\end{figure}

The MovieLens 1M dataset \cite{movielens} contains 1 million ratings (1–5 stars) from 6,040 users on 3,952 movies. Collaborative filtering on MovieLens has long been a benchmark for matrix-completion methods: neighborhood-based algorithms~\cite{sarwar2001item}, latent-factor models~\cite{koren2009matrix}, and, more recently, nearest neighbors interpreted as blind regression under a latent–variable model~\cite{li2019nearest}. These assist practitioners in data-driven recommendation systems, since more accurate rating imputation directly drives better personalized suggestions and user engagement. This is a standard scalar matrix completion problem with $N=6,040$ and $T=3,952$. Each rating is an integer in $\{1,\dots,5\}$. The dataset has a very high percentage of missing values: 95.53\% missing. Our task is to estimate unobserved ratings using various matrix completion algorithms. We benchmark the performance of nearest neighbors against matrix factorization by measuring absolute error on held‑out ratings. See \cref{app:movielens} for additional details on the dataset.

\paragraph{Results \& Discussion.} We fit the nearest neighbor methods using a random sample of size 100 from the first 80\% of the dataset to choose nearest neighbor hyperparameters via cross-validation.We then test the method on a random subsample of size 500 from the last 20\% of the dataset. As observed in \cref{fig:movielens-error}, all nearest neighbor methods have a lower average error than USVT and a much lower standard deviation of errors, with $\colnn$, $\rownn$, $\drnn$, and $\autonn$ performing the best out of the nearest neighbor methods. SoftImpute performs on par with the nearest neighbor methods. Note that the nearest neighbor methods perform well even while only being trained on a tiny subset of the data of size 100 out of the 1 million ratings available.


% ----------------
% \input{icml2025/llm_evaluation_new}
% \input{icml2025/llm_evaluation}

==> icml2025/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our main claims in our abstract are a unified framework, a unified Python package, and a new test bench for nearest neighbor-based matrix completion methods. We present our unified framework for nearest neighbor-based matrix completion methods in \cref{sec:unified-view}. We present our package structure in \cref{sec:library}. Finally, we describe the new test bench in \cref{sec:case-study}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss improvements to our Python package in \cref{sec:conclusion}. The algorithms described in \cref{sec:nn-overview} use theoretical assumptions for their theoretical guarantees, but these assumptions do not affect the algorithms themselves, and thus pose no limitations on our Python package or test bench.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not claim any theoretical results in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All of our results can be reproduced with the code on our GitHub, which is (anonymously) linked in the paper. Each experiment has its own folder with instructions on how to run the experiments. We provide Python files which automatically download the necessary data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide an anonymous GitHub link to our open-source code. Every experiment can be reproduced with the Python files we provide separately from our Package source files. The new Python package we present, also in the GitHub link, can be installed quickly on standard computing hardware and do not require access to GPU's or any other specialized hardware.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For each experimental setup, we describe how we split up the datasets into train and test sets. We describe in detail how our hyperparameters are chosen in the Appendix. We also provide the code we use to choose hyperparameters in our open-source repository.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe how we generate our boxplots to compare error across methods in \cref{app:case-studies}. We also detail how our error bars are generated in our figures in the respective figures which have error bars.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe our computing setup in \cref{app:case-studies}. It is standard laptop hardware.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our research conforms with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work does not have any direct societal impact. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our new Python package and test bench do not pose a significant risk for misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Every library and dataset used in this work is properly cited and credited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work primarily releases a new code library that we have placed under the MIT License.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve any work with human subjects nor crowdsourcing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include any human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper's proposed algorithms do not involve LLM's in an important way.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> icml2025/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

In this paper, we present a unified framework, Python library (\lib{}), and test bench (\lib{}-\textbf{Bench}) for nearest neighbor-based matrix completion algorithms. We demonstrate how our library supports a diverse set of datasets spanning patient-level healthcare causal inference (HeartSteps) and recommendation systems (MovieLens). 
% See the appendix for  counterfactual inference for panel data (Proposition 99), and LLM evaluation (PromptEval). 
Our framework and library facilitate researchers and practitioners to easily try different NN methods on their dataset of choice as well as extend the library to more complex methods.

In future work, we plan on speeding up the runtime of \lib{}, particularly for commonly used settings such as scalars-valued matrices. We also plan on adding support for distributed datasets too large to fit into memory. Finally, we plan on extending the library to other nearest neighbor algorithms, such as approximate nearest neighbors methods and ones that use linear regression instead of simple averaging.

% \ag{Future work: (1) speeding up, (2) bringing together approximate nearest neighbors (find references from supervised learning literature: \url{https://scholar.google.com/citations?user=9r7_pN8AAAAJ&hl=en})}

==> icml2025/intro.tex <==
\section{Introduction}

Nearest neighbor methods are a class of non-parametric algorithms widely used for regression, classification and pattern recognition. Due to their scalability and success under models with minimal assumptions, nearest neighbor methods have recently been adopted for practical fields such as matrix completion and counterfactual inference in panel data settings. Matrix completion is a well-established field that supplies practitioners with many tools to recover underlying matrices using partial or even noisy observations~\cite{hastie2015matrix,chatterjee2015matrix,keshavan2010matrix}, with recommendation systems~\cite{koren2009matrix,recht2011simpler} as an important use-case. Panel data counterfactual inference aims at learning the treatment effect of policies across time~\cite{bai2009panel,bai2021matrix,athey2021matrix}. One important example is individualized healthcare predictions~\cite{klasnja2019efficacy}. Nearest neighbor methods were recently recognized as effective in providing granular inference guarantees for both matrix completion and counterfactual inference when either the missingness or the policy treatment are not completely random and confounded~\cite{ma2019missing,dwivedi2022counterfactual,agarwal2023causal}. 

% because they have bee?n shown to be competitive in terms of accuracy, can impute entry-wise, and are widely used in practice.


% Data scientists looking to use matrix completion to impute missing data have a diverse set of tools at their disposal including spectral based methods~\cite{hastie2015matrix,chatterjee2015matrix}, gradient methods (\cite{keshavan2010matrix}), 

% and nearest neighbor methods~\cite{li2019nearest,dwivedi2022counterfactual,agarwal2023causal,choi2024learning,feitelberg2024distributional}. 

Despite nearest neighbor methods popularity, there is no unified package that lets a user easily switch between different kinds of nearest neighbor algorithms for matrix completion and counterfactual inference. In this paper, we present a package~(\href{https://github.com/aashish-khub/NearestNeighbors}{GitHub link: \lib{}}) to unify several nearest neighbor methods under a single interface, so users can easily choose the method that suits their data the best. 
% Next, we review two broad applications of nearest neighbors and matrix completion: recommendation systems and panel data settings.

% \paragraph{Recommendation systems} In the problem of a recommendation system, multiple users submit ratings / preferences for a subset of items, and the vendor recommends items based on the partial rating information \cite{rennie2005fast}. Prediction of unseen ratings is the key to a good recommendation, and the predictions are based on the patterns of the partially observed ratings which can be formalized into a matrix completion problem. A popular instance is the Netflix problem, an open competition for the best prediction algorithm of user ratings of films. Users~(rows of matrix) have the option to rate the films~(columns of matrix). However, users typically rate only a subset of films, and the ratings are commonly biased towards their preferences. Under the common belief that only a few factors drive the preference and ratings of the users, many matrix completion algorithms have resorted to the low rank assumption on the ratings matrix~\cite{recht2011simpler,candes2012exact}. Variants of nearest neighbors~(in short, $\nn$) recently were introduced to correct for the potential bias originating from the fact that observation patterns are influenced by the matrix entries~(e.g. ratings) themselves and by unmeasured confounders~\cite{agarwal2023causal,abadie2024doubly}. 

% \paragraph{Panel data} Panel data constitutes measurements of multiple units that are tracked over time~(hence a type of longitudinal data) as they undergo different types of interventions at different times~\cite{bai2009panel}. Panel data is used to analyze the causal effects of any policies, treatments, or business decisions that affect the subjects in the data, making this data type essential in econometrics and health studies. Matrix completion algorithms enable estimation of these causal effects at the unit$\times$time level, the most granular scale where causal effects can be estimated~\cite{athey2021matrix,agarwal2023causal}. For example, consider a mobile health app trying to learn the effectiveness of two exercise routines. Suppose the app alternates two routines across $N$ different users repeatedly over $T$ weeks, where their health activities~(say physical step counts) throughout each week are recorded. Then, we can use matrix completion to impute the counterfactual step counts under treatment and control, allowing us to estimate causal effects at the most granular scale.

\subsection{Our contributions}

\newcommand{\starnn}{\mathsf{StarNN}}
\newcommand{\autonn}{\mathsf{AutoNN}}

Overall, our contributions in this paper are summarized below: 
% \kc{if we are not using (C1)... later in the paper, maybe consider using simple dots?}
% \begin{enumerate}[label=(C\arabic*)]
\begin{enumerate}
    \item We provide a unified, easy to implement nearest neighbor library that contains a breadth of nearest neighbor algorithms for matrix completion problems.
    \item We present a unified framework for nearest neighbor algorithms that facilitates extending to new variants.
    % \item We introduce a new nearest neighbors algorithm, auto nearest neighbors~(in short $\autonn$), which aims both to improve on the existing methods and demonstrate the ease of developing new variants with our library.
    \item We demonstrate our library's wide applicability through several real-world data sets in a new test bench called \lib{}\textbf{-Bench}.
\end{enumerate}

\subsection{Related work}
We contextualize our contributions in the context of both nearest neighbors as a general algorithm and matrix completion specifically.

\paragraph{Nearest neighbors}

As introduced above, nearest neighbor methods are widely used for non-parametric regression, classification, and pattern recognition~\cite{cover1967nearest,cannings2020local}. Recently, nearest neighbor methods were introduced as an effective algorithm for matrix completion problems~\cite{li2019nearest,agarwal2023causal,dwivedi2022counterfactual}, especially when the missingness depended on observations and unobserved confounders. The fact that nearest neighbor methods target a single entry at a time via matching makes it effective against various types of missing patterns. The class of algorithms has grown to account for a wide range of applications~\cite{dwivedi2022doubly,choi2024learning,feitelberg2024distributional,sadhukhan2024adaptivity, sadhukhan2025adaptivelyweightednearestneighborsmatrix}, with a focus on inference for personalized treatment effects in the causal inference literature. Our library, \lib{}, is designed to easily implement the vanilla versions of nearest neighbors~\cite{li2019nearest,dwivedi2022counterfactual} as well as its unweighted~\cite{dwivedi2022doubly,sadhukhan2024adaptivity} and weighted~\cite{sadhukhan2025adaptivelyweightednearestneighborsmatrix} variants. Finally, \lib{} is also capable of distributional matrix completion~\cite{choi2024learning,feitelberg2024distributional}.

\paragraph{Other matrix completion methods}

% \kc{@ MP, TS: Let's make this less notation heavy, more comprehensive citations, include soft-impute~\cite{hastie2015matrix} as it is one of our benchmarks.} 

Universal singular value thresholding (USVT), proposed in \cite{chatterjee2015matrix,bhattacharya2022matrix}, is a classical spectral-based method for performing matrix completion; its core functionality is based on a singular value decomposition of the matrix and thresholding the singular values.
%
SoftImpute, introduced by \cite{hastie2015matrix}, is another widely used optimization-based algorithm for matrix completion. The algorithm computes ridge-regression updates of the low-rank factors iteratively and finally soft-thresholds the singular values to impose a nuclear norm penalty. 
%
Notably USVT and SoftImpute have provable guarantees when missingness is completely at random, but empirically fail when the missing pattern depends on the observed entries or the unobserved confounders~\cite{agarwal2023causal}. Our real-world analysis in \cref{sec:case-study} once again demonstrates this point.

% The USVT algorithm completes a matrix by imputing zero for all the missing entries of the matrix, obtaining a estimate $\widehat p$ of the observation probability, performing a singular value decomposition of the imputed matrix, and retaining only those singular values that exceed $\tau \sqrt{\min\{N, T\}}$ (where $\tau > 2 \widehat p$). 

% \cite{chatterjee2015matrix} shows that the proposed algorithm attains minimax optimal performance when estimating matrices constrained by a bounded nuclear norm. 

\paragraph{Existing software for matrix completion and nearest neighbors}

Scikit-Learn \cite{scikit-learn}, a popular Python package for machine learning tools, implements a simple k-nearest neighbor algorithm for imputing missing values in a feature matrix. However, their implementation is designed for the feature matrix setting. So, neighbors are only defined across samples (row-wise). Additionally, they do not provide any implementation for more advanced nearest neighbor algorithms, nor does their package allow for easy extendability like our proposed package. 
% Another package which implements nearest neighbors for matrix completion is the Synthetic Nearest Neighbors (SNN) package (\url{https://github.com/deshen24/syntheticNN}). SNN implements a specific nearest neighbor algorithm for the causal matrix completion setting. 

\paragraph{Organization}

\cref{sec:nn-overview} contains an overview of the existing nearest neighbor algorithms implemented in our library, \lib{}. 
% \cref{sec:new-nn} introduces a new nearest neighbor algorithm, $\autonn$, that is also implemented in \lib{}. 
\cref{sec:library} touches upon the high-level (class) structure of \lib{}, as well as the interface for practitioners. \cref{sec:case-study} tests different variants of nearest neighbor methods and classical methods on our new test bench of diverse datasets called \lib{}-\textbf{Bench}. Finally, in \cref{sec:conclusion}, we provide concluding remarks and outline future directions of research.








==> icml2025/llm_evaluation.tex <==
\subsection{Efficient LLM evaluation}

Recent works show there is non-trivial variability of performance of language models across different prompting techniques\cite{sclar2023quantifying,polo2024efficient}, a natural follow up task being identification of the best performing prompting templates for certain tasks and language models~\cite{shi2024best,polo2024efficient}. The difficulty here is that there are near infinite ways of prompting, so an efficient evaluation framework has been investigated thoroughly~\cite{ye2023predictable,perlitz2023efficient}. Motivated by \cite{polo2024efficient}, we use the MMLU dataset~\cite{hendrycks2020measuring} and empirically demonstrate that our nearest neighbors method can achieve efficient evaluation. Under a fixed task~(e.g. abstract algebra, political science) various questions / examples are queried to a specific model, where each questions are restructured using different prompting templates. Either the model answers the question correctly or not and correctness is recorded. 

\paragraph{Results \& Discussion}

\kc{Do both SNN and DNN}

There are $57$ tasks and $15$ models total; the number of questions / examples depend on the task of interest and there is a fixed set of $100$ prompting templates that is applied to whatever question of whatever task. \kc{Could make a sub-section that explains MMLU.}


We consider a distributional matrix completion setup and implement a Dist-NN to estimate the distribution of averaged scores across templates~(template instances are of no value, as we aim to learn the overall variation) leveraging information across different models and different tasks. Imputation in \cite{polo2024efficient} was done while fixing model and task, so the commonalities that may exist across different models and tasks were not utilized.




% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figure/template_subject_model_by_propensity.pdf}
%     \caption{\kc{Figure needs adjustment, will not include boxplots of MMD errors for Kernel NN as most of them are zero---Wasserstein NN might have meaningful boxplots.} p = , standardize X }
%     \label{fig:temp_sub_model}
% \end{figure}



==> icml2025/llm_evaluation_new.tex <==
\subsection{Efficient LLM evaluation: PromptEval}
\label{sub:llm}

% \begin{wrapfigure}{R}{0.5\textwidth}
%     \begin{center}
%     \includegraphics{figure/prompteval_est_errors_boxplot-p0.5.pdf}
%     \end{center}
%     \caption{\tbf{Kolmogorov-Smirnov distance with missingness at 50\%.} $\mmd$ using column-wise nearest neighbors performs the best in terms of the KS distance.}
%     \label{fig:ks}
% \end{wrapfigure}

The rapid advancement of LLMs have placed them at the center of many modern machine learning systems, from chatbots to aids in medical education \cite{geathers2025benchmarking}. In practice, system architects want to strike the right balance of real-world performance and cost, but navigating this Pareto frontier is a daunting task. 2024 alone saw at least 10 new models from Anthropic, Google, Meta, and OpenAI, not even counting the multitude of open-source fine-tuned models built on top of these.
% (Moreover, this number is likely to only grow as training models becomes more accessible, thanks in part to DeepSeek R1.) 
On specific tasks, smaller, fine-tuned models may even outperform the latest frontier models, in addition to being more cost effective.

We investigate how matrix completion, specifically nearest neighbor methods, can alleviate some of these burdens. We use the PromptEval dataset \cite{polo2024efficient}, which evaluates $15$ open-source language models (ranging in size from 3B to 70B parameters) and $100$ different prompting techniques across the 57 tasks of the MMLU benchmark \citep{hendrycks2020measuring}. In practice, the performance of a model depends---sometimes dramatically---on the precise input prompt. This suggests that we need to consider the performance of a model across a wide range of prompts, rather than any one prompt in particular. 
Thus, we model this problem as a distributional matrix completion problem with $N=15$, $T=57$, and $n=100$.
Given one of 57 tasks, we aim to accurately characterize the performance of each model without resorting to exhaustive evaluation.
Nearest neighbors leverage commonalities across models and tasks to estimate the performance distribution of each entry, which was otherwise not considered in \cite{polo2024efficient}; previous literature achieves efficient evaluation per model and task in isolation without leveraging any across model / task information. 

% \rd{We have to explain why this method is better here.}

% Scalar matrix completion is one approach to achieving such parsimony. In the language of matrix completion, we define the rows to be model-prompt pairs and the columns to be MMLU questions (14,079 in total).
% \ag{probably have to explain what a prompt is}
% Widely used to evaluate frontier LLMs, MMLU comprises $57$ tasks (e.g. abstract algebra, political science) \ag{insert the total number of questions} totally $14079$ questions in the test set.
% Each task is associated with varying questions, each associated with a ground-truth answer. 
% When faced with identifying the best prompting technique, considering all combinations of (1) model, (2) prompting technique, and (3) task is not only expensive, but also highly wasteful \cite{shi2024best,polo2024efficient}. 
% Nearest neighbor methods enable a cheap way to identify the best prompt.
% \citet{sclar2023quantifying,polo2024efficient} show that different prompting techniques lead to widely different results.
% \paragraph{Speeding up best prompt identification.}
% For a given a model, our first problem is to estimate the fitness of a prompting technique on a particular task. Note that each MMLU task is associated with a set of question (ranging in size from 100 to ???).
% We then randomly include each entry of the matrix independently with probability $p$ and estimate the missing entries.
% For each model, task, and prompt combination, we aggregate the scores (both observed and estimated) to obtain a value between 0 and 1. We then apply further aggregation to obtain a distribution for each model-task pair.
% \cref{tab:llm_scalar} shows the Kolmogorov statistic between the estimated and ground-truth distributions.
% In principle, standard matrix completition methods like USVT are well-suited for MCAR settings like the one considered here, yet nearest neighbor methods still perform the best empirically.
% Nearest neighbor methods are able to leverage commonalities across questions and prompts to estimate missing entries.

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=0.47\textwidth]{figure/ksbyp_prompteval_plot.pdf} 
        &  
        \includegraphics[width=0.45\textwidth]{figure/distributions-entry40-tp4.0.pdf} 
        \\
        (a) Mean KS distance between estimated and
        &
        (b) $\kernelnn$ vs. $\wassersteinnn$ \\
         ground-truth distributions
    \end{tabular}
    \caption{\textbf{Distributional nearest neighbor methods enable efficient LLM evaluation on MMLU.} We estimate LLM score distributions across all models and tasks given only a limited number of model-task evaluations, determined by the propensity $p$. See \cref{sub:llm} for a detailed discussion.}
    \label{fig:llm}
\end{figure}

\paragraph{Results \& Discussion.}
We randomly include each entry in the matrix independently with probability $p\in \braces{0.3,0.5,0.7}$ and impute the missing entries using the $\kernelnn$ and $\wassersteinnn$ methods of \cref{tab:summary}. For each method, we consider both the the row-wise and column-wise variants.
\cref{fig:llm}(a) reports the mean Kolmogorov-Smirnov (KS) distance between the imputed and ground-truth distributions across the entries in the test set for varying missingness values. As expected, estimation error decreases as $p$ increases.
% the number of observed entries increases. 
% versus the ground truth at varying levels of $p$ for a select entry in the matrix. At $p=0.3$, we avoid 70\% of LLM evaluations, yet still recover the distribution of prompt scores with reasonable quality. At $p=0.5$ and $p=0.7$, column-wise NN with $\mmd$ performs the best.
\cref{fig:llm}(b) visualizes the imputed distributions using row-wise $\kernelnn$ and column-wise $\wassersteinnn$ (at $p=0.7$) for a select entry, along with the ground-truth distribution. Even with 30\% of matrix entries missing, distributional NN methods are able to recover the underlying distribution.

% To further reduce estimation error, we look to exploit commonalities across the models.
% We consider a distributional matrix completion setup and implement a Dist-NN to estimate the distribution of averaged scores across templates~(template instances are of no value, as we aim to learn the overall variation) leveraging information across different models and different tasks. 
% Imputation in \cite{polo2024efficient} was done while fixing model and task, so the commonalities that may exist across different models and tasks were not utilized.

% \ag{Maybe we should also include baseline from PromptEval for the distributional setting? That will make this section even stronger I think.}


% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figure/template_subject_model_by_propensity.pdf}
%     \caption{\kc{Figure needs adjustment, will not include boxplots of MMD errors for Kernel NN as most of them are zero---Wasserstein NN might have meaningful boxplots.} p = , standardize X }
%     \label{fig:temp_sub_model}
% \end{figure}



==> icml2025/nn-new.tex <==
\subsection{New variant: Auto nearest neighbors}\label{sec:new-nn}

$\tsnn$ is a generalization of $\rownn$ and $\colnn$ by setting one of the tuning parameters to zero~(see \cref{tab:summary}), whereas the idea underlying $\drnn$ is fundamentally different from that of $\tsnn$; $\drnn$ debiases a naive combination of $\rownn$ and $\colnn$ whereas $\tsnn$ simply boosts the number of measurements averaged upon, thereby gaining from lower variance. 
So we simply interpolate the two methods for some hyper-parameter $\alpha \in [0, 1]$; see \cref{tab:summary}.
Notably the hyper-parameter $\tuning$ for both $\drnn$ and $\tsnn$ are identical when interpolated.

Suppose $\dist{i, t} = \theta_{i, t} + \varepsilon_{i, t}$ in \cref{eq:model} where $\varepsilon_{i, t}$ are centered i.i.d. sub-Gaussian distributions across $i $ and $t$.
% \rd{why do we need Gaussian noise?}. 
When $\sigma$ is large in magnitude, $\tsnn$ denoises the estimate by averaging over more samples, hence providing a superior performance compared to $\drnn$ in a noisy scenario. When $\sigma$ is small so that bias of nearest neighbor is more prominent, $\drnn$ effectively debiases the estimate so as to provide a superior performance compared to $\tsnn$. The linear interpolator $\autonn$ \textit{automatically} adjusts to the underlying noise level and debiases or denoises accordingly; such property is critical when applying nearest neighbors to real world data set where the noise level is unknown. We refer to \cref{fig:auto_perf} for visual evidence.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.35\textwidth]{figure/sims_plot_mednoise_format.pdf}
    \includegraphics[width=0.35\textwidth]{figure/sims_plot_highnoise_format.pdf}
    \caption{\tbf{Synthetic data experiments.} The data on the left has high signal-to-noise ratio, whereas the data on the right has low signal-to-noise ratio. See \cref{app:synthetic_gen} for details on the data generating process. Each point corresponds to the mean absolute error ± 1 standard error across 30 trials.}
    \label{fig:auto_perf}
\end{figure}

\newcommand{\colsize}{N_{1, \eta_2}^{\mrm{col}}}
\newcommand{\rowsize}{N_{1, \eta_1}^{\mrm{row}}}

==> icml2025/nn-overview.tex <==
\section{Nearest Neighbors for Matrix Completion}\label{sec:nn-overview}


% \kc{Start with a table as in page 2 of \href{https://arxiv.org/pdf/2404.12290}{link}. Then refer to the specific algorithms within the table~(with appropriate references). Then present 4 modules: distance calculation, averaging, subraction, weighting. Start with the abstract modules and specify. For DNN, add as a specific in the row-wise NN. All the settings compress. Need to cut it by page 4. }

% \kc{(2 pages)}

We now introduce the mathematical model for matrix completion:
% \kc{$\dist{i, t}$ to additive noise model.}
\begin{align}
\qtext{for} i \in [N], t\in[T]:\\ \measurement{i, t}  :=
     \begin{cases}
        \sample{1}(i, t), ..., \sample{n}(i, t) \ \sim \ \dist{i, t}&\qtext{if} \missing{i, t}=1, \\
        \mrm{unknown}&\qtext{if} \missing{i, t}=0.
    \end{cases}
    \label{eq:model}
\end{align}
In other words, for matrix entries where $\missing{i, t} = 1$, we observe $n$ measurements $\measurement{i, t}$ that takes value $\sample{i, t}$ realized from distribution $\dist{i, t}$. When $n = 1$, i.e., $\measurement{i,t} = \sample{1}(i, t)$, we refer to \cref{eq:model} as the \textit{scalar matrix completion} model; scalar matrix completion is the most common problem posed in the literature~\cite{candes2012exact,recht2011simpler,koren2009matrix,hastie2015matrix,chatterjee2015matrix,dwivedi2022counterfactual,dwivedi2022doubly,agarwal2023causal}, where the goal is to learn the mean of the underlying distributions $\sbraces{ \meanparam{i, t} = \int x d\dist{i, t}(x)}_{i \in [N],t \in [T]}.$ When there are more than one observed measurements per entry, i.e., $\measurement{i, t} = [\sample{1}(i, t), ..., \sample{n}(i, t)]$ for $n \geq 2$, we refer to \cref{eq:model} as the \textit{distributional matrix completion} problem, the goal being the recovery of the distributions as a whole.
%
We refer the readers to \cref{app:guarantees} for a detailed discussion on the structural assumptions imposed on the model \cref{eq:model}.

==> icml2025/prop99.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figure/CA-synthetic-control.pdf} \\
    (a) Synthetic controls for California in post-intervention period \\
    \includegraphics[width=0.47\textwidth]{figure/sc_est_errors_boxplot.pdf} \\
    (b) Absolute error on control states
    \caption{\tbf{Nearest neighbor methods generate high-fidelity synthetic controls in counterfactual inference for panel data.} 
    % \rd{Are we trying to promote synthetic control? We should label it as SC. Also all colors in the left side is not easy.}
    % \ag{Todo: get rid of vertical grid lines in left plot; add ``Cigarette consumption (packs per capita)'' to y-axis on right figure; add line segments from label to line}
    }
    \label{fig:prop99}
\end{figure}

% \cite{cdcStateTobacco}
Next we consider a panel data setting, where our goal is to estimate the effect of the California Tobacco Tax and Health Protection Act of 1988 (a.k.a. Proposition 99) on annual state-level cigarette consumption\footnote{measured as per capita cigarette sales in packs}.
By definition, the counterfactual cigarette consumption in California---had Proposition 99 never been enacted---is not observed. 
\cite{abadie2010synthetic} introduce the notion of a ``synthetic control'' to serve as a proxy for this unobserved value based on ``neighboring'' \emph{control states} that never instituted a tobacco tax. These states are not close in a geographical sense, but rather close due to similarities in other covariates\footnote{GDP per capita, beer consumption, percent aged 15–24, and cigarette retail prices}. 
% See also: \cite{abadie2003economic}
We take a different approach and use only the observed cigarette consumption levels from the control states, of which there are 38 in total. Thus, we frame our problem as a scalar matrix completion problem with $N=39$ and $T=31$ (see \cref{eq:model}). The last row in the matrix corresponds to the state of California. 
% \ag{Mention that the staggered adoption missingness pattern, which falls under MNAR \cref{app:missingness} makes the estimation problem challenging.}
% We only observe measurements for California in the pre-intervention period (before 1989). 
% Thus, the missingness pattern is known as \emph{staggered adoption} \todo{cite}.
% Variants of nearest neighbors were adopted to construct synthetic controls to account for potentially existing unobserved confounders~\cite{agarwal2023causal}.

\paragraph{Results \& Discussion.}
% Whereas \cref{sub:hs} saw how nearest neighbor methods can effectively estimate counterfactual quantities for personalized treatments, 
For each method, we use a 64-16-20 train-validation-test split and use cross validation to fit any hyperparameters. \cref{fig:prop99} plots the various synthetic controls for California (left) and absolute error of each method on the 38 control states, for which we do observe the no-treatment values (right).
From \cref{fig:prop99}(a), we see that nearest neighbor methods, in particular $\tsnn$ and $\rownn$, are roughly on par with the gold-standard synthetic control method of \cite{abadie2010synthetic} (``SC'') for estimating California's counterfactual cigarette consumption in the post-intervention period (after 1989). This is despite the fact that the nearest neighbor methods rely on less information for the estimation task.
From \cref{fig:prop99}(b), we see that all nearest neighbor methods, with the exception of $\colnn$, achieve similar error levels as the synthetic control baseline. $\rownn$ achieves even lower error levels.
See supplementary experiment details in \cref{app:prop99}.

==> neurips2026/case-study.tex <==
\section{\lib{}-Bench and Results}\label{sec:case-study}

In this section, we evaluate several nearest neighbor algorithms provided by our library, \lib{}, on real-world data. As part of our package, we include data loaders which automatically download the necessary datasets and format them for evaluation. These datasets and loaders comprise our proposed benchmark for nearest neighbor matrix completion algorithms, \lib{}-\textbf{Bench}. We also test several existing popular matrix completion techniques~(\cite{hastie2015matrix,chatterjee2015matrix}). For details on our experimental setup, computing hardware, and boxplot generation, see \cref{app:case-studies}.


% ----------------
\iffalse
\subsection{Synthetic data}
\label{sub:simulations}


We first compare different matrix completion techniques on a synthetically generated data set. Our goal is to track the performance of different algorithms as the matrix size scales. We generate data matrix of size $N \times T$, where measurements $\measurement{i, t}$~(when $\missing{i, t} = 1$) are generated from distribution $\mu_{i, t} = \theta_{i, t} + \varepsilon_{i, t}$ where $\varepsilon_{i, t}$ are exogenous and i.i.d. centered Normal random variables. For more specifics on the data generation, see \cref{app:synthetic_gen}. The task here is to
\fi

% our synthetic data matrices with $d$-dimensional row latent factors $\uset := \{u_i, i\in[N]\}$, and column latent factors $\vset := \{v_t, t\in[T]\}$. For the following experiments, we let ${u_i \sim \text{Unif}[-0.5, 0.5]}$ for all $i \in [N]$ and ${v_t \sim \text{Unif}[-0.5, 0.5]}$ for all $t \in [T]$. 

% ----------------
\subsection{Personalized healthcare: HeartSteps}
\label{sub:hs}

% \paragraph{Case-study introduction}

The HeartSteps V1 study~(HeartSteps study for short) is a clinical trial designed to measure the efficacy of the HeartSteps mobile application for encouraging non-sedentary activity \cite{klasnja2019efficacy}. The HeartSteps V1 data and its subsequent extensions have been widely used for benchmarking a variety of tasks including counterfactual inference of treatment effect \cite{dwivedi2022counterfactual, choi2024learning}, reinforcement learning for intervention selection \cite{liao2019rlheartsteps}, and micro-randomized trial design \cite{qian2022microrandomized}. In the HeartSteps study, $N = 37$ participants were under a 6-week period micro-randomized trial, where they were provided with a mobile application and an activity tracker. Participants independently received a notification with probability $p = 0.6$ for $5$ pre-determined decision points per day for 40 days~($T = 200$). We denote observed entries $Z_{i, t}$ as the mean participant step count for one hour after a notification was sent and unobserved entries as the unknown step count for decision points where no notification was sent. Our task is to estimate the counterfactual outcomes: the participant's step count should they have received a different treatment (notification or no notification) than they did at specific time points during the study. 
% By computing the counterfactual outcome, we can also estimate the treatment effect of an intervention on an individual.
 

% Thus, the treatment application~(notification sent) is subject to an an individual's latent characteristics such as their personal schedule and daily routines. 

%availability of individuals encoded in the randomized trial implies that treatment application~(notification sent)

%Further, as notification are never sent during non-available times, positivity is clearly violated in this example.    % random given that they are available, positivity is violated as unavailable times has 0.0 probability 


% We proceed on our empirical analysis by imposing the potential outcome observation model \cref{mod:potential-outcome} on the HeartSteps data. 


\paragraph{Results \& Discussion.} We benchmark the performance of the matrix completion methods by measuring absolute error on held-out observed step counts across 10 participants in the last 50 decision points. We use the remaining data to find nearest neighbor hyperparameters using cross-validation. To benchmark the distributional nearest neighbors methods ($\kernelnn$ and $\wassersteinnn$) against the scalar methods, we first set each entry to have the number of samples $n = 60$, where each sample is the 1 minute step count before imputation. Then, we take the mean of the imputed empirical distribution as the estimate. 

In \cref{fig:hs-results}(a), we compare the absolute error of the imputed values across the nearest neighbor and baseline methods. The scalar nearest neighbor methods far out-perform USVT and are on par with SoftImpute. The two distributional nearest neighbor methods far outperform all methods operating in the scalar setting; it suggests that matching by distributions collect more homogeneous neighbors, thereby decreases the bias of the method, compared to matching only the first moments as done in most scalar matrix nearest neighbor methods. 

% which suggests that finding neighbors using a distributional distance can enhance the quality of the neighbors and reduce the bias of the estimate. 

In \cref{fig:hs-results} panel (b), we show an example of an imputed entry in the distributional nearest neighbors setting. In this case, the ground truth distribution is bimodal, as the participant was largely sedentary (0 steps) with small amounts of activity. While both $\kernelnn$ and $\wassersteinnn$ capture the sedentary behavior of the participant, $\kernelnn$ is able to recover the bimodality of the original distribution whereas $\wassersteinnn$ cannot. 


% \begin{wrapfigure}{R}{0.5\textwidth}
%     \begin{center}        \includegraphics{figure/hs_est_errors_boxplot.pdf}
%     \end{center}
%     \caption{\tbf{HeartSteps V1: Estimation error under notification sent.} We apply log-transform to the raw step counts before imputing.}
%     \label{fig:hs-results}
% \end{wrapfigure}

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.47\textwidth]{figure/hs_est_errors_boxplot.pdf} &  
        \includegraphics[width=0.33\textwidth]{figure/hs_distplot_48.pdf} \\
        (a) Absolute error of mean step count prediction &
        (b) $\kernelnn$ vs. $\wassersteinnn$
    \end{tabular}
    \caption{\tbf{HeartSteps: estimating step count under scalar and distributional matrix completion settings.} Panel (a) shows the absolute error of predicted step count of the nearest neighbor methods against matrix completion baselines (SoftImpute, USVT). Panel (b) shows an example of an imputed entry in the distributional matrix completion setting.
    }
    \label{fig:hs-results}
\end{figure}
% ----------------

\subsection{Movie recommendations: MovieLens}\label{sec:movielens}
\begin{wrapfigure}{R}{0.5\textwidth}
    \begin{center}        \includegraphics{figure/movielens_est_errors_boxplot.pdf}
    \end{center}
    \caption{\tbf{MovieLens: Estimation error for a random subsample of size 500.} For experimental settings and discussion see \cref{sec:movielens}.}
    \label{fig:movielens-error}
\end{wrapfigure}

The MovieLens 1M dataset \cite{movielens} contains 1 million ratings (1–5 stars) from 6,040 users on 3,952 movies. Collaborative filtering on MovieLens has long been a benchmark for matrix-completion methods: neighborhood-based algorithms~\cite{sarwar2001item}, latent-factor models~\cite{koren2009matrix}, and, more recently, nearest neighbors interpreted as blind regression under a latent–variable model~\cite{li2019nearest}. These assist practitioners in data-driven recommendation systems, since more accurate rating imputation directly drives better personalized suggestions and user engagement. This is a standard scalar matrix completion problem with $N=6,040$ and $T=3,952$. Each rating is an integer in $\{1,\dots,5\}$. The dataset has a very high percentage of missing values: 95.53\% missing. Our task is to estimate unobserved ratings using various matrix completion algorithms. We benchmark the performance of nearest neighbors against matrix factorization by measuring absolute error on held‑out ratings. See \cref{app:movielens} for additional details on the dataset.

\paragraph{Results \& Discussion.} We fit the nearest neighbor methods using a random sample of size 100 from the first 80\% of the dataset to choose nearest neighbor hyperparameters via cross-validation.We then test the method on a random subsample of size 500 from the last 20\% of the dataset. As observed in \cref{fig:movielens-error}, all nearest neighbor methods have a lower average error than USVT and a much lower standard deviation of errors, with $\colnn$, $\rownn$, $\drnn$, and $\autonn$ performing the best out of the nearest neighbor methods. SoftImpute performs on par with the nearest neighbor methods. Note that the nearest neighbor methods perform well even while only being trained on a tiny subset of the data of size 100 out of the 1 million ratings available.

\subsection{Counterfactual inference for panel data: Proposition 99}
\label{sub:prop99}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figure/california-synthetic-control.pdf}
%     \caption{\tbf{Counterfactual cigarette consumption had Proposition 99 never been passed.} We display synthetic controls constructed using various matrix completition methods. See detailed discussion in \cref{sub:prop99}
%     % \ag{can probably make this figure take up way less vertical space by putting the labels directly next to the corresponding line} 
%     \ag{Could also replace this with a figure like \cite[Fig. 8]{agarwal2023causal} to show the robustness of NN to unobserved confounding.}
%     }
%     \label{fig:prop99}
% \end{figure} 
\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.42\textwidth]{figure/CA-synthetic-control.pdf} &
        \includegraphics[width=0.47\textwidth]{figure/sc_est_errors_boxplot.pdf} \\
        (a) Synthetic controls for California &
        (b) Absolute error on control states \\ in post-intervention period
    \end{tabular}
    \caption{\tbf{Nearest neighbor methods generate high-fidelity synthetic controls in counterfactual inference for panel data.} For exact settings and further discussion see \cref{sub:prop99}.
    }
    \label{fig:prop99}
\end{figure}

% \cite{cdcStateTobacco}
Next we consider a panel data setting, where our goal is to estimate the effect of the California Tobacco Tax and Health Protection Act of 1988 (a.k.a. Proposition 99) on annual state-level cigarette consumption\footnote{measured as per capita cigarette sales in packs}.
By definition, the counterfactual cigarette consumption in California---had Proposition 99 never been enacted---is not observed. 
\cite{abadie2010synthetic} introduce the notion of a ``synthetic control'' to serve as a proxy for this unobserved value based on ``neighboring'' \emph{control states} that never instituted a tobacco tax. These states are not close in a geographical sense, but rather close due to similarities in other covariates\footnote{GDP per capita, beer consumption, percent aged 15–24, and cigarette retail prices}. 
% See also: \cite{abadie2003economic}
We take a different approach and use only the observed cigarette consumption levels from the control states, of which there are 38 in total. Thus, we frame our problem as a scalar matrix completion problem with $N=39$ and $T=31$ (see \cref{eq:model}). The last row in the matrix corresponds to the state of California. 
% \ag{Mention that the staggered adoption missingness pattern, which falls under MNAR \cref{app:missingness} makes the estimation problem challenging.}
% We only observe measurements for California in the pre-intervention period (before 1989). 
% Thus, the missingness pattern is known as \emph{staggered adoption} \todo{cite}.
% Variants of nearest neighbors were adopted to construct synthetic controls to account for potentially existing unobserved confounders~\cite{agarwal2023causal}.

\paragraph{Results \& Discussion.}
% Whereas \cref{sub:hs} saw how nearest neighbor methods can effectively estimate counterfactual quantities for personalized treatments, 
For each method, we use a 64-16-20 train-validation-test split and use cross validation to fit any hyperparameters. \cref{fig:prop99} plots the various synthetic controls for California (left) and absolute error of each method on the 38 control states, for which we do observe the no-treatment values (right).
From \cref{fig:prop99}(a), we see that nearest neighbor methods, in particular $\tsnn$ and $\rownn$, are roughly on par with the gold-standard synthetic control method of \cite{abadie2010synthetic} (``SC'') for estimating California's counterfactual cigarette consumption in the post-intervention period (after 1989). This is despite the fact that the nearest neighbor methods rely on less information for the estimation task.
From \cref{fig:prop99}(b), we see that all nearest neighbor methods, with the exception of $\colnn$, achieve similar error levels as the synthetic control baseline. $\rownn$ achieves even lower error levels.
See supplementary experiment details in \cref{app:prop99}.

% can estimate counterfactual quantities for large-scale interventions, like legislation at the state level. Moreover, we show that nearest neighbor methods are on par with conventional methods that leverage additional information.
% shows the synthetic controls constructed using the various nearest neighbor algorithms of \ag{cref}. Remarkably, $\starnn$ achieves a similarly high-fidelity synthetic control as the regression-based method of \cite{abadie2010synthetic}, which uses additional covariate information.

% \ag{Do we want an experiment to show that NN is more robust to unobserved confounding? Can then connect with the ideas introduced in \cref{sub:simulations}.}

% Missingness known as the staggered adoption pattern arises commonly in public policies. A powerful method to identify the treatment effect in such case is the synthetic controls~\cite{abadie2010synthetic} technique. 

% See \href{https://pypi.org/project/SyntheticControlMethods/}{here} for python version of SC and data.

% \paragraph{Data \& Pre-processing}

% ----------------

==> neurips2026/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our main claims in our abstract are a unified framework, a unified Python package, and a new test bench for nearest neighbor-based matrix completion methods. We present our unified framework for nearest neighbor-based matrix completion methods in \cref{sec:unified-view}. We present our package structure in \cref{sec:library}. Finally, we describe the new test bench in \cref{sec:case-study}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss improvements to our Python package in \cref{sec:conclusion}. The algorithms described in \cref{sec:nn-overview} use theoretical assumptions for their theoretical guarantees, but these assumptions do not affect the algorithms themselves, and thus pose no limitations on our Python package or test bench.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not claim any theoretical results in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All of our results can be reproduced with the code on our GitHub, which is (anonymously) linked in the paper. Each experiment has its own folder with instructions on how to run the experiments. We provide Python files which automatically download the necessary data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide an anonymous GitHub link to our open-source code. Every experiment can be reproduced with the Python files we provide separately from our Package source files. The new Python package we present, also in the GitHub link, can be installed quickly on standard computing hardware and do not require access to GPU's or any other specialized hardware.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For each experimental setup, we describe how we split up the datasets into train and test sets. We describe in detail how our hyperparameters are chosen in the Appendix. We also provide the code we use to choose hyperparameters in our open-source repository.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe how we generate our boxplots to compare error across methods in \cref{app:case-studies}. We also detail how our error bars are generated in our figures in the respective figures which have error bars.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe our computing setup in \cref{app:case-studies}. It is standard laptop hardware.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our research conforms with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work does not have any direct societal impact. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our new Python package and test bench do not pose a significant risk for misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Every library and dataset used in this work is properly cited and credited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work primarily releases a new code library that we have placed under the MIT License.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve any work with human subjects nor crowdsourcing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include any human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper's proposed algorithms do not involve LLM's in an important way.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> neurips2026/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

In this paper, we present a unified framework, Python library (\lib{}), and test bench (\lib{}-\textbf{Bench}) for nearest neighbor-based matrix completion algorithms for both scalar and distributional settings. We demonstrate how our library supports a diverse set of datasets spanning recommendation systems (MovieLens), patient-level healthcare causal inference (HeartSteps), counterfactual inference for panel data (Proposition 99), and LLM evaluation (PromptEval). Our framework and library facilitate researchers and practitioners to easily try out different nearest neighbor methods on their dataset of choice as well as extend the library to more complex nearest neighbor methods.

Several future directions are natural from our work. Here we focused on unweighted and specific weighing schemes; several other weighting strategies can be easily incorporated into the library. Next, being able to deal with larger matrices requires handling distributed datasets as well as speeding up the runtime of \lib{}, e.g., via efficient implementations using matrix multiplication or approximate nearest neighbors strategies.
% would allow . We also plan on adding support for distributed datasets too large to fit into memory. Finally, we plan on extending the library to other nearest neighbor algorithms, such as approximate nearest neighbors methods and ones that use linear regression instead of simple averaging.

% \ag{Future work: (1) speeding up, (2) bringing together approximate nearest neighbors (find references from supervised learning literature: \url{https://scholar.google.com/citations?user=9r7_pN8AAAAJ&hl=en})}

==> neurips2026/intro.tex <==
\section{Introduction}

Nearest neighbor methods are a class of non-parametric algorithms widely used for regression, classification and pattern recognition. Due to their scalability and success under models with minimal assumptions, nearest neighbor methods have recently been adopted for practical fields such as matrix completion and counterfactual inference in panel data settings. Matrix completion is a well-established field that supplies practitioners with many tools to recover underlying matrices using partial or even noisy observations~\cite{hastie2015matrix,chatterjee2015matrix,keshavan2010matrix}, with recommendation systems~\cite{koren2009matrix,recht2011simpler} as an important use-case. Panel data counterfactual inference aims at learning the treatment effect of policies across time~\cite{bai2009panel,bai2021matrix,athey2021matrix}. One important example is individualized healthcare predictions~\cite{klasnja2019efficacy}. Nearest neighbor methods were recently recognized as effective in providing granular inference guarantees for both matrix completion and counterfactual inference when either the missingness or the policy treatment are not completely random and confounded~\cite{ma2019missing,dwivedi2022counterfactual,agarwal2023causal}. They have also been recently leveraged to tackle distributional matrix completion settings~\cite{feitelberg2024distributional,choi2024learning}

% because they have bee?n shown to be competitive in terms of accuracy, can impute entry-wise, and are widely used in practice.


% Data scientists looking to use matrix completion to impute missing data have a diverse set of tools at their disposal including spectral based methods~\cite{hastie2015matrix,chatterjee2015matrix}, gradient methods (\cite{keshavan2010matrix}), 

% and nearest neighbor methods~\cite{li2019nearest,dwivedi2022counterfactual,agarwal2023causal,choi2024learning,feitelberg2024distributional}. 

Despite nearest neighbor methods popularity, there is no unified package that lets a user easily switch between different kinds of nearest neighbor algorithms for matrix completion and counterfactual inference. In this paper, we present a package\footnote{\url{https://anonymous.4open.science/r/NearestNeighbors-23A6}} to unify several nearest neighbor methods under a single interface, so users can easily choose the method that suits their data the best, for both scalar and distributional missing data problems. Next, we review two broad applications of nearest neighbors and matrix completion: recommendation systems and panel data settings.

\paragraph{Recommendation systems} In the problem of a recommendation system, multiple users submit ratings / preferences for a subset of items, and the vendor recommends items based on the partial rating information \cite{rennie2005fast}. Prediction of unseen ratings is the key to a good recommendation, and the predictions are based on the patterns of the partially observed ratings which can be formalized into a matrix completion problem. A popular instance is the Netflix problem, an open competition for the best prediction algorithm of user ratings of films. Users~(rows of matrix) have the option to rate the films~(columns of matrix). However, users typically rate only a subset of films, and the ratings are commonly biased towards their preferences. Under the common belief that only a few factors drive the preference and ratings of the users, many matrix completion algorithms have resorted to the low rank assumption on the ratings matrix~\cite{recht2011simpler,candes2012exact}. Variants of nearest neighbors~(in short, $\nn$) recently were introduced to correct for the potential bias originating from the fact that observation patterns are influenced by the matrix entries~(e.g. ratings) themselves and by unmeasured confounders~\cite{agarwal2023causal,abadie2024doubly}. 

\paragraph{Panel data} Panel data constitutes measurements of multiple units that are tracked over time~(hence a type of longitudinal data) as they undergo different types of interventions at different times~\cite{bai2009panel}. Panel data is used to analyze the causal effects of any policies, treatments, or business decisions that affect the subjects in the data, making this data type essential in econometrics and health studies. Matrix completion algorithms enable estimation of these causal effects at the unit$\times$time level, the most granular scale where causal effects can be estimated~\cite{athey2021matrix,agarwal2023causal}. For example, consider a mobile health app trying to learn the effectiveness of two exercise routines. Suppose the app alternates two routines across $N$ different users repeatedly over $T$ weeks, where their health activities~(say physical step counts) throughout each week are recorded. Then, we can use matrix completion to impute the counterfactual step counts under treatment and control, allowing us to estimate causal effects at the most granular scale.

\newcommand{\starnn}{\mathsf{StarNN}}
\newcommand{\autonn}{\mathsf{AutoNN}}

\paragraph{Our contributions}
We make the following contributions:
First, we present a unified framework for nearest neighbor algorithms that facilitates extending to new variants, especially for matrix completion problems. We leverage this framework to introduce then a new nearest neighbors algorithm, auto nearest neighbors~(in short $\autonn$), which aims both to improve on the existing methods and demonstrate the ease of developing new variants with our library.
Next, we introduce a unified, easy-to-implement nearest neighbor library that contains a breadth of nearest neighbor algorithms for matrix completion problems.
Next, we present a test bench called \lib{}\textbf{-Bench} that comprises of several real-world data sets across applications. Finally, we illustrate our library's wide applicability on the test benchmark.

% First, we introduce a framework for reasoning about the zoo of nearest neighbor algorithms via three modules: $\distancemod$, $\averagemod$, and \texttt{DataType} (\cref{sec:unified-view}).
% Second, we introduce a new variant, $\autonn$, that automatically balances between debiasing and denoising depending on the underlying noise level in a given problem (\cref{sec:new-nn}).
% Third, we present a testbed for NN-based matrix completion,  \lib{}\textbf{-Bench}, comprised of several real-world data sets across applications (\cref{sec:case-study}). We provide the first comprehensive comparison of NN methods on real-world matrix completion problems.
% Our investigation leads to new insights regarding how NN methods should be used in practice.
% For scalar matrix completion problems, $\autonn$ emerges as the new default method. For distributional matrix completion methods, $\kernelnn$ emerges as the default method.


\subsection{Related work}
We contextualize our contributions in the context of both nearest neighbors as a general algorithm and matrix completion specifically.

\paragraph{Nearest neighbors}

As introduced above, nearest neighbor methods are widely used for non-parametric regression, classification, and pattern recognition~\cite{cover1967nearest,cannings2020local}. Recently, nearest neighbor methods were introduced as an effective algorithm for matrix completion problems~\cite{li2019nearest,agarwal2023causal,dwivedi2022counterfactual}, especially when the missingness depended on observations and unobserved confounders. The fact that nearest neighbor methods target a single entry at a time via matching makes them effective against various types of missing patterns. The class of algorithms has grown to account for a wide range of applications involving scalar or distributional settings; for instance, nearest neighbors are used for evaluating the personalized recommendation effect of a healthcare app on the average and the distribution of physical step counts~\cite{dwivedi2022counterfactual,choi2024learning,feitelberg2024distributional,sadhukhan2024adaptivity} and are also used for policy evaluations~\cite{agarwal2023causal}.
% \rd{e.g., A, B, C, and cite for each use case.}~\cite{dwivedi2022doubly,choi2024learning,feitelberg2024distributional,sadhukhan2024adaptivity, sadhukhan2025adaptivelyweightednearestneighborsmatrix}, with a focus on inference for personalized treatment effects in the causal inference literature. 
Our library, \lib{}, is designed to easily implement the vanilla scalar versions of nearest neighbors~\cite{li2019nearest,dwivedi2022counterfactual} as well as its unweighted~\cite{dwivedi2022doubly,sadhukhan2024adaptivity} and weighted~\cite{sadhukhan2025adaptivelyweightednearestneighborsmatrix} variants. Finally, \lib{} is also capable of distributional matrix completion~\cite{choi2024learning,feitelberg2024distributional}.

\paragraph{Other matrix completion methods}

% \kc{@ MP, TS: Let's make this less notation heavy, more comprehensive citations, include soft-impute~\cite{hastie2015matrix} as it is one of our benchmarks.} 

Universal singular value thresholding (USVT), proposed in \cite{chatterjee2015matrix,bhattacharya2022matrix}, is a classical spectral-based method for performing matrix completion; its core functionality is based on a singular value decomposition of the matrix and thresholding the singular values.
%
SoftImpute, introduced by \cite{hastie2015matrix}, is another widely used optimization-based algorithm for matrix completion. The algorithm computes ridge-regression updates of the low-rank factors iteratively and finally soft-thresholds the singular values to impose a nuclear norm penalty. 
%
Notably USVT and SoftImpute have provable guarantees when missingness is completely at random, but empirically fail when the missing pattern depends on the observed entries or the unobserved confounders~\cite{agarwal2023causal}. Our real-world analysis in \cref{sec:case-study} once again demonstrates this point.

% The USVT algorithm completes a matrix by imputing zero for all the missing entries of the matrix, obtaining a estimate $\widehat p$ of the observation probability, performing a singular value decomposition of the imputed matrix, and retaining only those singular values that exceed $\tau \sqrt{\min\{N, T\}}$ (where $\tau > 2 \widehat p$). 

% \cite{chatterjee2015matrix} shows that the proposed algorithm attains minimax optimal performance when estimating matrices constrained by a bounded nuclear norm. 

\paragraph{Existing software for matrix completion and nearest neighbors}

Scikit-Learn \cite{scikit-learn}, a popular Python package for machine learning tools, implements a simple k-nearest neighbor algorithm for imputing missing values in a feature matrix. However, their implementation is designed for the feature matrix setting. So, neighbors are only defined across samples (row-wise). Additionally, they do not provide any implementation for more advanced nearest neighbor algorithms, nor does their package allow for easy extendability like our proposed package. 
% Another package which implements nearest neighbors for matrix completion is the Synthetic Nearest Neighbors (SNN) package (\url{https://github.com/deshen24/syntheticNN}). SNN implements a specific nearest neighbor algorithm for the causal matrix completion setting. 


% \cref{sec:nn-overview} contains an overview of the existing nearest neighbor algorithms implemented in our library, \lib{}. \cref{sec:new-nn} introduces a new nearest neighbor algorithm, $\autonn$, that is also implemented in \lib{}. \cref{sec:library} touches upon the high-level (class) structure of \lib{}, as well as the interface for practitioners. \cref{sec:case-study} tests different variants of nearest neighbor methods and classical methods on our new test bench of diverse datasets called \lib{}-\textbf{Bench}. Finally, in \cref{sec:conclusion}, we provide concluding remarks and outline future directions of research.


==> neurips2026/llm_evaluation.tex <==
\subsection{Efficient LLM evaluation}

Recent works show there is non-trivial variability of performance of language models across different prompting techniques\cite{sclar2023quantifying,polo2024efficient}, a natural follow up task being identification of the best performing prompting templates for certain tasks and language models~\cite{shi2024best,polo2024efficient}. The difficulty here is that there are near infinite ways of prompting, so an efficient evaluation framework has been investigated thoroughly~\cite{ye2023predictable,perlitz2023efficient}. Motivated by \cite{polo2024efficient}, we use the MMLU dataset~\cite{hendrycks2020measuring} and empirically demonstrate that our nearest neighbors method can achieve efficient evaluation. Under a fixed task~(e.g. abstract algebra, political science) various questions / examples are queried to a specific model, where each questions are restructured using different prompting templates. Either the model answers the question correctly or not and correctness is recorded. 

\paragraph{Results \& Discussion}

\kc{Do both SNN and DNN}

There are $57$ tasks and $15$ models total; the number of questions / examples depend on the task of interest and there is a fixed set of $100$ prompting templates that is applied to whatever question of whatever task. \kc{Could make a sub-section that explains MMLU.}


We consider a distributional matrix completion setup and implement a Dist-NN to estimate the distribution of averaged scores across templates~(template instances are of no value, as we aim to learn the overall variation) leveraging information across different models and different tasks. Imputation in \cite{polo2024efficient} was done while fixing model and task, so the commonalities that may exist across different models and tasks were not utilized.




% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figure/template_subject_model_by_propensity.pdf}
%     \caption{\kc{Figure needs adjustment, will not include boxplots of MMD errors for Kernel NN as most of them are zero---Wasserstein NN might have meaningful boxplots.} p = , standardize X }
%     \label{fig:temp_sub_model}
% \end{figure}



==> neurips2026/llm_evaluation_new.tex <==
\subsection{Efficient LLM evaluation: PromptEval}
\label{sub:llm}

% \begin{wrapfigure}{R}{0.5\textwidth}
%     \begin{center}
%     \includegraphics{figure/prompteval_est_errors_boxplot-p0.5.pdf}
%     \end{center}
%     \caption{\tbf{Kolmogorov-Smirnov distance with missingness at 50\%.} $\mmd$ using column-wise nearest neighbors performs the best in terms of the KS distance.}
%     \label{fig:ks}
% \end{wrapfigure}

The rapid advancement of LLMs have placed them at the center of many modern machine learning systems, from chatbots to aids in medical education \cite{geathers2025benchmarking}. In practice, system architects want to strike the right balance of real-world performance and cost, but navigating this Pareto frontier is a daunting task. 2024 alone saw at least 10 new models from Anthropic, Google, Meta, and OpenAI, not even counting the multitude of open-source fine-tuned models built on top of these.
% (Moreover, this number is likely to only grow as training models becomes more accessible, thanks in part to DeepSeek R1.) 
On specific tasks, smaller, fine-tuned models may even outperform the latest frontier models, in addition to being more cost effective.

We investigate how matrix completion, specifically nearest neighbor methods, can alleviate some of these burdens. We use the PromptEval dataset \cite{polo2024efficient}, which evaluates $15$ open-source language models (ranging in size from 3B to 70B parameters) and $100$ different prompting techniques across the 57 tasks of the MMLU benchmark \citep{hendrycks2020measuring}. In practice, the performance of a model depends---sometimes dramatically---on the precise input prompt. This suggests that we need to consider the performance of a model across a wide range of prompts, rather than any one prompt in particular. 
Thus, we model this problem as a distributional matrix completion problem with $N=15$, $T=57$, and $n=100$.
Given one of 57 tasks, we aim to accurately characterize the performance of each model without resorting to exhaustive evaluation.
Nearest neighbors leverage commonalities across models and tasks to estimate the performance distribution of each entry, which was otherwise not considered in \cite{polo2024efficient}; previous literature achieves efficient evaluation per model and task in isolation without leveraging any across model / task information. 

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.47\textwidth]{figure/ksbyp_prompteval_plot.pdf} & \includegraphics[width=0.45\textwidth]{figure/distributions-entry40-tp4.0.pdf} \\
        (a) Mean KS distance between estimated &
        (b) $\kernelnn$ vs. $\wassersteinnn$ \\
        and ground-truth distributions
    \end{tabular}
    \caption{\textbf{Distributional nearest neighbor methods enable efficient LLM evaluation on MMLU.} We estimate LLM score distributions across all models and tasks given only a limited number of model-task evaluations, determined by the propensity $p$. See \cref{sub:llm} for a detailed discussion.}
    \label{fig:llm}
\end{figure}

\paragraph{Results \& Discussion.}
We randomly include each entry in the matrix independently with probability $p\in \braces{0.3,0.5,0.7}$ and impute the missing entries using the $\kernelnn$ and $\wassersteinnn$ methods of \cref{tab:summary}. For each method, we consider both the the row-wise and column-wise variants.
\cref{fig:llm}(a) reports the mean Kolmogorov-Smirnov (KS) distance between the imputed and ground-truth distributions across the entries in the test set for varying missingness values. As expected, estimation error decreases as $p$ increases.
% the number of observed entries increases. 
% versus the ground truth at varying levels of $p$ for a select entry in the matrix. At $p=0.3$, we avoid 70\% of LLM evaluations, yet still recover the distribution of prompt scores with reasonable quality. At $p=0.5$ and $p=0.7$, column-wise NN with $\mmd$ performs the best.
\cref{fig:llm}(b) visualizes the imputed distributions using row-wise $\kernelnn$ and column-wise $\wassersteinnn$ (at $p=0.7$) for a select entry, along with the ground-truth distribution. Even with 30\% of matrix entries missing, distributional NN methods are able to recover the underlying distribution.

==> neurips2026/nn-new.tex <==
\subsection{New variant: Auto nearest neighbors}\label{sec:new-nn}

% \kc{Moved AWNN in the appendix as it seems that we will cite(?) the work. If the paper is not out before submission, we can make a subsection of $\awnn$ later. For now, subsection 2.3 will be about $\autonn.$}

% We introduce and discuss two new variants of nearest neighbors that improve upon the shortcomings of previously introduced nearest neighbor algorithms on the scalar matrix \cref{eq:model}. First, cross-validation is a crucial step for all nearest neighbors, but the computation run-time scales as $O(N^2T^2|E|)$ where $E$ is the search space for $\tuning$ and $|E|$ its cardinality; there are $NT$ number of $\tuning$ to determine for $NT$ number of estimands and the row or column distance calculation requires at most $N^2 \vee T^2$ number of calculations. \kc{@TS, MP: How does $\awnn$ improve exactly in terms of order?.} Second, 

% $\autonn$ enables an automatic adaption to the underlying environment via cross-validation.




% Weighted $k$-nearest neighbors have been a fundamental non-parametric method of interest. 


% \subsubsection{Automatic nearest neighbors~($\autonn$)}

% \kc{May need to delete if we don't have promising experiment results.}


% The vanilla versions of nearest neighbors~(i.e., $\rownn, \colnn$) are shown to be dominated by $\tsnn$ in performance  under reasonable assumptions~(see \cref{app:guarantees}). 

% Two $\drnn$ and $\tsnn$ perform optimally on different assumptions~(\kc{exactly how?}), and verification of the assumptions on real world data is difficult. 


% \footnote{\kc{See ..., $\awnn$ cannot recover $\drnn$ nor $\tsnn$.}}.
% TSNN and DRNN is of different nature, whereas TSNN generalizes; see..., and also note AWNN (cts weight version) also is constructed via different spirit.
$\tsnn$ is a generalization of $\rownn$ and $\colnn$ by setting one of the tuning parameters to zero~(see \cref{tab:summary}), whereas the idea underlying $\drnn$ is fundamentally different from that of $\tsnn$; $\drnn$ debiases a naive combination of $\rownn$ and $\colnn$ whereas $\tsnn$ simply boosts the number of measurements averaged upon, thereby gaining from lower variance. 
So we simply interpolate the two methods 
% and propose
% \newcommand{\interpolate}{\mathsf{LI}}
% \begin{align}\label{eq:inter-nn}
%     \what\theta_{i, t, \tuning, \alpha}^{\interpolate} = \alpha \what{\theta}_{i, t, \tuning}^{\dr} + (1 - \alpha) \what{\theta}_{i, t, \tuning}^{\ts}
% \end{align}
for some hyper-parameter $\alpha \in [0, 1]$; see \cref{tab:summary}. 
% where $\what{\theta}_{i, t, \tuning}^{\dr}$ and $\what{\theta}_{i, t, \tuning}^{\ts}$ are the output of running methods $\drnn$ and $\tsnn$ in \cref{tab:summary} respectively. 
Notably the hyper-parameter $\tuning$ for both $\drnn$ and $\tsnn$ are identical when interpolated.

Suppose $\dist{i, t} = \theta_{i, t} + \varepsilon_{i, t}$ in \cref{eq:model} where $\varepsilon_{i, t}$ are centered i.i.d. sub-Gaussian distributions across $i $ and $t$.
% \rd{why do we need Gaussian noise?}. 
When $\sigma$ is large in magnitude, $\tsnn$ denoises the estimate by averaging over more samples, hence providing a superior performance compared to $\drnn$ in a noisy scenario. When $\sigma$ is small so that bias of nearest neighbor is more prominent, $\drnn$ effectively debiases the estimate so as to provide a superior performance compared to $\tsnn$. The linear interpolator $\autonn$ \textit{automatically} adjusts to the underlying noise level and debiases or denoises accordingly; such property is critical when applying nearest neighbors to real world data set where the noise level is unknown. We refer to \cref{fig:auto_perf} for visual evidence.




% s that $\tsnn$ is a generalization of $\rownn$ and $\colnn$ by setting one of the tuning parameters to zero~(see \cref{tab:summary}); however $\drnn$ cannot be recovered from the $\tsnn$. 

% A common understanding is that $\tsnn$ outperforms $\drnn$ when the noise level of data is high, whereas $\drnn$ performs better with data of high signal. \kc{@CC: Do you think it would be good to blend the synthetic experiment in this section, by showing the two plots?}

\begin{figure}[H]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.43\textwidth]{figure/sims_plot_mednoise_format.pdf} &  
        \includegraphics[width=0.43\textwidth]{figure/sims_plot_highnoise_format.pdf}
        \\ (a) High SNR & (b) Low SNR
    \end{tabular}
    % \caption{\tbf{Comparing $\drnn$, $\tsnn$ and $\autonn$ with synthetic data.} The data used for the left panel has high signal compared to the noise, whereas the data for the right panel has high noise level compared to the signal. See \cref{app:synthetic_gen} for details on the data-generating process.}
    \caption{\tbf{Error scaling for certain NN variants in synthetic experiments.}
    See \cref{app:synthetic_gen} for details on the data-generating process and how the signal-to-noise ratio (SNR) is defined. Each point corresponds to the mean absolute error ± 1 standard error across 30 trials.}
    \label{fig:auto_perf}
\end{figure}


% note that the hyper-parameter $\tuning = (\tuning_1,\tuning_2)$ are identical. Then 



% \begin{figure}
%     \begin{center}        \includegraphics{figure/autonn_sims_sigma001.pdf}
%     \end{center}
%     %\caption{\tbf{\cc{This is noise with sigma 0.001}.}
%     \label{fig:autonn_sim_error}
% \end{figure}
% \begin{figure}
%     \begin{center}        \includegraphics{figure/autonn_sims_sigma1.pdf}
%     \end{center}
%     %\caption{\tbf{\cc{This is noise with sigma 1}.}
%     \label{fig:autonn_sim_error_highnoise}
% \end{figure}
% \kc{We set $f_\gamma(x) = (1 - \gamma)x + \gamma$ and $g_\gamma(x) = $}





% Interpolation between the two requires specification of 
% \begin{enumerate}
%     \item[(i)] how to distribute the entries in the matrix to each methods,
%     \item[(ii)] how to define the average. 
% \end{enumerate}

% \subsection{One way to proceed}
% \begin{figure}
%     \centering
%     {\includegraphics[width=14cm]{figure/Geom-balancing.pdf} }
%     \label{fig:geom-balance}%
% \end{figure}

% For the target entry $(i, t)$, let $(\eta_1, \eta_2)$ be the tuning parameters that determine the row and column threshold used for TSNN~(and also probably DRNN)\footnote{Natural question: are there any relations between the tuning parameters of DRNN and TSNN?}. Let the matrix in figure \ref{fig:geom-balance} be the sub-matrix sieved out by $\eta:= (\eta_1, \eta_2)$. Define $\mathcal I_{i, t}(\eta)$ as the collection of matrix entry indices that were chosen by $\eta$ around the target entry $(i, t)$. 

% The additional tuning parameter $\alpha$ and the function 
% \begin{align}
%     S_\alpha : \mathcal I_{i, t}(\eta) \mapsto  \mathcal T_{i, t}(\alpha)
% \end{align}
% where $\mathcal T_{i, t}$ corresponds to the \textcolor{blue}{blue} entries in figure \ref{fig:geom-balance}\footnote{Natural question: How does the performance of TSNN change if the column and row observations are excluded?}
% ---tuning parameter $\alpha$ controls the \textit{convexity} of the red line in figure \ref{fig:geom-balance}, thereby controlling $|\mathcal T_{i, t}|$ in a continuous manner. Each entry contains measurement $Y_{j, s} \in \mathbb R$ whenever $A_{i, t} = 1$, which is otherwise~($A_{i, t} = 0$) missing. Then one interpolation of DRNN~\cite{dwivedi2022doubly} and TSNN~\cite{sadhukhan2024adaptivity} is
% \begin{align}
%     \widehat{\theta}_{i, t, \alpha, \eta} := \frac{ \sum_{(j, s) \in \mathcal T_{i, t} }A_{j, s}Y_{j, s} + \sum_{(j, s) \in \mathcal I_{i, t}(\eta) \setminus \mathcal T_{i, t}(\alpha)} A_{i, s}A_{j, t}A_{j, s} \big( Y_{i, s} + Y_{j, t} - Y_{j, s} \big) }{\sum_{(j, s) \in \mathcal I_{i, t}(\eta)} A_{j, s}}.
% \end{align}
% Again, as TSNN dominates Vanilla-NN, automated navigation of the best NN can be realized by choosing the parameters $(\alpha, \eta)$ in a data-dependent manner.

\newcommand{\colsize}{N_{1, \eta_2}^{\mrm{col}}}
\newcommand{\rowsize}{N_{1, \eta_1}^{\mrm{row}}}

% \subsection{Another way to proceed}
% We argue that the way Figure \ref{fig:geom-balance} distributed data points to each methods is not optimal. We briefly discuss the guarantees of DRNN~\cite{dwivedi2022doubly} and TSNN~\cite{sadhukhan2024adaptivity}. Let $\theta_{1, 1}$ be the target of interest and set $\mbf N_{1, \eta_1}^{\mrm{row}}$ be the row-wise neighbor~(not adjusted for missingness) and $\mbf N_{1, \eta_2}^{\mrm{col}}$ be the column-wise neighbor. The cardinality of each neighbors are $N_{1, \eta_1}^{\mrm{row}} = |\mbf N_{1, \eta_1}^{\mrm{row}}|$ and $N_{1, \eta_2}^{\mrm{col}} = |\mbf N_{1, \eta_2}^{\mrm{col}}|$. Assume bi-linear factor model for simplicity and assume $A_{i, t} = 1$ for all $(i, t) \in [N] \times [T]$, so every entry is observed. 

% Then \cite[Cor. 1]{dwivedi2022doubly} and \cite[Thm. 1]{sadhukhan2024adaptivity} states 
% \begin{align}\label{eq:guarantees}
%     &\big( \what \theta_{1, 1, \eta}^{\mrm{DR}} - \theta_{1, 1} \big)^2 \leq O_p\biggparenth{\eta_1\cdot \eta_2 + \frac{1}{\rowsize} + \frac{1}{\colsize}}\quad \text{and} \\ &\big( \what \theta_{1, 1, \eta}^{\mrm{TS}} - \theta_{1, 1} \big)^2 \leq O_p\biggparenth{\eta_1 + \eta_2 + \frac{1}{\rowsize\cdot\colsize}}.
% \end{align}

% We return to the claim that partition of entries as done in Figure \ref{fig:geom-balance} is not optimal. The bias of NN in general is governed by the maximum number of entries used throughout each columns or rows. Variance of TSNN is governed by the total number of entries used, regardless of how the set of blue entries is shaped. So to optimally use TSNN, we need to
% \begin{itemize}
%     \item maximize volume of the set of blue entries
%     \item while keeping the length of the boundary of the set minimal.
% \end{itemize}
% For that end, the square is the most efficient shape to assign for TSNN. 


% \begin{figure}
% \centering
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=1.2\linewidth]{figure/Geom-balancing1.pdf}
%   \label{fig:geom-balance2-1}
% \end{minipage}%
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=1.2\linewidth]{figure/Geom-balancing2.pdf}
%   % \captionof{figure}{Another figure}
%   \label{fig:geom-balance2-2}
% \end{minipage}
% \end{figure}

% So we do the procedure as depicted in Figure \ref{fig:geom-balance2-1}.. The blue entries used for TSNN are far away from the target $\theta_{1, 1}$ but it wouldn't matter as long as all the entries within the blue set contributes via averaging. There are two yellow set, both on which DRNN is applied. The overlap of the two yellow set need to be dealt with care (\kc{not sure how?}). 

% Then the resulting guarantee for $\what \theta_{1, 1, \alpha, \beta, \eta}$~(\kc{define! --- for now let's use a similar averaging as done above}) is
% \begin{align}
%     &\big( \what \theta_{1, 1, \alpha, \beta, \eta} - \theta_{1, 1} \big)^2 \\
%     &\leq O\biggparenth{\alpha \eta_1 + \beta \eta_2 + \frac{1}{\alpha \beta \rowsize \colsize} + (1 - \beta) \eta_1\eta_2 + \frac{1}{\rowsize} + \frac{1}{(1 - \beta)\colsize} + (1 - \alpha) \eta_1\eta_2 + \frac{1}{(1 - \alpha) \rowsize} + \frac{1}{\colsize}}.
% \end{align}
% Note that $N_{1, \alpha \eta_1}^{\mrm{row}} = \alpha \rowsize$ for any $\alpha$ as everything here is linear. The conclusion here is 
% \begin{itemize}
%     % \item Simple linear interpolation is at most as good as either DRNN or TSNN, so useless.
%     \item Gaining both Bias and Variance is impossible.
%     \item Gaining only one of Bias or Variance is also near impossible.
%     \item Gaining either in Bias while losing a bit of Variance~(or vice versa) is feasible, and $\alpha, \beta$ serves as an additional tuning parameter to balance between the two terms --- can't know if there is an improvement unless analytically solved. 
% \end{itemize}

% \kc{It is difficult to develop a method via geometric approach --- distributing entries is doable but a good averaging procedure is not easy. So we proceed with a more algebraic approach, elaborated in the next subsection.}

% \begin{align}
%     \widetilde{\theta}^{\mrm{TS}}_{1, 1, \eta} = \frac{1}{(\rowsize + 1)(\colsize + 1)} \sum_{j \in  \mbf N_{1, \eta_1}^{\mrm{row}}, s\in  \mbf N_{1, \eta_2}^{\mrm{col}}} \big\{ Y_{j, 1} + Y_{1, s} + Y_{j, s} \big\}.
% \end{align}
% The idea is that adding measurements from one more row and one more column would not change the guarantees in terms of convergence rate, i.e. 
% \begin{align}
%     \E\big[ ( \tilde \theta^{\mrm{TS}}_{1, 1} - \theta_{1, 1, \eta} )^2 \big] \asymp  \E\big[ ( \what\theta^{\mrm{TS}}_{1, 1, \eta} - \theta_{1, 1} )^2 \big].
% \end{align}
% For each $j, s$ define a set of parameters $ \Gamma := \{ \gamma_{j, s} \}_{j \in [N], s \in [T]}$. Define an estimator
% \begin{align}
%     \what{\theta}^{\Gamma}_{1, 1, \eta} := \frac{1}{(\rowsize + 1)(\colsize + 1)} \sum_{j \in  \mbf N_{1, \eta_1}^{\mrm{row}}, s\in  \mbf N_{1, \eta_2}^{\mrm{col}}} \big\{ Y_{j, 1} + Y_{1, s} + \gamma_{j, s}Y_{j, s} \big\}.
% \end{align}
% If $\gamma_{j, s} = 1$ for all $j, s$, then $\what \theta^\Gamma_{1, 1, \eta}$ recovers TSNN and if $\gamma_{j, s} = -1$ for all $j, s$, then it recovers DRNN. For simplicity, let $\gamma_{j, s} = \gamma$ or $\gamma_{j, s} = \gamma^{\mrm{row}}_j \cdot \gamma^{\mrm{col}}_s$ for all $j, s$ and then optimize. 

% \kc{Let's try experiment without missingness, linear factor model, no noise.}


==> neurips2026/nn-overview.tex <==
\section{Nearest Neighbors for Matrix Completion}\label{sec:nn-overview}


% \kc{Start with a table as in page 2 of \href{https://arxiv.org/pdf/2404.12290}{link}. Then refer to the specific algorithms within the table~(with appropriate references). Then present 4 modules: distance calculation, averaging, subraction, weighting. Start with the abstract modules and specify. For DNN, add as a specific in the row-wise NN. All the settings compress. Need to cut it by page 4. }

% \kc{(2 pages)}

We now introduce the mathematical model for matrix completion:
% \kc{$\dist{i, t}$ to additive noise model.}
\begin{align}
\qtext{for} i \in [N], t\in[T]:\quad \measurement{i, t} :=
     \begin{cases}
        \sample{1}(i, t), ..., \sample{n}(i, t) \ \sim \ \dist{i, t}&\qtext{if} \missing{i, t}=1, \\
        \mrm{unknown}&\qtext{if} \missing{i, t}=0.
    \end{cases}
    \label{eq:model}
\end{align}
In other words, for matrix entries where $\missing{i, t} = 1$, we observe $n$ measurements $\measurement{i, t}$ that takes value $\sample{i, t}$ realized from distribution $\dist{i, t}$. When $n = 1$, i.e., $\measurement{i,t} = \sample{1}(i, t)$, we refer to \cref{eq:model} as the \textit{scalar matrix completion} model; scalar matrix completion is the most common problem posed in the literature~\cite{candes2012exact,recht2011simpler,koren2009matrix,hastie2015matrix,chatterjee2015matrix,dwivedi2022counterfactual,dwivedi2022doubly,agarwal2023causal}, where the goal is to learn the mean of the underlying distributions $\sbraces{ \meanparam{i, t} = \int x d\dist{i, t}(x)}_{i \in [N],t \in [T]}.$ When there are more than one observed measurements per entry, i.e., $\measurement{i, t} = [\sample{1}(i, t), ..., \sample{n}(i, t)]$ for $n \geq 2$, we refer to \cref{eq:model} as the \textit{distributional matrix completion} problem, the goal being the recovery of the distributions as a whole.
%
We refer the readers to \cref{app:guarantees} for a detailed discussion on the structural assumptions imposed on the model \cref{eq:model}.


% \ag{Just a thought: do these other papers handle the case when $n>1$? If not, we can highlight that nearest neighbors can handle this setting and more, which leads us into the next paragraph!}

% Given this data with missing observations, the practitioner is interested in estimating the moments of the distributions $\{\dist{i, t}\}_{i \in [N], t \in [T]}$; under the scalar matrix completion problem, the target is only on the mean of the distributions $\sbraces{ \meanparam{i, t} = \int x d\dist{i, t}(x)}_{i \in [N],t \in [T]}.$ % When $\missing{i, t} = 0$, we have no accessible information from $\dist{i, t}$, and when $A_{i, t} = 1$, we do not have access to the exact distribution $\mu_{i, t}$ rather only a single measurement from $\dist{i, t}$ are available. 

\subsection{Unified framework}\label{sec:unified-view}
We introduce two general modules~(namely $\distancemod$ and $\averagemod$) from which the variants of nearest neighbors are constructed. We introduce several shorthands used in the modules. Denote the collection of measurements, missingness, and weights:
\begin{align}
    \mc Z:=\big\{\measurement{j, s}\big\}_{j \in [N] , s \in [T]} , \quad  \mc A := \sbraces{\missing{j, s}}_{j \in [N], s \in [T]}, \qtext{and} \mc W := \sbraces{w_{j, s}}_{j \in [N],s \in [T]}.
\end{align} 
Let $\entrydist{x, x'}$ be a metric between $x, x' \in \mc X$ for some space $\mc X$. Further define $\entrydistest{\measurement{i, t}, \measurement{j, s}}$ as a data-dependent distance between any two observed entries $(i, t)$ and $(j, s)$ of the matrix \cref{eq:model}. The two modules can now be defined: 
\begin{itemize}
    \item[(i)] $\distancemod (\what{\varphi}, \mc Z, \mc A)$: Additional input is the data-dependent distance between entries of matrix $\what{\varphi}$ and output is the collection of row-wise and column-wise distance of matrix:
    \begin{align}\label{mod:distance}
        \distance{i, j}^{\row} := \frac{\sum_{s \neq t}\missing{i, s}\missing{j, s}\entrydistest{\measurement{i, s}, \measurement{j, s}}}{\sum_{s \neq t} \missing{i, s}\missing{j, s}} \qtext{and} \distance{t, s}^{\col} := \frac{\sum_{j \neq i}\missing{j, t}\missing{j, s}\entrydistest{\measurement{j, t}, \measurement{j, s}}}{\sum_{j \neq i} \missing{j, t}\missing{j, s}},
    \end{align}
    \item[(ii)] $\averagemod (\varphi, \mc W, \mc Z, \mc A)$: Additional input are the weights $\mc W$, metric $\varphi$ and output is the optimizer
        \begin{align}\label{eq:ave-output}
           \what{\theta} = \argmin_{x \in \mc X}\sum_{j \in [N], s \in [T]} \weight{j, s}\missing{j, s}\entrydist{x, \measurement{j, s}}.
        \end{align}
        \iffalse
    \item[(iii)] \composemod($\what \theta_1$, $\what \theta_2$): For any two optimizers \cref{eq:ave-output} as input, the output is $f(\what \theta_1, \what \theta_2)$ for some function $f$.
    \fi
    % \begin{itemize}
    %     \item[$\mbf{subMod}2$] ($\weightmod$) 
    %     \item[$\mbf{subMod}1$] ($\neighbormod$) 
    % \end{itemize} 
    % \item[$\mbf{Mod}3$] $\subtractmod()$ Taking the difference of averages attained in module $\averagemod$.
\end{itemize}
% \begin{remark}
%     The two modules $\distancemod$ and $\averagemod$ are implicitly coupled via the weights $\weight{}$ in $\averagemod.$ For instance, a binary weight defined via the module $\distancemod$ and tuning parameters $\tuning$
%         \begin{align}\label{eq:std-weight}
%             \weight{j, s} = \indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}.
%         \end{align}
%     recovers $\rownn, \distnn, \tsnn, \drnn$. Otherwise, a non-binary weight $\weight{}$ recovers $\awnn$~\kc{@MP, TS: Fill up details.}
% \end{remark}
The $\distancemod$ module calculates the row-wise and column-wise distance of the matrix, by taking the average of the observed entry-wise distance $\entrydistest{\cdot, \cdot}$. The $\averagemod$ module calculates the weighted average of observed measurements, where the notion of average depends on the metric $\varphi$ and the space $\mc X$ on which the metric $\varphi$ is defined. 
\iffalse
If $\mc X = \real$ and $\varphi(x, x') = (x - x')^2$, then the average is simply weighted sample mean of observed entries. If $\mc X$ is the space of all square integrable probability measures on the real line, then the average is the barycenter of probability measures; see \cite{muandet2017kernel,bigot2017geodesic} and \cref{app:guarantees} for a comparison on the $\mmd$ and $\wasserstein$ barycenters. 
\fi
Notably, the weights $\mc W$ in the $\averagemod$ module encodes the entry information of the estimand. 

\begin{remark}\label{rem:row-nn}
The vanilla row-wise nearest neighbors~\cite{li2019nearest} that targets the mean $\theta_{i, t} = \int x d\dist{i, t}(x)$ of entry $(i, t)$ is recovered by first applying $\distancemod$ with $\entrydistest{\measurement{j, s}, \measurement{j', s'}} = {(\measurement{j, s} - \measurement{j', s'})^2}$, applying $\averagemod$ with the non-smooth weight
% with entry information $(i, t)$ and tuning parameter $\Vec{\tuning} = (\tuning_1, \tuning_2)$,
${\weight{j, s} = \indic{\distance{i,j}^\row \leq \tuning_1}\cdot \indic{\distance{s, t}^\col \leq 0}}$, and using the metric $\entrydist{x, y} = (x - y)^2$. Note that the non-smooth weight satisfies $\weight{j, t} = \indic{\distance{i, j}^\row \leq \tuning_1}$, whereas $\weight{j, s} = 0$ for $s \neq t$; by defining the nearest neighbor set $\mbf N_{t, \tuning_1} := \{ j \in [N] : \distance{j, t}^\row \leq \tuning_1 \}$, the $\averagemod$ module output can be rewritten as ${\argmin_{x \in \real} \sum_{j \in \mbf N_{t, \tuning_1}} \missing{j, t}(x - \measurement{j, t})^2 = |\mbf N_{t, \tuning_1}|^{-1}\sum_{j \in \mbf N_{t, \tuning_1}}\measurement{j, t}}$.
% In other words, the simple average of the nearest neighbors within column $t$.
\end{remark}




% When there are multiple measurements per entry~(i.e., $n > 1$ in \cref{eq:model}), $\entrydistest{\measurement{i, t}, \measurement{j, s}}$ would represent an estimated distributional distance between $\dist{i, t}$ and $\dist{j, s}$ using data $\measurement{i, t}, \measurement{j, s}$. For instance, the squared maximum mean discrepency~(in short $\entrydist{\dist{i, t}, \dist{j, s}} = \mmd_\kernel^2(\dist{i, t}, \dist{j, s})$, see \cite{muandet2017kernel}) are estimated via the unbiased U-statistics estimator~(in short $\entrydistest{\measurement{i, t}, \measurement{j, s}} = \what \mmd_\kernel^2(\measurement{i, t}, \measurement{j, s})$). The same goes for the Wasserstein metric~(in short $\entrydist{\dist{i, t}, \dist{j, s}} = \wasserstein(\dist{i, t}, \dist{j, s})$) and its estimator (in short $\entrydistest{\measurement{i, t}, \measurement{j, s}} = \hatwasserstein(\measurement{i, t}, \measurement{j, s})$, see \cite{bigot2020}). See \cref{app:guarantees} for a detailed review on the distributional versions of $\what{\varphi}$. 

% enables estimation of the distributional distance of choice between two entries; for instance, the maximum mean discrepency~(in short $\mmd$, see \cite{muandet2017kernel}) between $\mu_{i, t}$ and $\mu_{j, s}$ can be estimated by an unbiased U-statistics estimator and similarly for the Wasserstein distance~(in short $\wasserstein$, see \cite{bigot2020}). See \cref{app:guarantees} for a detailed exposition on the estimators of $\mmd$ and $\wasserstein$.



\iffalse
For any two distributions $\mu, \nu$, $\varphi(\mu, \nu)$ denotes a distributional metric between the two distributions, later specified as either the estimated $\mmd$~\cite{muandet2017kernel} or $\wasserstein$~\cite{bigot2020}; let $\entrydistest{\measurement{j, s}, \measurement{j', s'}}$ be either the estimator $\what{\mmd}_\kernel$ or $\hatwasserstein$. The multiple measurements $\measurement{i, t}$ in \cref{eq:model-dist} can be equivalently regarded as an empirical distribution; that is $n^{-1}\sum_{i = 1}^{n}\dirac_{\sample{i}(i, t)}$. Refer to \cref{app:guarantees} for details. 
\fi

\subsection{Existing methods}
\label{subsec: existing methods}
We present existing variants of nearest neighbors using the two modules introduced \cref{sec:unified-view}; all the methods presented here are recovered by sequentially applying $\distancemod$ and $\averagemod$ with the appropriate specification of $\what \varphi$, $\varphi$ and $\mc W$. 
\iffalse
For simple notation, we introduce a shorthand for the non-continuous weight
\begin{align}
    \weight{j, s}^{(i, t)}(\tuning_1, \tuning_2) := \indic{\distance{i,j}^\row \leq \tuning_1}\cdot \indic{\distance{s, t}^\col \leq \tuning_2}.
\end{align}
\fi
% Here we provide a new variant of nearest neighbors introduced in \cref{tab:summary}, $\awnn$, designed to automatically adapt to the underlying unknown data characteristics; adaptivity is made possible by generalizing the algorithm so as to encapsulate all the nearest neighbor methods for scalar matrix completion problem, that uses non-smooth weights~(i.e., $\rownn, \colnn, \tsnn, \drnn$ in \cref{tab:summary}).

All methods except $\awnn$ and our newly proposed $\autonn$, have binary weights i.e., $w_{j,s}\in\sbraces{0,1}$. $\autonn$, detailed in \cref{sec:new-nn}, uses weights to carefully pool together the benefits of $\tsnn$ and $\drnn$. $\awnn$~\cite{sadhukhan2025adaptivelyweightednearestneighborsmatrix} improves upon $\rownn$  by adaptively choosing the weights which optimally balances the bias-variance tradeoff of $\rownn$ as follows % For notational convenience, we define a vector
\begin{align}\label{eq:star-nn-weight}
  \big(\weight{1}^\star(i, t), ..., \weight{N}^\star(i, t)\big):= \argmin_{(v_{1}, ..., v_{N})\in \Delta_N} 2\log(2N)\widehat \sigma^2 \sum_{k \in [N]}v_{k}^2 + \sum_{k \in [N]}v_{k} A_{k,t}\distance{i,k}^\row  .
\end{align}
where $\widehat \sigma^2$ is the estimated error and $\Delta_N$ is a simplex in $\real^N$; see \cite{sadhukhan2025adaptivelyweightednearestneighborsmatrix} for details of \cref{eq:star-nn-weight}. \cref{tab:summary} contains a concise summary of the existing nearest neighbor variants; see \cref{app:nn-algo} for a detailed exposition for each methods.


\iffalse
We also define the following weight function,
\begin{align}
    \widetilde {\weight{j, s}}^{(i, t)}:= \widetilde{\weight{j}}^{(i, t)} \cdot \indic{\distance{s, t}^\col \leq 0},
\end{align}
where the vector $\widetilde{\weight{}}^{(i, t)} = (\widetilde{\weight{1}}^{(i, t)}, \cdots, \widetilde{\weight{n}}^{(i, t)})$ is defined as,
 \begin{align}
  \widetilde{\weight{}}^{(i, t)}  := \mbox{arg min}_{\weight{}^{(i, t)}} \Big[2\log(2m)\widehat \sigma^2\|\weight{}^{(i, t)}\|_2^2 + \sum_{j =1 }^m  \weight{j}^{(i, t)} A_{j,t}\distance{i,j}^\row  \Big].
\end{align}
In the above optimization, $\weight{}^{(i, t)}$ is used to denote a candidate non-negative weight vector, the sum of whose elements is $1$. The estimate of error variance $\widehat \sigma^2$ is computed from $\mc Z$. 
\fi

% \clearpage
% \begin{table}[H]
% \caption{\label{tab:summary_of_nn}\textbf{Variants of nearest neighbor data types.} The two modules \jf{Should the indicators be different on the last column?}}
%   % \kc{any better ideas for the table? there seems to be repeated info and also DRNN does not fully blend in.}} 
%   % \ag{You could use a single, large box to cover the ``Euclidean'' entries}}
%   \centering
%   \begin{tabular}{cccccc}
%     \toprule
%     \tbf{Type}
%     & \tbf{Algorithm}
%     & $\entrydistest{\cdot, \cdot}$
%     & $\entrydist{\cdot, \cdot}$
%     & $\tuning = (\tuning_1, \tuning_2)$ 
%     & $\weight{}$
%     \\
%     \midrule
%     $n = 1$
%     &$\rownn$
%     & Euclidean
%     & Euclidean
%     & $(\tuning_1, 0)$
%     & $\indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}$
%     \\
%     $n = 1$
%     &$\colnn$
%     & Euclidean
%     & Euclidean
%     & $(0, \tuning_2)$
%     & $\indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}$
%     \\
%     $n = 1$
%     &$\tsnn$
%     & Euclidean
%     & Euclidean
%     & $(\tuning_1, \tuning_2)$
%     & $\indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}$
%     \\
%     $n = 1$
%     &$\awnn$
%     & Euclidean
%     & Euclidean
%     & $(\tuning_1, \tuning_2)$
%     & 
%     \\
%     \midrule
%     $n = 1$
%     &$\drnn$
%     & $\rownn$
%     & $+ \colnn$
%     & $- \tsnn$
%     & 
%     \\
%     \midrule
%     $n > 1$
%     &$\kernelnn$
%     & $\what{\mmd}_\kernel$
%     & $\mmd$
%     & $(\tuning_1, 0)$
%     & $\indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}$
%     \\
%     $n > 1$
%     &$\wassersteinnn$
%     & $\hatwasserstein$
%     & $\wasserstein$
%     & $(\tuning_1, 0)$
%     & $\indic{\distance{i, j}^\row \leq \tuning_1 \qtext{or} \distance{s, t}^\col \leq \tuning_2}$
%     \\
%   \end{tabular}
% \end{table}

% \kc{Make three tables depending on data types. Composition as another module. make weights explicit in the first table.}

% \begin{table}[H]
% \caption{\label{tab:summary}\textbf{Variants of nearest neighbors for scalar matrix completion \cref{eq:model}}}
%   \centering
%   \begin{tabular}{lccc}
%     \toprule
%     \tbf{Method} 
%     & ${\what\varphi}(x, y)$ 
%     & \def\arraystretch{1.2}\begin{tabular}{c} $\varphi(x, y)$
%     \end{tabular} 
%     & $\weight{j, s}$
%     \\
%     \midrule
%     $\rownn$ \ \citep{li2019nearest} (\cref{algo:vanilla-nn}) & $(x - y)^2$
%     & $(x - y)^2$
%     & $\weight{j, s}^{(i, t)}(\tuning_1, 0)$
%     \\ 
%     $\colnn$ \ \citep{li2019nearest} (\cref{algo:vanilla-nn}) & $(x - y)^2$
%     & $(x - y)^2$
%     & $\weight{j, s}^{(i, t)}(0, \tuning_2)$
%     \\
%     $\tsnn$ \ \citep{sadhukhan2024adaptivity} \textup{(\cref{algo:tsnn})}
%      & $(x - y)^2$
%      & $(x - y)^2$ 
%     & $\weight{j, s}^{(i, t)}(\tuning_1, \tuning_2)$
%     \\ 
%     $\awnn$ 
%     & $(x - y)^2$
%     & $(x - y)^2$ 
%     & $\widetilde {\weight{j, s}}^{(i, t)}$
%     \\ \bottomrule
%   \end{tabular}
% \end{table}

% \rd{we only need the second table not the first one.}

\setlength\cellspacetoplimit{5pt}
\setlength\cellspacebottomlimit{5pt}

\begin{table}[H]
  \caption{\label{tab:summary}\textbf{Variants of nearest neighbors for matrix completion.}}
  \centering
  \begin{tabular}{clccc}
    \toprule
    \tbf{Type}
    &\tbf{Method} 
    & ${\what\varphi}(x, y)$ 
    & \def\arraystretch{1.2}\begin{tabular}{c} $\varphi(x, y)$
    \end{tabular} 
    & $\weight{j, s}$
    \\
    \midrule
   $n = 1$ &
    $\rownn$ \ \citep{li2019nearest} (\cref{algo:vanilla-nn}) & $(x - y)^2$
    & $(x - y)^2$
    & $\indic{\distance{i, j}^\row\leq \tuning_1, \distance{s, t}^\col \leq 0}$
    \\ 
    % \midrule
    &
    $\colnn$ \ \citep{li2019nearest} (\cref{algo:vanilla-nn}) & $(x - y)^2$
    & $(x - y)^2$
    & $\indic{\distance{i, j}^\row\leq 0, \distance{s, t}^\col \leq \tuning_2}$
    \\
    &
    $\tsnn$ \ \citep{sadhukhan2024adaptivity} \textup{(\cref{algo:tsnn})}
     & $(x - y)^2$
     & $(x - y)^2$ 
    & $\indic{\distance{i, j}^\row\leq \tuning_1, \distance{s, t}^\col \leq \tuning_2}$
    \\ 
    % \midrule
    % \midrule
    &
    $\awnn$ \ \citep{sadhukhan2025adaptivelyweightednearestneighborsmatrix} \textup{(\cref{algo:awnn})}
    & $(x - y)^2$
    & $(x - y)^2$ 
    & $\weight{j}^\star(i, t)\cdot\indic{\distance{s, t}^\col \leq 0}$
    \\
    \noalign{\vspace{5pt}}
    \cline{2-5}
    \noalign{\vspace{5pt}}
    &
    $\drnn$ \ \citep{dwivedi2022doubly} {(\cref{algo:dsnn})}
     & \multicolumn{3}{c}{$\rownn + \colnn - \tsnn$} 
    \\
    &
    $\autonn$ \ (\cref{sec:new-nn})
     & \multicolumn{3}{c}{$\alpha \cdot \drnn + (1 - \alpha) \cdot \tsnn$} 
    \\
     \midrule
$n > 1$     &
    $\kernelnn$ \ \citep{choi2024learning} (\cref{algo:vanilla-dnn}) & $\what \mmd_\kernel^2(x, y)$
    & $\mmd_\kernel^2(x, y)$
    & $\indic{\distance{i, j}^\row\leq \tuning_1, \distance{s, t}^\col \leq 0}$
    \\
    % \midrule
    &
    $\wassersteinnn$ \ \citep{feitelberg2024distributional} (\cref{algo:vanilla-dnn}) & $\hatwasserstein^2(x, y)$
    & $\wasserstein^2(x, y)$
    & $\indic{\distance{i, j}^\row\leq \tuning_1, \distance{s, t}^\col \leq 0}$
    \\ \bottomrule
  \end{tabular}
\end{table}

% For example, if $\mc X$ is the real line then $\entrydist{x, x'} = (x - x')^2$ and 

Under the distributional matrix completion setting~($n > 1$ in \cref{eq:model}), the methods $\kernelnn$ and $\wassersteinnn$ in \cref{tab:summary} take $\mu, \nu \in \mc X$ as square integrable probability measures, and $\entrydist{\mu, \nu}$ as either the squared maximum mean discrepency~(i.e. $\mmd_\kernel^2(\mu, \nu)$, see \cite{muandet2017kernel}) or squared Wasserstein metric~(i.e., $\wasserstein(\mu, \nu)$, see \cite{bigot2020}).
% For instance under the scalar matrix completion setting, i.e., $\measurement{i, t} = \sample{1}(i, t), \measurement{j, s} = \sample{1}(i, t)$ we may set $\entrydistest{\measurement{i, t}, \measurement{j, s}} = (\measurement{i, t} - \measurement{j, s})^2$ and 
Further, the entry-wise distance $\entrydistest{x, y}$ in this case is either the unbiased U-statistics estimator $\what{\mmd}_\kernel^2(\measurement{i, t}, \measurement{j, s})$ for $\mmd_\kernel^2(\dist{i, t}, \dist{j, s})$~(see \cite{muandet2017kernel})
% the unbiased U-statistics estimator $\what{\mmd}_\kernel^2(x, y)$ for $\mmd_\kernel^2(\dist{i, t}, \dist{j, s})$~(see \cite{muandet2017kernel}) or $\entrydistest{\measurement{i, t}, \measurement{j, s}}$ as the unbiased U-statistics estimator $\what{\mmd}_\kernel^2(\measurement{i, t}, \measurement{j, s})$ for $\mmd_\kernel^2(\dist{i, t}, \dist{j, s})$~(see \cite{muandet2017kernel}) 
or the quantile based estimator $\hatwasserstein(\measurement{i, t}, \measurement{j, s})$ for $\wasserstein(\dist{i, t}, \dist{j, s})$~(see \cite{bigot2020}).





% \paragraph{Distributional nearest neighbors~($\distnn$)} Given multiple measurements $\measurement{j, s}= [\sample{1}(i, t), ..., \sample{n}(i, t)]$ per entry, we set  sequentially implement modules $\distancemod$ and $\averagemod$ sequentially with the following specifics;
% \begin{align}
%     \entrydistest{\measurement{j, s}, \measurement{j', s'}} &= \begin{cases}
%         \what{\mmd}_\kernel(\measurement{j, s}, \measurement{j', s'})  \ &\text{for $\kernelnn$}\\
%     \hatwasserstein(\measurement{j, s}, \measurement{j', s'}) \ &\text{for $\wassersteinnn$}
%     \end{cases} \ \text{and} \  \what{\mmd}_\kernel(\measurement{j, s}, \measurement{j', s'}), \ \entrydist{\dist{j, s}, \dist{j', s'}} = \mmd_\kernel(\dist{j, s}, \dist{j', s'})
% \end{align}
% \paragraph{Two-sided nearest neighbors~($\tsnn$)}

% \paragraph{Doubly-robust nearest neighbors~($\drnn$)}



% \begin{table*}[t!]
%   \caption{\label{tab:summary}\textbf{Variants of nearest neighbors}}
%   \centering
%   \resizebox{\textwidth}{!}{
%   \begin{tabular}{cccc}
%     \toprule
%     \tbf{Module}
%     & $\rownn$
%     & 
%     & \tbf{Distributional ($\wasserstein$)}
%     \\
%     \midrule
%     $\rownn$
%     & $(x-y)^2$
%     & $\what{\mmd}_\kernel(x,y)$
%     & $\hatwasserstein(x,y)$
%     \\
%     $\colnn$
%     & $\frac1n \sum_{i=1}^n x_i$
%     & Mixture distribution
%     & Wasserstein barycenter
%     \\
%     $\tsnn$
%     & $x - y$
%     & -
%     & -
%     \\
%     $\drnn$
%     & $\frac1n \sum_{i=1}^n x_i$
%     & Mixture distribution
%     & Wasserstein barycenter
%     \\
%     $\awnn$
%     & $\frac1n \sum_{i=1}^n x_i$
%     & Mixture distribution
%     & Wasserstein barycenter
%     \\
%   \end{tabular}}
% \end{table*}






% \kc{Will make the algo clean, @channel let me know how it looks like}
% \ag{Beautiful! I wonder if this might scare off the NeurIPS reviewers tho? maybe put in appendix?}



% We introduce the mathematical model for matrix completion:
% \kc{$\dist{i, t}$ to additive noise model.}
% \begin{align}
% \qtext{for} i \in [N], t\in[T]:\quad \measurement{i, t} :=
%      \begin{cases}
%         \sample{i, t} \ \sim \ \dist{i, t}&\qtext{if} \missing{i, t}=1, \\
%         \mrm{unknown}&\qtext{if} \missing{i, t}=0.
%     \end{cases}
%     \label{eq:model-scalar}
% \end{align}
% In other words, for matrix entries where $\missing{i, t} = 1$, we observe a single measurement $\measurement{i, t}$ that takes value $\sample{i, t}$ realized from distribution $\dist{i, t}$. 




% \section{Library}

\iffalse
\begin{table*}[t!]
  \caption{\label{tab:summary}\textbf{Variants of nearest neighbor data types.}}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{cccc}
    \toprule
    \tbf{Module}
    & \tbf{Scalar}
    & \tbf{Distributional ($\mmd$)}
    & \tbf{Distributional ($\wasserstein$)}
    \\
    \midrule
    $\distancemod : \entrydist{x,y}$
    & $(x-y)^2$
    & $\what{\mmd}_\kernel(x,y)$
    & $\hatwasserstein(x,y)$
    \\
    $\averagemod: (x_1,\dots,x_n)$
    & $\frac1n \sum_{i=1}^n x_i$
    & Mixture distribution
    & Wasserstein barycenter
    \\
    $\subtractmod: (x,y)$: 
    & $x - y$
    & -
    & -
  \end{tabular}}
\end{table*}

\begin{table*}[t!]
  \caption{\label{tab:summary}\textbf{Variants of nearest neighbor estimation methods.}}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{cccc}
    \toprule
    \tbf{Module}
    & \tbf{Row-wise}
    & \tbf{Two-sided}
    & \tbf{Doubly-robust}
    \\
    \midrule 
    $\distancemod : \entrydist{x,y}$
    & 
    & 
    & 
    \\
    $\averagemod: (x_1,\dots,x_n)$
    & 
    & 
    & 
    \\
    $\subtractmod: (x,y)$: 
    & 
    & 
    & 
  \end{tabular}}
\end{table*}
\fi

==> neurips2026_tmp/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our main claims in our abstract are a unified framework, a unified Python package, and a new test bench for nearest neighbor-based matrix completion methods. We present our unified framework for nearest neighbor-based matrix completion methods in \cref{sec:unified-view}. We present our package structure in \cref{sec:library}. Finally, we describe the new test bench in \cref{sec:case-study}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss improvements to our Python package in \cref{sec:conclusion}. The algorithms described in \cref{sec:nn-overview} use theoretical assumptions for their theoretical guarantees, but these assumptions do not affect the algorithms themselves, and thus pose no limitations on our Python package or test bench.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not claim any theoretical results in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All of our results can be reproduced with the code on our GitHub, which is (anonymously) linked in the paper. Each experiment has its own folder with instructions on how to run the experiments. We provide Python files which automatically download the necessary data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide an anonymous GitHub link to our open-source code. Every experiment can be reproduced with the Python files we provide separately from our Package source files. The new Python package we present, also in the GitHub link, can be installed quickly on standard computing hardware and do not require access to GPU's or any other specialized hardware.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For each experimental setup, we describe how we split up the datasets into train and test sets. We describe in detail how our hyperparameters are chosen in the Appendix. We also provide the code we use to choose hyperparameters in our open-source repository.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe how we generate our boxplots to compare error across methods in \cref{app:case-studies}. We also detail how our error bars are generated in our figures in the respective figures which have error bars.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe our computing setup in \cref{app:case-studies}. It is standard laptop hardware.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our research conforms with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work does not have any direct societal impact. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our new Python package and test bench do not pose a significant risk for misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Every library and dataset used in this work is properly cited and credited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work primarily releases a new code library that we have placed under the MIT License.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve any work with human subjects nor crowdsourcing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include any human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper's proposed algorithms do not involve LLM's in an important way.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> neurips2026_tmp/llm_evaluation.tex <==
\subsection{Efficient LLM evaluation}

Recent works show there is non-trivial variability of performance of language models across different prompting techniques\cite{sclar2023quantifying,polo2024efficient}, a natural follow up task being identification of the best performing prompting templates for certain tasks and language models~\cite{shi2024best,polo2024efficient}. The difficulty here is that there are near infinite ways of prompting, so an efficient evaluation framework has been investigated thoroughly~\cite{ye2023predictable,perlitz2023efficient}. Motivated by \cite{polo2024efficient}, we use the MMLU dataset~\cite{hendrycks2020measuring} and empirically demonstrate that our nearest neighbors method can achieve efficient evaluation. Under a fixed task~(e.g. abstract algebra, political science) various questions / examples are queried to a specific model, where each questions are restructured using different prompting templates. Either the model answers the question correctly or not and correctness is recorded. 

\paragraph{Results \& Discussion}

\kc{Do both SNN and DNN}

There are $57$ tasks and $15$ models total; the number of questions / examples depend on the task of interest and there is a fixed set of $100$ prompting templates that is applied to whatever question of whatever task. \kc{Could make a sub-section that explains MMLU.}


We consider a distributional matrix completion setup and implement a Dist-NN to estimate the distribution of averaged scores across templates~(template instances are of no value, as we aim to learn the overall variation) leveraging information across different models and different tasks. Imputation in \cite{polo2024efficient} was done while fixing model and task, so the commonalities that may exist across different models and tasks were not utilized.




% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figure/template_subject_model_by_propensity.pdf}
%     \caption{\kc{Figure needs adjustment, will not include boxplots of MMD errors for Kernel NN as most of them are zero---Wasserstein NN might have meaningful boxplots.} p = , standardize X }
%     \label{fig:temp_sub_model}
% \end{figure}


